Watermarks and Fingerprints as Soft Bindings for Content Provenance: An Open-Licence Benchmark for Images, Audio and Video

Content-provenance standards such as C2PA let a platform recover a stripped manifest through a soft binding: an invisible watermark read from the content, or a fingerprint looked up in a registry. We benchmarked both families under one protocol, restricted to openly available models whose licences we audited, on public media, with false-match rates calibrated on held-out negatives and source-level bootstrap intervals for performance estimates. For watermarking we evaluated 25 image, 7 audio and 7 video configurations from 12 methods on perceptual quality, robustness, false positives and cost; for fingerprinting, 35 methods on registries of up to 98,985 images, partial edits and adversarial attacks. PixelSeal gave the best balance for image and video watermarks and AudioSeal for audio, but the error-correcting detector of every TrustMark variant fired on 5.9 to 15.3% of unmarked images, so a verifier should test the expected payload. Among fingerprints, copy detectors trained on non-commercial data detected up to 75.5% of transformed images at a pair-level false-match rate of $10^{-7}$ and DINOv2, the best permissively licensed method, 65.0%; near-copies in a product catalogue dominated the false matches, and no detection improvement from geometric verification was observed under a matched calibration false-binding constraint in the evaluated image pipelines. On the same attacked copies the two families failed differently: the union of watermark and fingerprint successes covered 69% of image copies; fingerprints covered more audio queries, whereas expected-key watermark verification covered more video queries. Embedding a watermark moved the ISCC code of 62.0% of images past its match threshold, and platform-dependent colour conversion changed watermark bits between x86 and ARM hosts.

==> generated/numbers.tex <==
\makeatletter
\newcommand{\val}[1]{\ifcsname val@#1\endcsname\csname val@#1\endcsname\else\PackageError{numbers}{Undefined value #1}{Run the source papers' build_numbers.py and assemble.py}\fi}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/abs_dlufs\endcsname{0.013}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/abs_dlufs/hi\endcsname{0.016}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/abs_dlufs/lo\endcsname{0.010}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/blind\endcsname{0.0000}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/blindhi\endcsname{0.0089}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/blindpct\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/comb\endcsname{0.98}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/combq\endcsname{0.98}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/cost\endcsname{4.9}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/costcpu\endcsname{10}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/costgpu\endcsname{4.9}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/cpu\endcsname{60.8}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/dlufs\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/dlufs/hi\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/dlufs/lo\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/exact_gate\endcsname{0.978}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/gate\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/gpu\endcsname{4.90}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq\endcsname{4.44}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq/hi\endcsname{4.46}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq/lo\endcsname{4.42}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq_music\endcsname{4.23}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq_music/hi\endcsname{4.3}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq_music/lo\endcsname{4.1}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/pesq_pooled\endcsname{4.42}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/aac_128\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/aac_256\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/aac_64\endcsname{0.998}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/gain_-6db\endcsname{0.998}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/mp3_128\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/mp3_320\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/mp3_64\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/noise_30db\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/none\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/resample_22k\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/rob/resample_8k\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/si_snr\endcsname{27.0}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/si_snr/hi\endcsname{27.8}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/si_snr/lo\endcsname{26.1}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/snr\endcsname{27.3}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/snr/hi\endcsname{28.3}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/snr/lo\endcsname{26.4}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/spec_diff_db\endcsname{0.4}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/spec_diff_db/hi\endcsname{0.4}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/spec_diff_db/lo\endcsname{0.4}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/stoi\endcsname{0.9967}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/stoi/hi\endcsname{0.9978}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/stoi/lo\endcsname{0.9952}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/worst\endcsname{0.979}
\expandafter\def\csname val@wm:audio/AudioSeal-base@1/worstset\endcsname{music@44100}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/abs_dlufs\endcsname{0.004}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/abs_dlufs/hi\endcsname{0.007}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/abs_dlufs/lo\endcsname{0.002}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/blind\endcsname{0.0000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/blindhi\endcsname{0.0089}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/blindpct\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/comb\endcsname{0.91}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/combq\endcsname{0.94}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/cost\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/costcpu\endcsname{10}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/costgpu\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/cpu\endcsname{59.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/dlufs\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/dlufs/hi\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/dlufs/lo\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/exact_gate\endcsname{0.986}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/gate\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/gpu\endcsname{5.83}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq\endcsname{4.55}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq/hi\endcsname{4.57}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq/lo\endcsname{4.52}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq_music\endcsname{4.56}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq_music/hi\endcsname{4.6}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq_music/lo\endcsname{4.5}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/pesq_pooled\endcsname{4.55}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/aac_128\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/aac_256\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/aac_64\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/gain_-6db\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/mp3_128\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/mp3_320\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/mp3_64\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/noise_30db\endcsname{0.947}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/resample_22k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/rob/resample_8k\endcsname{0.505}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/si_snr\endcsname{32.7}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/si_snr/hi\endcsname{34.4}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/si_snr/lo\endcsname{31.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/snr\endcsname{32.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/snr/hi\endcsname{34.8}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/snr/lo\endcsname{31.1}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/spec_diff_db\endcsname{0.8}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/spec_diff_db/hi\endcsname{0.8}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/spec_diff_db/lo\endcsname{0.7}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/stoi\endcsname{0.9999}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/stoi/hi\endcsname{1.0000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/stoi/lo\endcsname{0.9999}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/worst\endcsname{0.988}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@0.5/worstset\endcsname{speech@48000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/abs_dlufs\endcsname{0.025}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/abs_dlufs/hi\endcsname{0.035}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/abs_dlufs/lo\endcsname{0.017}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/blind\endcsname{0.0000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/blindhi\endcsname{0.0089}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/blindpct\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/comb\endcsname{0.90}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/combq\endcsname{0.92}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/cost\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/costcpu\endcsname{10}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/costgpu\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/cpu\endcsname{59.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/dlufs\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/dlufs/hi\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/dlufs/lo\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/exact_gate\endcsname{0.993}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/gate\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/gpu\endcsname{5.83}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq\endcsname{4.36}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq/hi\endcsname{4.41}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq/lo\endcsname{4.29}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq_music\endcsname{4.43}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq_music/hi\endcsname{4.5}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq_music/lo\endcsname{4.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/pesq_pooled\endcsname{4.37}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/aac_128\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/aac_256\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/aac_64\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/gain_-6db\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/mp3_128\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/mp3_320\endcsname{0.996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/mp3_64\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/noise_30db\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/resample_22k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/rob/resample_8k\endcsname{0.507}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/si_snr\endcsname{25.8}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/si_snr/hi\endcsname{27.5}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/si_snr/lo\endcsname{24.2}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/snr\endcsname{26.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/snr/hi\endcsname{27.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/snr/lo\endcsname{24.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/spec_diff_db\endcsname{1.4}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/spec_diff_db/hi\endcsname{1.4}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/spec_diff_db/lo\endcsname{1.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/stoi\endcsname{0.9997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/stoi/hi\endcsname{0.9998}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/stoi/lo\endcsname{0.9996}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/worst\endcsname{0.988}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1.1/worstset\endcsname{speech@48000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/abs_dlufs\endcsname{0.018}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/abs_dlufs/hi\endcsname{0.026}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/abs_dlufs/lo\endcsname{0.012}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/blind\endcsname{0.0000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/blindhi\endcsname{0.0089}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/blindpct\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/comb\endcsname{0.90}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/combq\endcsname{0.92}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/cost\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/costcpu\endcsname{10}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/costgpu\endcsname{5.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/cpu\endcsname{59.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/dlufs\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/dlufs/hi\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/dlufs/lo\endcsname{0.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/exact_gate\endcsname{0.993}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/gate\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/gpu\endcsname{5.83}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq\endcsname{4.39}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq/hi\endcsname{4.44}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq/lo\endcsname{4.33}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq_music\endcsname{4.45}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq_music/hi\endcsname{4.5}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq_music/lo\endcsname{4.4}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/pesq_pooled\endcsname{4.40}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/aac_128\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/aac_256\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/aac_64\endcsname{0.995}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/gain_-6db\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/mp3_128\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/mp3_320\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/mp3_64\endcsname{0.997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/noise_30db\endcsname{0.999}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/resample_22k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/rob/resample_8k\endcsname{0.512}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/si_snr\endcsname{26.6}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/si_snr/hi\endcsname{28.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/si_snr/lo\endcsname{25.0}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/snr\endcsname{26.9}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/snr/hi\endcsname{28.8}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/snr/lo\endcsname{25.1}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/spec_diff_db\endcsname{1.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/spec_diff_db/hi\endcsname{1.3}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/spec_diff_db/lo\endcsname{1.2}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/stoi\endcsname{0.9998}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/stoi/hi\endcsname{0.9998}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/stoi/lo\endcsname{0.9997}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/worst\endcsname{0.989}
\expandafter\def\csname val@wm:audio/AudioSeal-streaming@1/worstset\endcsname{speech@48000}
\expandafter\def\csname val@wm:audio/Perth/abs_dlufs\endcsname{0.245}
\expandafter\def\csname val@wm:audio/Perth/abs_dlufs/hi\endcsname{0.333}
\expandafter\def\csname val@wm:audio/Perth/abs_dlufs/lo\endcsname{0.174}
\expandafter\def\csname val@wm:audio/Perth/blind\endcsname{0.0435}
\expandafter\def\csname val@wm:audio/Perth/blindhi\endcsname{0.0678}
\expandafter\def\csname val@wm:audio/Perth/blindpct\endcsname{4.3}
\expandafter\def\csname val@wm:audio/Perth/cost\endcsname{1.3}
\expandafter\def\csname val@wm:audio/Perth/costcpu\endcsname{1.3}
\expandafter\def\csname val@wm:audio/Perth/costgpu\endcsname{1.6}
\expandafter\def\csname val@wm:audio/Perth/cpu\endcsname{7.72}
\expandafter\def\csname val@wm:audio/Perth/dlufs\endcsname{0.1}
\expandafter\def\csname val@wm:audio/Perth/dlufs/hi\endcsname{0.2}
\expandafter\def\csname val@wm:audio/Perth/dlufs/lo\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/Perth/gate\endcsname{0.978}
\expandafter\def\csname val@wm:audio/Perth/gpu\endcsname{1.59}
\expandafter\def\csname val@wm:audio/Perth/pesq\endcsname{4.38}
\expandafter\def\csname val@wm:audio/Perth/pesq/hi\endcsname{4.41}
\expandafter\def\csname val@wm:audio/Perth/pesq/lo\endcsname{4.35}
\expandafter\def\csname val@wm:audio/Perth/pesq_music\endcsname{4.48}
\expandafter\def\csname val@wm:audio/Perth/pesq_music/hi\endcsname{4.5}
\expandafter\def\csname val@wm:audio/Perth/pesq_music/lo\endcsname{4.4}
\expandafter\def\csname val@wm:audio/Perth/pesq_pooled\endcsname{4.40}
\expandafter\def\csname val@wm:audio/Perth/si_snr\endcsname{15.8}
\expandafter\def\csname val@wm:audio/Perth/si_snr/hi\endcsname{16.1}
\expandafter\def\csname val@wm:audio/Perth/si_snr/lo\endcsname{15.5}
\expandafter\def\csname val@wm:audio/Perth/snr\endcsname{15.5}
\expandafter\def\csname val@wm:audio/Perth/snr/hi\endcsname{15.9}
\expandafter\def\csname val@wm:audio/Perth/snr/lo\endcsname{15.1}
\expandafter\def\csname val@wm:audio/Perth/spec_diff_db\endcsname{1.0}
\expandafter\def\csname val@wm:audio/Perth/spec_diff_db/hi\endcsname{1.2}
\expandafter\def\csname val@wm:audio/Perth/spec_diff_db/lo\endcsname{0.9}
\expandafter\def\csname val@wm:audio/Perth/stoi\endcsname{0.9931}
\expandafter\def\csname val@wm:audio/Perth/stoi/hi\endcsname{0.9936}
\expandafter\def\csname val@wm:audio/Perth/stoi/lo\endcsname{0.9922}
\expandafter\def\csname val@wm:audio/Perth/worst\endcsname{0.833}
\expandafter\def\csname val@wm:audio/Perth/worstset\endcsname{music@16000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/abs_dlufs\endcsname{0.009}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/abs_dlufs/hi\endcsname{0.013}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/abs_dlufs/lo\endcsname{0.005}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/blind\endcsname{0.0024}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/blindhi\endcsname{0.0134}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/blindpct\endcsname{0.2}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/cost\endcsname{7.1}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/costcpu\endcsname{75}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/costgpu\endcsname{7.1}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/cpu\endcsname{437}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/dlufs\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/dlufs/hi\endcsname{0.0}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/dlufs/lo\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/gate\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/gpu\endcsname{7.09}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq\endcsname{4.59}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq/hi\endcsname{4.60}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq/lo\endcsname{4.58}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq_music\endcsname{4.59}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq_music/hi\endcsname{4.6}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq_music/lo\endcsname{4.6}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/pesq_pooled\endcsname{4.59}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/aac_128\endcsname{0.992}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/aac_256\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/aac_64\endcsname{0.927}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/gain_-6db\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/mp3_128\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/mp3_320\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/mp3_64\endcsname{0.976}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/noise_30db\endcsname{0.397}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/resample_22k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/rob/resample_8k\endcsname{0.823}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/si_snr\endcsname{44.1}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/si_snr/hi\endcsname{45.0}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/si_snr/lo\endcsname{43.0}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/snr\endcsname{44.5}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/snr/hi\endcsname{45.2}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/snr/lo\endcsname{43.7}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/spec_diff_db\endcsname{1.3}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/spec_diff_db/hi\endcsname{1.4}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/spec_diff_db/lo\endcsname{1.2}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/stoi\endcsname{0.9987}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/stoi/hi\endcsname{0.9997}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/stoi/lo\endcsname{0.9970}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/worst\endcsname{1.000}
\expandafter\def\csname val@wm:audio/SilentCipher-44.1k/worstset\endcsname{music@16000}
\expandafter\def\csname val@wm:audio/WavMark/abs_dlufs\endcsname{0.008}
\expandafter\def\csname val@wm:audio/WavMark/abs_dlufs/hi\endcsname{0.021}
\expandafter\def\csname val@wm:audio/WavMark/abs_dlufs/lo\endcsname{0.001}
\expandafter\def\csname val@wm:audio/WavMark/blind\endcsname{0.0000}
\expandafter\def\csname val@wm:audio/WavMark/blindhi\endcsname{0.0089}
\expandafter\def\csname val@wm:audio/WavMark/blindpct\endcsname{0.0}
\expandafter\def\csname val@wm:audio/WavMark/comb\endcsname{0.37}
\expandafter\def\csname val@wm:audio/WavMark/combq\endcsname{0.53}
\expandafter\def\csname val@wm:audio/WavMark/cost\endcsname{34}
\expandafter\def\csname val@wm:audio/WavMark/costcpu\endcsname{--}
\expandafter\def\csname val@wm:audio/WavMark/costgpu\endcsname{34}
\expandafter\def\csname val@wm:audio/WavMark/cpu\endcsname{--}
\expandafter\def\csname val@wm:audio/WavMark/dlufs\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/WavMark/dlufs/hi\endcsname{0.0}
\expandafter\def\csname val@wm:audio/WavMark/dlufs/lo\endcsname{-0.0}
\expandafter\def\csname val@wm:audio/WavMark/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/gate\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/gpu\endcsname{33.5}
\expandafter\def\csname val@wm:audio/WavMark/keytrials\endcsname{21{,}114}
\expandafter\def\csname val@wm:audio/WavMark/keyupper\endcsname{0.00014}
\expandafter\def\csname val@wm:audio/WavMark/pesq\endcsname{4.15}
\expandafter\def\csname val@wm:audio/WavMark/pesq/hi\endcsname{4.21}
\expandafter\def\csname val@wm:audio/WavMark/pesq/lo\endcsname{4.08}
\expandafter\def\csname val@wm:audio/WavMark/pesq_music\endcsname{4.36}
\expandafter\def\csname val@wm:audio/WavMark/pesq_music/hi\endcsname{4.5}
\expandafter\def\csname val@wm:audio/WavMark/pesq_music/lo\endcsname{4.2}
\expandafter\def\csname val@wm:audio/WavMark/pesq_pooled\endcsname{4.18}
\expandafter\def\csname val@wm:audio/WavMark/rob/aac_128\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/aac_256\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/aac_64\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/gain_-6db\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/mp3_128\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/mp3_320\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/mp3_64\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/noise_30db\endcsname{0.967}
\expandafter\def\csname val@wm:audio/WavMark/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/resample_22k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/rob/resample_8k\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/si_snr\endcsname{35.9}
\expandafter\def\csname val@wm:audio/WavMark/si_snr/hi\endcsname{36.5}
\expandafter\def\csname val@wm:audio/WavMark/si_snr/lo\endcsname{35.0}
\expandafter\def\csname val@wm:audio/WavMark/snr\endcsname{36.3}
\expandafter\def\csname val@wm:audio/WavMark/snr/hi\endcsname{36.6}
\expandafter\def\csname val@wm:audio/WavMark/snr/lo\endcsname{35.9}
\expandafter\def\csname val@wm:audio/WavMark/spec_diff_db\endcsname{2.8}
\expandafter\def\csname val@wm:audio/WavMark/spec_diff_db/hi\endcsname{3.0}
\expandafter\def\csname val@wm:audio/WavMark/spec_diff_db/lo\endcsname{2.6}
\expandafter\def\csname val@wm:audio/WavMark/stoi\endcsname{0.9932}
\expandafter\def\csname val@wm:audio/WavMark/stoi/hi\endcsname{0.9973}
\expandafter\def\csname val@wm:audio/WavMark/stoi/lo\endcsname{0.9873}
\expandafter\def\csname val@wm:audio/WavMark/worst\endcsname{1.000}
\expandafter\def\csname val@wm:audio/WavMark/worstset\endcsname{music@16000}
\expandafter\def\csname val@wm:audio/n_configs\endcsname{7}
\expandafter\def\csname val@wm:audio/n_items\endcsname{138}
\expandafter\def\csname val@wm:audio/n_music\endcsname{18}
\expandafter\def\csname val@wm:audio/n_qualify\endcsname{5}
\expandafter\def\csname val@wm:audio/n_sources\endcsname{46}
\expandafter\def\csname val@wm:audio/n_speech\endcsname{120}
\expandafter\def\csname val@wm:audio/win/combined\endcsname{AudioSeal base (1)}
\expandafter\def\csname val@wm:audio/win/combined_q\endcsname{AudioSeal base (1)}
\expandafter\def\csname val@wm:audio/win/cost\endcsname{AudioSeal base (1)}
\expandafter\def\csname val@wm:audio/win/speed\endcsname{AudioSeal base (1)}
\expandafter\def\csname val@wm:audioseal/unmarked_max_score\endcsname{0.24}
\expandafter\def\csname val@wm:corpus/audio\endcsname{141}
\expandafter\def\csname val@wm:corpus/image\endcsname{160}
\expandafter\def\csname val@wm:corpus/video\endcsname{10}
\expandafter\def\csname val@wm:count/audio\endcsname{7}
\expandafter\def\csname val@wm:count/families\endcsname{12}
\expandafter\def\csname val@wm:count/image\endcsname{25}
\expandafter\def\csname val@wm:count/transforms\endcsname{32}
\expandafter\def\csname val@wm:count/transforms/audio\endcsname{10}
\expandafter\def\csname val@wm:count/transforms/image\endcsname{14}
\expandafter\def\csname val@wm:count/transforms/video\endcsname{8}
\expandafter\def\csname val@wm:count/video\endcsname{7}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal base/blind_src_fm\endcsname{0}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal base/blind_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal base/blind_src_upper\endcsname{7.7}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal streaming/blind_src_fm\endcsname{0}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal streaming/blind_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/AudioSeal streaming/blind_src_upper\endcsname{7.7}
\expandafter\def\csname val@wm:fpr/audio/Perth/blind_src_fm\endcsname{2}
\expandafter\def\csname val@wm:fpr/audio/Perth/blind_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/Perth/blind_src_upper\endcsname{14.8}
\expandafter\def\csname val@wm:fpr/audio/SilentCipher/blind_src_fm\endcsname{1}
\expandafter\def\csname val@wm:fpr/audio/SilentCipher/blind_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/SilentCipher/blind_src_upper\endcsname{11.5}
\expandafter\def\csname val@wm:fpr/audio/SilentCipher/own_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/SilentCipher/own_src_upper\endcsname{7.7}
\expandafter\def\csname val@wm:fpr/audio/WavMark/blind_src_fm\endcsname{0}
\expandafter\def\csname val@wm:fpr/audio/WavMark/blind_src_n\endcsname{46}
\expandafter\def\csname val@wm:fpr/audio/WavMark/blind_src_upper\endcsname{7.7}
\expandafter\def\csname val@wm:fpr/image/ChunkySeal/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/ChunkySeal/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/InvisMark/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/InvisMark/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/PixelSeal/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/PixelSeal/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/RivaGAN/own_src_n\endcsname{60}
\expandafter\def\csname val@wm:fpr/image/RivaGAN/own_src_upper\endcsname{6.0}
\expandafter\def\csname val@wm:fpr/image/TrustMark-B/blind_src_fm\endcsname{10}
\expandafter\def\csname val@wm:fpr/image/TrustMark-B/blind_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-B/blind_src_upper\endcsname{20.6}
\expandafter\def\csname val@wm:fpr/image/TrustMark-B/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-B/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/TrustMark-C/blind_src_fm\endcsname{13}
\expandafter\def\csname val@wm:fpr/image/TrustMark-C/blind_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-C/blind_src_upper\endcsname{24.7}
\expandafter\def\csname val@wm:fpr/image/TrustMark-C/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-C/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/TrustMark-P/blind_src_fm\endcsname{5}
\expandafter\def\csname val@wm:fpr/image/TrustMark-P/blind_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-P/blind_src_upper\endcsname{13.2}
\expandafter\def\csname val@wm:fpr/image/TrustMark-P/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-P/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/TrustMark-Q/blind_src_fm\endcsname{8}
\expandafter\def\csname val@wm:fpr/image/TrustMark-Q/blind_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-Q/blind_src_upper\endcsname{17.7}
\expandafter\def\csname val@wm:fpr/image/TrustMark-Q/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/TrustMark-Q/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/VideoSeal-1.0/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/VideoSeal-1.0/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/WAM/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/WAM/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/image/invisible-watermark/own_src_n\endcsname{85}
\expandafter\def\csname val@wm:fpr/image/invisible-watermark/own_src_upper\endcsname{4.2}
\expandafter\def\csname val@wm:fpr/sources_for_1e-3\endcsname{3{,}688}
\expandafter\def\csname val@wm:fpr/video/ChunkySeal/own_src_n\endcsname{6}
\expandafter\def\csname val@wm:fpr/video/ChunkySeal/own_src_upper\endcsname{45.9}
\expandafter\def\csname val@wm:fpr/video/PixelSeal/own_src_n\endcsname{6}
\expandafter\def\csname val@wm:fpr/video/PixelSeal/own_src_upper\endcsname{45.9}
\expandafter\def\csname val@wm:fpr/video/VideoSeal-1.0/own_src_n\endcsname{6}
\expandafter\def\csname val@wm:fpr/video/VideoSeal-1.0/own_src_upper\endcsname{45.9}
\expandafter\def\csname val@wm:image/ChunkySeal@default/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/ChunkySeal@default/costcpu\endcsname{0.92}
\expandafter\def\csname val@wm:image/ChunkySeal@default/costgpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/ChunkySeal@default/cpu\endcsname{19069}
\expandafter\def\csname val@wm:image/ChunkySeal@default/cvvdp\endcsname{9.84}
\expandafter\def\csname val@wm:image/ChunkySeal@default/cvvdp/hi\endcsname{9.87}
\expandafter\def\csname val@wm:image/ChunkySeal@default/cvvdp/lo\endcsname{9.80}
\expandafter\def\csname val@wm:image/ChunkySeal@default/exact_gate\endcsname{0.035}
\expandafter\def\csname val@wm:image/ChunkySeal@default/flip\endcsname{0.048}
\expandafter\def\csname val@wm:image/ChunkySeal@default/flip/hi\endcsname{0.050}
\expandafter\def\csname val@wm:image/ChunkySeal@default/flip/lo\endcsname{0.045}
\expandafter\def\csname val@wm:image/ChunkySeal@default/gate\endcsname{0.934}
\expandafter\def\csname val@wm:image/ChunkySeal@default/gpu\endcsname{50.4}
\expandafter\def\csname val@wm:image/ChunkySeal@default/keymatch_gate\endcsname{0.941}
\expandafter\def\csname val@wm:image/ChunkySeal@default/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/ChunkySeal@default/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/ChunkySeal@default/lpips\endcsname{0.0090}
\expandafter\def\csname val@wm:image/ChunkySeal@default/lpips/hi\endcsname{0.0101}
\expandafter\def\csname val@wm:image/ChunkySeal@default/lpips/lo\endcsname{0.0080}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ms_ssim\endcsname{0.9961}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ms_ssim/hi\endcsname{0.9965}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ms_ssim/lo\endcsname{0.9957}
\expandafter\def\csname val@wm:image/ChunkySeal@default/psnr\endcsname{44.4}
\expandafter\def\csname val@wm:image/ChunkySeal@default/psnr/hi\endcsname{44.8}
\expandafter\def\csname val@wm:image/ChunkySeal@default/psnr/lo\endcsname{44.0}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/blur1\endcsname{0.998}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/bright0.8\endcsname{0.998}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/bright1.2\endcsname{0.997}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/crop50\endcsname{0.842}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/crop70\endcsname{0.973}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/crop90\endcsname{0.993}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/jpeg50\endcsname{0.890}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/jpeg60\endcsname{0.912}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/jpeg75\endcsname{0.934}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/jpeg90\endcsname{0.997}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/none\endcsname{0.998}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/resize0.5\endcsname{0.998}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/resize0.75\endcsname{0.998}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/webp60\endcsname{0.861}
\expandafter\def\csname val@wm:image/ChunkySeal@default/rob/webp80\endcsname{0.922}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ssim\endcsname{0.9925}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ssim/hi\endcsname{0.9940}
\expandafter\def\csname val@wm:image/ChunkySeal@default/ssim/lo\endcsname{0.9909}
\expandafter\def\csname val@wm:image/ChunkySeal@default/worst\endcsname{0.789}
\expandafter\def\csname val@wm:image/ChunkySeal@default/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/comb\endcsname{0.20}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/combq\endcsname{0.28}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/costgpu\endcsname{0.11}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/cpu\endcsname{296}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/cvvdp\endcsname{9.90}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/cvvdp/hi\endcsname{9.92}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/cvvdp/lo\endcsname{9.88}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/exact_gate\endcsname{0.576}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/flip\endcsname{0.051}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/flip/hi\endcsname{0.054}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/flip/lo\endcsname{0.049}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/gate\endcsname{0.974}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/gpu\endcsname{409}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/keymatch_gate\endcsname{0.953}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/lpips\endcsname{0.0323}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/lpips/hi\endcsname{0.0371}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/lpips/lo\endcsname{0.0279}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ms_ssim\endcsname{0.9862}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ms_ssim/hi\endcsname{0.9874}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ms_ssim/lo\endcsname{0.9850}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/psnr\endcsname{39.1}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/psnr/hi\endcsname{39.5}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/psnr/lo\endcsname{38.8}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/bright0.8\endcsname{0.564}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/bright1.2\endcsname{0.687}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/crop50\endcsname{0.646}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/crop70\endcsname{0.514}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/crop90\endcsname{0.525}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/jpeg50\endcsname{0.781}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/jpeg60\endcsname{0.884}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/jpeg75\endcsname{0.974}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/resize0.5\endcsname{0.511}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/resize0.75\endcsname{0.525}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/webp60\endcsname{0.706}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/rob/webp80\endcsname{0.783}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ssim\endcsname{0.9782}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ssim/hi\endcsname{0.9802}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/ssim/lo\endcsname{0.9759}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/worst\endcsname{0.961}
\expandafter\def\csname val@wm:image/DWT-DCT-SVD/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/DWT-DCT/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/DWT-DCT/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/DWT-DCT/costgpu\endcsname{0.11}
\expandafter\def\csname val@wm:image/DWT-DCT/cpu\endcsname{296}
\expandafter\def\csname val@wm:image/DWT-DCT/cvvdp\endcsname{9.95}
\expandafter\def\csname val@wm:image/DWT-DCT/cvvdp/hi\endcsname{9.96}
\expandafter\def\csname val@wm:image/DWT-DCT/cvvdp/lo\endcsname{9.95}
\expandafter\def\csname val@wm:image/DWT-DCT/exact_gate\endcsname{0.000}
\expandafter\def\csname val@wm:image/DWT-DCT/flip\endcsname{0.029}
\expandafter\def\csname val@wm:image/DWT-DCT/flip/hi\endcsname{0.030}
\expandafter\def\csname val@wm:image/DWT-DCT/flip/lo\endcsname{0.028}
\expandafter\def\csname val@wm:image/DWT-DCT/gate\endcsname{0.518}
\expandafter\def\csname val@wm:image/DWT-DCT/gpu\endcsname{409}
\expandafter\def\csname val@wm:image/DWT-DCT/keymatch_gate\endcsname{0.012}
\expandafter\def\csname val@wm:image/DWT-DCT/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/DWT-DCT/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/DWT-DCT/lpips\endcsname{0.0212}
\expandafter\def\csname val@wm:image/DWT-DCT/lpips/hi\endcsname{0.0261}
\expandafter\def\csname val@wm:image/DWT-DCT/lpips/lo\endcsname{0.0169}
\expandafter\def\csname val@wm:image/DWT-DCT/ms_ssim\endcsname{0.9896}
\expandafter\def\csname val@wm:image/DWT-DCT/ms_ssim/hi\endcsname{0.9905}
\expandafter\def\csname val@wm:image/DWT-DCT/ms_ssim/lo\endcsname{0.9887}
\expandafter\def\csname val@wm:image/DWT-DCT/psnr\endcsname{39.3}
\expandafter\def\csname val@wm:image/DWT-DCT/psnr/hi\endcsname{39.6}
\expandafter\def\csname val@wm:image/DWT-DCT/psnr/lo\endcsname{38.9}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/blur1\endcsname{0.688}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/bright0.8\endcsname{0.831}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/bright1.2\endcsname{0.867}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/crop50\endcsname{0.593}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/crop70\endcsname{0.496}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/crop90\endcsname{0.506}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/jpeg50\endcsname{0.498}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/jpeg60\endcsname{0.507}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/jpeg75\endcsname{0.518}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/jpeg90\endcsname{0.906}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/none\endcsname{0.875}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/resize0.5\endcsname{0.495}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/resize0.75\endcsname{0.503}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/webp60\endcsname{0.489}
\expandafter\def\csname val@wm:image/DWT-DCT/rob/webp80\endcsname{0.517}
\expandafter\def\csname val@wm:image/DWT-DCT/ssim\endcsname{0.9673}
\expandafter\def\csname val@wm:image/DWT-DCT/ssim/hi\endcsname{0.9698}
\expandafter\def\csname val@wm:image/DWT-DCT/ssim/lo\endcsname{0.9648}
\expandafter\def\csname val@wm:image/DWT-DCT/worst\endcsname{0.508}
\expandafter\def\csname val@wm:image/DWT-DCT/worstset\endcsname{hdr16}
\expandafter\def\csname val@wm:image/InvisMark/cost\endcsname{0.0024}
\expandafter\def\csname val@wm:image/InvisMark/costcpu\endcsname{--}
\expandafter\def\csname val@wm:image/InvisMark/costgpu\endcsname{0.0024}
\expandafter\def\csname val@wm:image/InvisMark/cpu\endcsname{--}
\expandafter\def\csname val@wm:image/InvisMark/cvvdp\endcsname{9.99}
\expandafter\def\csname val@wm:image/InvisMark/cvvdp/hi\endcsname{9.99}
\expandafter\def\csname val@wm:image/InvisMark/cvvdp/lo\endcsname{9.99}
\expandafter\def\csname val@wm:image/InvisMark/exact_gate\endcsname{0.000}
\expandafter\def\csname val@wm:image/InvisMark/flip\endcsname{0.022}
\expandafter\def\csname val@wm:image/InvisMark/flip/hi\endcsname{0.024}
\expandafter\def\csname val@wm:image/InvisMark/flip/lo\endcsname{0.020}
\expandafter\def\csname val@wm:image/InvisMark/gate\endcsname{0.919}
\expandafter\def\csname val@wm:image/InvisMark/gpu\endcsname{8.73}
\expandafter\def\csname val@wm:image/InvisMark/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/InvisMark/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/InvisMark/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/InvisMark/lpips\endcsname{0.0017}
\expandafter\def\csname val@wm:image/InvisMark/lpips/hi\endcsname{0.0019}
\expandafter\def\csname val@wm:image/InvisMark/lpips/lo\endcsname{0.0015}
\expandafter\def\csname val@wm:image/InvisMark/ms_ssim\endcsname{0.9990}
\expandafter\def\csname val@wm:image/InvisMark/ms_ssim/hi\endcsname{0.9991}
\expandafter\def\csname val@wm:image/InvisMark/ms_ssim/lo\endcsname{0.9988}
\expandafter\def\csname val@wm:image/InvisMark/psnr\endcsname{50.1}
\expandafter\def\csname val@wm:image/InvisMark/psnr/hi\endcsname{50.6}
\expandafter\def\csname val@wm:image/InvisMark/psnr/lo\endcsname{49.6}
\expandafter\def\csname val@wm:image/InvisMark/rob/blur1\endcsname{0.949}
\expandafter\def\csname val@wm:image/InvisMark/rob/bright0.8\endcsname{0.950}
\expandafter\def\csname val@wm:image/InvisMark/rob/bright1.2\endcsname{0.943}
\expandafter\def\csname val@wm:image/InvisMark/rob/crop50\endcsname{0.506}
\expandafter\def\csname val@wm:image/InvisMark/rob/crop70\endcsname{0.939}
\expandafter\def\csname val@wm:image/InvisMark/rob/crop90\endcsname{0.932}
\expandafter\def\csname val@wm:image/InvisMark/rob/jpeg50\endcsname{0.841}
\expandafter\def\csname val@wm:image/InvisMark/rob/jpeg60\endcsname{0.871}
\expandafter\def\csname val@wm:image/InvisMark/rob/jpeg75\endcsname{0.919}
\expandafter\def\csname val@wm:image/InvisMark/rob/jpeg90\endcsname{0.949}
\expandafter\def\csname val@wm:image/InvisMark/rob/none\endcsname{0.950}
\expandafter\def\csname val@wm:image/InvisMark/rob/resize0.5\endcsname{0.949}
\expandafter\def\csname val@wm:image/InvisMark/rob/resize0.75\endcsname{0.950}
\expandafter\def\csname val@wm:image/InvisMark/rob/webp60\endcsname{0.789}
\expandafter\def\csname val@wm:image/InvisMark/rob/webp80\endcsname{0.848}
\expandafter\def\csname val@wm:image/InvisMark/ssim\endcsname{0.9963}
\expandafter\def\csname val@wm:image/InvisMark/ssim/hi\endcsname{0.9976}
\expandafter\def\csname val@wm:image/InvisMark/ssim/lo\endcsname{0.9947}
\expandafter\def\csname val@wm:image/InvisMark/worst\endcsname{0.873}
\expandafter\def\csname val@wm:image/InvisMark/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/cost\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/costcpu\endcsname{0.053}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/costgpu\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/cpu\endcsname{1104}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/cvvdp\endcsname{9.97}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/cvvdp/hi\endcsname{9.97}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/cvvdp/lo\endcsname{9.97}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/exact_gate\endcsname{0.024}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/flip\endcsname{0.016}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/flip/hi\endcsname{0.017}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/flip/lo\endcsname{0.015}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/gate\endcsname{0.907}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/gpu\endcsname{9.13}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/keymatch_gate\endcsname{0.988}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/lpips\endcsname{0.0006}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/lpips/hi\endcsname{0.0007}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/lpips/lo\endcsname{0.0005}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ms_ssim\endcsname{0.9993}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ms_ssim/hi\endcsname{0.9994}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ms_ssim/lo\endcsname{0.9993}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/psnr\endcsname{51.6}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/psnr/hi\endcsname{52.1}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/psnr/lo\endcsname{51.1}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/blur1\endcsname{0.916}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/bright0.8\endcsname{0.919}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/bright1.2\endcsname{0.908}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/crop50\endcsname{0.679}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/crop70\endcsname{0.808}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/crop90\endcsname{0.872}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/jpeg50\endcsname{0.876}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/jpeg60\endcsname{0.884}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/jpeg75\endcsname{0.907}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/jpeg90\endcsname{0.920}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/none\endcsname{0.923}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/resize0.5\endcsname{0.920}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/resize0.75\endcsname{0.922}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/webp60\endcsname{0.843}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/rob/webp80\endcsname{0.874}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ssim\endcsname{0.9983}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ssim/hi\endcsname{0.9988}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/ssim/lo\endcsname{0.9977}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/worst\endcsname{0.863}
\expandafter\def\csname val@wm:image/PixelSeal@0.1/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/cost\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/costcpu\endcsname{0.053}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/costgpu\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/cpu\endcsname{1104}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/cvvdp\endcsname{9.95}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/cvvdp/hi\endcsname{9.96}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/cvvdp/lo\endcsname{9.94}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/exact_gate\endcsname{0.106}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/flip\endcsname{0.020}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/flip/hi\endcsname{0.021}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/flip/lo\endcsname{0.019}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/gate\endcsname{0.965}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/gpu\endcsname{9.13}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/keymatch_gate\endcsname{0.988}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/lpips\endcsname{0.0009}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/lpips/hi\endcsname{0.0010}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/lpips/lo\endcsname{0.0008}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ms_ssim\endcsname{0.9990}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ms_ssim/hi\endcsname{0.9991}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ms_ssim/lo\endcsname{0.9989}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/psnr\endcsname{49.8}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/psnr/hi\endcsname{50.2}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/psnr/lo\endcsname{49.3}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/blur1\endcsname{0.971}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/bright0.8\endcsname{0.973}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/bright1.2\endcsname{0.969}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/crop50\endcsname{0.770}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/crop70\endcsname{0.904}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/crop90\endcsname{0.957}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/jpeg50\endcsname{0.943}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/jpeg60\endcsname{0.950}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/jpeg75\endcsname{0.965}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/jpeg90\endcsname{0.974}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/none\endcsname{0.977}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/resize0.5\endcsname{0.976}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/resize0.75\endcsname{0.975}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/webp60\endcsname{0.920}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/rob/webp80\endcsname{0.941}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ssim\endcsname{0.9976}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ssim/hi\endcsname{0.9983}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/ssim/lo\endcsname{0.9966}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/worst\endcsname{0.936}
\expandafter\def\csname val@wm:image/PixelSeal@0.125/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/comb\endcsname{0.95}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/combq\endcsname{0.94}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/cost\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/costcpu\endcsname{0.053}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/costgpu\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/cpu\endcsname{1104}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/cvvdp\endcsname{9.93}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/cvvdp/hi\endcsname{9.94}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/cvvdp/lo\endcsname{9.92}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/exact_gate\endcsname{0.318}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/flip\endcsname{0.024}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/flip/hi\endcsname{0.025}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/flip/lo\endcsname{0.022}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/gate\endcsname{0.988}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/gpu\endcsname{9.13}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/lpips\endcsname{0.0012}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/lpips/hi\endcsname{0.0014}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/lpips/lo\endcsname{0.0011}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ms_ssim\endcsname{0.9986}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ms_ssim/hi\endcsname{0.9987}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ms_ssim/lo\endcsname{0.9985}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/psnr\endcsname{48.3}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/psnr/hi\endcsname{48.7}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/psnr/lo\endcsname{47.8}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/blur1\endcsname{0.992}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/bright0.8\endcsname{0.992}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/bright1.2\endcsname{0.988}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/crop50\endcsname{0.826}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/crop70\endcsname{0.957}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/crop90\endcsname{0.984}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/jpeg50\endcsname{0.976}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/jpeg60\endcsname{0.981}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/jpeg75\endcsname{0.988}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/jpeg90\endcsname{0.992}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/none\endcsname{0.993}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/resize0.5\endcsname{0.992}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/resize0.75\endcsname{0.993}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/webp60\endcsname{0.958}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/rob/webp80\endcsname{0.977}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ssim\endcsname{0.9969}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ssim/hi\endcsname{0.9977}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/ssim/lo\endcsname{0.9958}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/worst\endcsname{0.980}
\expandafter\def\csname val@wm:image/PixelSeal@0.15/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/comb\endcsname{0.79}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/combq\endcsname{0.65}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/cost\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/costcpu\endcsname{0.053}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/costgpu\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/cpu\endcsname{1104}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/cvvdp\endcsname{9.57}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/cvvdp/hi\endcsname{9.61}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/cvvdp/lo\endcsname{9.53}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/exact_gate\endcsname{0.871}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/flip\endcsname{0.051}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/flip/hi\endcsname{0.054}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/flip/lo\endcsname{0.049}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/gate\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/gpu\endcsname{9.13}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/lpips\endcsname{0.0077}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/lpips/hi\endcsname{0.0087}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/lpips/lo\endcsname{0.0068}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ms_ssim\endcsname{0.9915}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ms_ssim/hi\endcsname{0.9921}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ms_ssim/lo\endcsname{0.9910}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/psnr\endcsname{40.1}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/psnr/hi\endcsname{40.6}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/psnr/lo\endcsname{39.6}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/bright1.2\endcsname{0.998}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/crop50\endcsname{0.911}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/crop70\endcsname{0.994}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/crop90\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/jpeg60\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/jpeg75\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/webp60\endcsname{0.998}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/rob/webp80\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ssim\endcsname{0.9863}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ssim/hi\endcsname{0.9888}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/ssim/lo\endcsname{0.9835}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@0.4/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/PixelSeal@default/comb\endcsname{0.90}
\expandafter\def\csname val@wm:image/PixelSeal@default/combq\endcsname{0.84}
\expandafter\def\csname val@wm:image/PixelSeal@default/cost\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@default/costcpu\endcsname{0.053}
\expandafter\def\csname val@wm:image/PixelSeal@default/costgpu\endcsname{0.0026}
\expandafter\def\csname val@wm:image/PixelSeal@default/cpu\endcsname{1104}
\expandafter\def\csname val@wm:image/PixelSeal@default/cvvdp\endcsname{9.88}
\expandafter\def\csname val@wm:image/PixelSeal@default/cvvdp/hi\endcsname{9.89}
\expandafter\def\csname val@wm:image/PixelSeal@default/cvvdp/lo\endcsname{9.86}
\expandafter\def\csname val@wm:image/PixelSeal@default/exact_gate\endcsname{0.765}
\expandafter\def\csname val@wm:image/PixelSeal@default/flip\endcsname{0.030}
\expandafter\def\csname val@wm:image/PixelSeal@default/flip/hi\endcsname{0.032}
\expandafter\def\csname val@wm:image/PixelSeal@default/flip/lo\endcsname{0.028}
\expandafter\def\csname val@wm:image/PixelSeal@default/gate\endcsname{0.998}
\expandafter\def\csname val@wm:image/PixelSeal@default/gpu\endcsname{9.13}
\expandafter\def\csname val@wm:image/PixelSeal@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/PixelSeal@default/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/PixelSeal@default/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/PixelSeal@default/lpips\endcsname{0.0020}
\expandafter\def\csname val@wm:image/PixelSeal@default/lpips/hi\endcsname{0.0022}
\expandafter\def\csname val@wm:image/PixelSeal@default/lpips/lo\endcsname{0.0018}
\expandafter\def\csname val@wm:image/PixelSeal@default/ms_ssim\endcsname{0.9977}
\expandafter\def\csname val@wm:image/PixelSeal@default/ms_ssim/hi\endcsname{0.9978}
\expandafter\def\csname val@wm:image/PixelSeal@default/ms_ssim/lo\endcsname{0.9975}
\expandafter\def\csname val@wm:image/PixelSeal@default/psnr\endcsname{45.9}
\expandafter\def\csname val@wm:image/PixelSeal@default/psnr/hi\endcsname{46.4}
\expandafter\def\csname val@wm:image/PixelSeal@default/psnr/lo\endcsname{45.5}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/blur1\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/bright0.8\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/bright1.2\endcsname{0.997}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/crop50\endcsname{0.877}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/crop70\endcsname{0.986}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/crop90\endcsname{0.997}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/jpeg50\endcsname{0.994}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/jpeg60\endcsname{0.996}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/jpeg75\endcsname{0.998}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/jpeg90\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/none\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/resize0.5\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/resize0.75\endcsname{0.999}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/webp60\endcsname{0.985}
\expandafter\def\csname val@wm:image/PixelSeal@default/rob/webp80\endcsname{0.994}
\expandafter\def\csname val@wm:image/PixelSeal@default/ssim\endcsname{0.9952}
\expandafter\def\csname val@wm:image/PixelSeal@default/ssim/hi\endcsname{0.9964}
\expandafter\def\csname val@wm:image/PixelSeal@default/ssim/lo\endcsname{0.9937}
\expandafter\def\csname val@wm:image/PixelSeal@default/worst\endcsname{0.996}
\expandafter\def\csname val@wm:image/PixelSeal@default/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/RivaGAN/cost\endcsname{1.5}
\expandafter\def\csname val@wm:image/RivaGAN/costcpu\endcsname{--}
\expandafter\def\csname val@wm:image/RivaGAN/costgpu\endcsname{1.5}
\expandafter\def\csname val@wm:image/RivaGAN/cpu\endcsname{--}
\expandafter\def\csname val@wm:image/RivaGAN/cvvdp\endcsname{9.85}
\expandafter\def\csname val@wm:image/RivaGAN/cvvdp/hi\endcsname{9.88}
\expandafter\def\csname val@wm:image/RivaGAN/cvvdp/lo\endcsname{9.82}
\expandafter\def\csname val@wm:image/RivaGAN/exact_gate\endcsname{0.900}
\expandafter\def\csname val@wm:image/RivaGAN/flip\endcsname{0.077}
\expandafter\def\csname val@wm:image/RivaGAN/flip/hi\endcsname{0.080}
\expandafter\def\csname val@wm:image/RivaGAN/flip/lo\endcsname{0.074}
\expandafter\def\csname val@wm:image/RivaGAN/gate\endcsname{0.996}
\expandafter\def\csname val@wm:image/RivaGAN/gpu\endcsname{5250}
\expandafter\def\csname val@wm:image/RivaGAN/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/RivaGAN/keytrials\endcsname{12{,}240}
\expandafter\def\csname val@wm:image/RivaGAN/keyupper\endcsname{0.00024}
\expandafter\def\csname val@wm:image/RivaGAN/lpips\endcsname{0.0643}
\expandafter\def\csname val@wm:image/RivaGAN/lpips/hi\endcsname{0.0764}
\expandafter\def\csname val@wm:image/RivaGAN/lpips/lo\endcsname{0.0530}
\expandafter\def\csname val@wm:image/RivaGAN/ms_ssim\endcsname{0.9852}
\expandafter\def\csname val@wm:image/RivaGAN/ms_ssim/hi\endcsname{0.9867}
\expandafter\def\csname val@wm:image/RivaGAN/ms_ssim/lo\endcsname{0.9837}
\expandafter\def\csname val@wm:image/RivaGAN/psnr\endcsname{40.5}
\expandafter\def\csname val@wm:image/RivaGAN/psnr/hi\endcsname{40.6}
\expandafter\def\csname val@wm:image/RivaGAN/psnr/lo\endcsname{40.5}
\expandafter\def\csname val@wm:image/RivaGAN/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/RivaGAN/rob/bright0.8\endcsname{0.999}
\expandafter\def\csname val@wm:image/RivaGAN/rob/bright1.2\endcsname{1.000}
\expandafter\def\csname val@wm:image/RivaGAN/rob/crop50\endcsname{0.998}
\expandafter\def\csname val@wm:image/RivaGAN/rob/crop70\endcsname{0.999}
\expandafter\def\csname val@wm:image/RivaGAN/rob/crop90\endcsname{0.999}
\expandafter\def\csname val@wm:image/RivaGAN/rob/jpeg50\endcsname{0.968}
\expandafter\def\csname val@wm:image/RivaGAN/rob/jpeg60\endcsname{0.984}
\expandafter\def\csname val@wm:image/RivaGAN/rob/jpeg75\endcsname{0.996}
\expandafter\def\csname val@wm:image/RivaGAN/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/RivaGAN/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/RivaGAN/rob/resize0.5\endcsname{0.833}
\expandafter\def\csname val@wm:image/RivaGAN/rob/resize0.75\endcsname{0.993}
\expandafter\def\csname val@wm:image/RivaGAN/rob/webp60\endcsname{0.952}
\expandafter\def\csname val@wm:image/RivaGAN/rob/webp80\endcsname{0.991}
\expandafter\def\csname val@wm:image/RivaGAN/ssim\endcsname{0.9735}
\expandafter\def\csname val@wm:image/RivaGAN/ssim/hi\endcsname{0.9760}
\expandafter\def\csname val@wm:image/RivaGAN/ssim/lo\endcsname{0.9709}
\expandafter\def\csname val@wm:image/RivaGAN/worst\endcsname{0.988}
\expandafter\def\csname val@wm:image/RivaGAN/worstset\endcsname{hdr16}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/cost\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/costcpu\endcsname{0.026}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/costgpu\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/cpu\endcsname{544}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/cvvdp\endcsname{9.95}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/cvvdp/hi\endcsname{9.96}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/cvvdp/lo\endcsname{9.95}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/exact_gate\endcsname{0.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/flip\endcsname{0.018}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/flip/hi\endcsname{0.020}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/flip/lo\endcsname{0.017}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/gate\endcsname{0.887}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/gpu\endcsname{8.79}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/lpips\endcsname{0.0006}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/lpips/hi\endcsname{0.0007}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/lpips/lo\endcsname{0.0006}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ms_ssim\endcsname{0.9992}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ms_ssim/hi\endcsname{0.9992}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ms_ssim/lo\endcsname{0.9991}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/psnr\endcsname{50.5}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/psnr/hi\endcsname{51.0}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/psnr/lo\endcsname{50.1}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/blur1\endcsname{0.899}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/bright0.8\endcsname{0.897}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/bright1.2\endcsname{0.884}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/crop50\endcsname{0.502}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/crop70\endcsname{0.552}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/crop90\endcsname{0.792}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/jpeg50\endcsname{0.867}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/jpeg60\endcsname{0.873}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/jpeg75\endcsname{0.887}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/jpeg90\endcsname{0.895}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/none\endcsname{0.901}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/resize0.5\endcsname{0.899}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/resize0.75\endcsname{0.899}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/webp60\endcsname{0.849}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/rob/webp80\endcsname{0.868}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ssim\endcsname{0.9985}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ssim/hi\endcsname{0.9988}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/ssim/lo\endcsname{0.9982}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/worst\endcsname{0.869}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.1/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/comb\endcsname{0.79}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/combq\endcsname{0.62}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/cost\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/costcpu\endcsname{0.026}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/costgpu\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/cpu\endcsname{544}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/cvvdp\endcsname{9.39}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/cvvdp/hi\endcsname{9.44}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/cvvdp/lo\endcsname{9.34}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/exact_gate\endcsname{0.906}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/flip\endcsname{0.058}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/flip/hi\endcsname{0.061}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/flip/lo\endcsname{0.054}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/gpu\endcsname{8.79}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/lpips\endcsname{0.0082}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/lpips/hi\endcsname{0.0094}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/lpips/lo\endcsname{0.0072}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ms_ssim\endcsname{0.9882}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ms_ssim/hi\endcsname{0.9891}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ms_ssim/lo\endcsname{0.9873}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/psnr\endcsname{38.9}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/psnr/hi\endcsname{39.4}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/psnr/lo\endcsname{38.5}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/bright1.2\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/crop50\endcsname{0.511}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/crop70\endcsname{0.903}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/crop90\endcsname{0.997}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/jpeg60\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/jpeg90\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/webp60\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/rob/webp80\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ssim\endcsname{0.9856}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ssim/hi\endcsname{0.9878}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/ssim/lo\endcsname{0.9831}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@0.4/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/comb\endcsname{0.90}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/combq\endcsname{0.80}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/cost\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/costcpu\endcsname{0.026}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/costgpu\endcsname{0.0025}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/cpu\endcsname{544}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/cvvdp\endcsname{9.82}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/cvvdp/hi\endcsname{9.84}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/cvvdp/lo\endcsname{9.80}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/exact_gate\endcsname{0.659}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/flip\endcsname{0.034}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/flip/hi\endcsname{0.036}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/flip/lo\endcsname{0.032}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/gate\endcsname{0.997}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/gpu\endcsname{8.79}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/lpips\endcsname{0.0021}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/lpips/hi\endcsname{0.0024}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/lpips/lo\endcsname{0.0019}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ms_ssim\endcsname{0.9969}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ms_ssim/hi\endcsname{0.9971}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ms_ssim/lo\endcsname{0.9966}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/psnr\endcsname{44.8}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/psnr/hi\endcsname{45.3}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/psnr/lo\endcsname{44.4}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/blur1\endcsname{0.998}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/bright0.8\endcsname{0.998}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/bright1.2\endcsname{0.995}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/crop50\endcsname{0.503}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/crop70\endcsname{0.806}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/crop90\endcsname{0.988}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/jpeg50\endcsname{0.993}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/jpeg60\endcsname{0.994}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/jpeg75\endcsname{0.997}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/jpeg90\endcsname{0.997}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/none\endcsname{0.998}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/resize0.5\endcsname{0.998}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/resize0.75\endcsname{0.998}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/webp60\endcsname{0.988}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/rob/webp80\endcsname{0.994}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ssim\endcsname{0.9953}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ssim/hi\endcsname{0.9962}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/ssim/lo\endcsname{0.9944}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/worst\endcsname{0.996}
\expandafter\def\csname val@wm:image/VideoSeal-1.0@default/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/WAM-MIT@1/comb\endcsname{0.57}
\expandafter\def\csname val@wm:image/WAM-MIT@1/combq\endcsname{0.56}
\expandafter\def\csname val@wm:image/WAM-MIT@1/cost\endcsname{0.0053}
\expandafter\def\csname val@wm:image/WAM-MIT@1/costcpu\endcsname{0.017}
\expandafter\def\csname val@wm:image/WAM-MIT@1/costgpu\endcsname{0.0053}
\expandafter\def\csname val@wm:image/WAM-MIT@1/cpu\endcsname{361}
\expandafter\def\csname val@wm:image/WAM-MIT@1/cvvdp\endcsname{9.97}
\expandafter\def\csname val@wm:image/WAM-MIT@1/cvvdp/hi\endcsname{9.98}
\expandafter\def\csname val@wm:image/WAM-MIT@1/cvvdp/lo\endcsname{9.97}
\expandafter\def\csname val@wm:image/WAM-MIT@1/exact_gate\endcsname{0.918}
\expandafter\def\csname val@wm:image/WAM-MIT@1/flip\endcsname{0.043}
\expandafter\def\csname val@wm:image/WAM-MIT@1/flip/hi\endcsname{0.046}
\expandafter\def\csname val@wm:image/WAM-MIT@1/flip/lo\endcsname{0.041}
\expandafter\def\csname val@wm:image/WAM-MIT@1/gate\endcsname{0.994}
\expandafter\def\csname val@wm:image/WAM-MIT@1/gpu\endcsname{19.1}
\expandafter\def\csname val@wm:image/WAM-MIT@1/keymatch_gate\endcsname{0.976}
\expandafter\def\csname val@wm:image/WAM-MIT@1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/WAM-MIT@1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/WAM-MIT@1/lpips\endcsname{0.0099}
\expandafter\def\csname val@wm:image/WAM-MIT@1/lpips/hi\endcsname{0.0113}
\expandafter\def\csname val@wm:image/WAM-MIT@1/lpips/lo\endcsname{0.0087}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ms_ssim\endcsname{0.9967}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ms_ssim/hi\endcsname{0.9971}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ms_ssim/lo\endcsname{0.9963}
\expandafter\def\csname val@wm:image/WAM-MIT@1/psnr\endcsname{45.3}
\expandafter\def\csname val@wm:image/WAM-MIT@1/psnr/hi\endcsname{45.7}
\expandafter\def\csname val@wm:image/WAM-MIT@1/psnr/lo\endcsname{44.9}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/blur1\endcsname{0.997}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/bright0.8\endcsname{0.990}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/bright1.2\endcsname{0.998}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/crop50\endcsname{0.616}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/crop70\endcsname{0.942}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/crop90\endcsname{0.968}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/jpeg50\endcsname{0.976}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/jpeg60\endcsname{0.981}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/jpeg75\endcsname{0.994}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/jpeg90\endcsname{0.997}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/none\endcsname{0.997}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/resize0.5\endcsname{0.997}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/resize0.75\endcsname{0.997}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/webp60\endcsname{0.976}
\expandafter\def\csname val@wm:image/WAM-MIT@1/rob/webp80\endcsname{0.987}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ssim\endcsname{0.9948}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ssim/hi\endcsname{0.9961}
\expandafter\def\csname val@wm:image/WAM-MIT@1/ssim/lo\endcsname{0.9932}
\expandafter\def\csname val@wm:image/WAM-MIT@1/worst\endcsname{0.990}
\expandafter\def\csname val@wm:image/WAM-MIT@1/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/WAM-MIT@default/comb\endcsname{0.51}
\expandafter\def\csname val@wm:image/WAM-MIT@default/combq\endcsname{0.44}
\expandafter\def\csname val@wm:image/WAM-MIT@default/cost\endcsname{0.0053}
\expandafter\def\csname val@wm:image/WAM-MIT@default/costcpu\endcsname{0.017}
\expandafter\def\csname val@wm:image/WAM-MIT@default/costgpu\endcsname{0.0053}
\expandafter\def\csname val@wm:image/WAM-MIT@default/cpu\endcsname{361}
\expandafter\def\csname val@wm:image/WAM-MIT@default/cvvdp\endcsname{9.88}
\expandafter\def\csname val@wm:image/WAM-MIT@default/cvvdp/hi\endcsname{9.90}
\expandafter\def\csname val@wm:image/WAM-MIT@default/cvvdp/lo\endcsname{9.85}
\expandafter\def\csname val@wm:image/WAM-MIT@default/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/flip\endcsname{0.071}
\expandafter\def\csname val@wm:image/WAM-MIT@default/flip/hi\endcsname{0.074}
\expandafter\def\csname val@wm:image/WAM-MIT@default/flip/lo\endcsname{0.067}
\expandafter\def\csname val@wm:image/WAM-MIT@default/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/gpu\endcsname{19.1}
\expandafter\def\csname val@wm:image/WAM-MIT@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/WAM-MIT@default/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/WAM-MIT@default/lpips\endcsname{0.0367}
\expandafter\def\csname val@wm:image/WAM-MIT@default/lpips/hi\endcsname{0.0408}
\expandafter\def\csname val@wm:image/WAM-MIT@default/lpips/lo\endcsname{0.0326}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ms_ssim\endcsname{0.9880}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ms_ssim/hi\endcsname{0.9894}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ms_ssim/lo\endcsname{0.9865}
\expandafter\def\csname val@wm:image/WAM-MIT@default/psnr\endcsname{39.4}
\expandafter\def\csname val@wm:image/WAM-MIT@default/psnr/hi\endcsname{39.8}
\expandafter\def\csname val@wm:image/WAM-MIT@default/psnr/lo\endcsname{39.1}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/bright1.2\endcsname{0.999}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/crop50\endcsname{0.964}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/crop70\endcsname{0.995}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/crop90\endcsname{0.993}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/jpeg50\endcsname{0.998}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/jpeg60\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/webp60\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ssim\endcsname{0.9852}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ssim/hi\endcsname{0.9881}
\expandafter\def\csname val@wm:image/WAM-MIT@default/ssim/lo\endcsname{0.9818}
\expandafter\def\csname val@wm:image/WAM-MIT@default/worst\endcsname{1.000}
\expandafter\def\csname val@wm:image/WAM-MIT@default/worstset\endcsname{clic}
\expandafter\def\csname val@wm:image/n_configs\endcsname{25}
\expandafter\def\csname val@wm:image/n_items\endcsname{85}
\expandafter\def\csname val@wm:image/n_qualify\endcsname{18}
\expandafter\def\csname val@wm:image/trustmark-B@1/blind\endcsname{0.0382}
\expandafter\def\csname val@wm:image/trustmark-B@1/blindhi\endcsname{0.0645}
\expandafter\def\csname val@wm:image/trustmark-B@1/blindpct\endcsname{3.8}
\expandafter\def\csname val@wm:image/trustmark-B@1/comb\endcsname{0.35}
\expandafter\def\csname val@wm:image/trustmark-B@1/combq\endcsname{0.42}
\expandafter\def\csname val@wm:image/trustmark-B@1/cost\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-B@1/costcpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-B@1/costgpu\endcsname{0.016}
\expandafter\def\csname val@wm:image/trustmark-B@1/cpu\endcsname{278}
\expandafter\def\csname val@wm:image/trustmark-B@1/cvvdp\endcsname{9.45}
\expandafter\def\csname val@wm:image/trustmark-B@1/cvvdp/hi\endcsname{9.49}
\expandafter\def\csname val@wm:image/trustmark-B@1/cvvdp/lo\endcsname{9.41}
\expandafter\def\csname val@wm:image/trustmark-B@1/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/flip\endcsname{0.043}
\expandafter\def\csname val@wm:image/trustmark-B@1/flip/hi\endcsname{0.044}
\expandafter\def\csname val@wm:image/trustmark-B@1/flip/lo\endcsname{0.041}
\expandafter\def\csname val@wm:image/trustmark-B@1/gate\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/gpu\endcsname{55.7}
\expandafter\def\csname val@wm:image/trustmark-B@1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-B@1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-B@1/lpips\endcsname{0.0029}
\expandafter\def\csname val@wm:image/trustmark-B@1/lpips/hi\endcsname{0.0032}
\expandafter\def\csname val@wm:image/trustmark-B@1/lpips/lo\endcsname{0.0026}
\expandafter\def\csname val@wm:image/trustmark-B@1/ms_ssim\endcsname{0.9919}
\expandafter\def\csname val@wm:image/trustmark-B@1/ms_ssim/hi\endcsname{0.9923}
\expandafter\def\csname val@wm:image/trustmark-B@1/ms_ssim/lo\endcsname{0.9916}
\expandafter\def\csname val@wm:image/trustmark-B@1/psnr\endcsname{41.0}
\expandafter\def\csname val@wm:image/trustmark-B@1/psnr/hi\endcsname{41.4}
\expandafter\def\csname val@wm:image/trustmark-B@1/psnr/lo\endcsname{40.6}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/bright0.8\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/bright1.2\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/crop50\endcsname{0.490}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/crop70\endcsname{0.551}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/jpeg60\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/jpeg75\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/jpeg90\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/webp60\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-B@1/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-B@1/ssim\endcsname{0.9940}
\expandafter\def\csname val@wm:image/trustmark-B@1/ssim/hi\endcsname{0.9950}
\expandafter\def\csname val@wm:image/trustmark-B@1/ssim/lo\endcsname{0.9929}
\expandafter\def\csname val@wm:image/trustmark-B@1/worst\endcsname{0.997}
\expandafter\def\csname val@wm:image/trustmark-B@1/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/trustmark-C@1/blind\endcsname{0.0441}
\expandafter\def\csname val@wm:image/trustmark-C@1/blindhi\endcsname{0.0717}
\expandafter\def\csname val@wm:image/trustmark-C@1/blindpct\endcsname{4.4}
\expandafter\def\csname val@wm:image/trustmark-C@1/comb\endcsname{0.34}
\expandafter\def\csname val@wm:image/trustmark-C@1/combq\endcsname{0.40}
\expandafter\def\csname val@wm:image/trustmark-C@1/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-C@1/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-C@1/costgpu\endcsname{0.015}
\expandafter\def\csname val@wm:image/trustmark-C@1/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-C@1/cvvdp\endcsname{9.38}
\expandafter\def\csname val@wm:image/trustmark-C@1/cvvdp/hi\endcsname{9.43}
\expandafter\def\csname val@wm:image/trustmark-C@1/cvvdp/lo\endcsname{9.34}
\expandafter\def\csname val@wm:image/trustmark-C@1/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-C@1/flip\endcsname{0.047}
\expandafter\def\csname val@wm:image/trustmark-C@1/flip/hi\endcsname{0.048}
\expandafter\def\csname val@wm:image/trustmark-C@1/flip/lo\endcsname{0.045}
\expandafter\def\csname val@wm:image/trustmark-C@1/gate\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-C@1/gpu\endcsname{54.4}
\expandafter\def\csname val@wm:image/trustmark-C@1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-C@1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-C@1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-C@1/lpips\endcsname{0.0035}
\expandafter\def\csname val@wm:image/trustmark-C@1/lpips/hi\endcsname{0.0038}
\expandafter\def\csname val@wm:image/trustmark-C@1/lpips/lo\endcsname{0.0032}
\expandafter\def\csname val@wm:image/trustmark-C@1/ms_ssim\endcsname{0.9902}
\expandafter\def\csname val@wm:image/trustmark-C@1/ms_ssim/hi\endcsname{0.9906}
\expandafter\def\csname val@wm:image/trustmark-C@1/ms_ssim/lo\endcsname{0.9897}
\expandafter\def\csname val@wm:image/trustmark-C@1/psnr\endcsname{40.0}
\expandafter\def\csname val@wm:image/trustmark-C@1/psnr/hi\endcsname{40.5}
\expandafter\def\csname val@wm:image/trustmark-C@1/psnr/lo\endcsname{39.6}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/blur1\endcsname{0.997}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/bright0.8\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/bright1.2\endcsname{0.986}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/crop50\endcsname{0.495}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/crop70\endcsname{0.665}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/crop90\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/jpeg50\endcsname{0.994}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/jpeg60\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/jpeg75\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/jpeg90\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/none\endcsname{0.997}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/resize0.5\endcsname{0.997}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/resize0.75\endcsname{0.997}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/webp60\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-C@1/rob/webp80\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-C@1/ssim\endcsname{0.9926}
\expandafter\def\csname val@wm:image/trustmark-C@1/ssim/hi\endcsname{0.9937}
\expandafter\def\csname val@wm:image/trustmark-C@1/ssim/lo\endcsname{0.9913}
\expandafter\def\csname val@wm:image/trustmark-C@1/worst\endcsname{0.992}
\expandafter\def\csname val@wm:image/trustmark-C@1/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/blind\endcsname{0.0206}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/blindhi\endcsname{0.0420}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/blindpct\endcsname{2.1}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/comb\endcsname{0.43}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/combq\endcsname{0.60}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/cost\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/costcpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/costgpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/cpu\endcsname{273}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/cvvdp\endcsname{9.98}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/cvvdp/hi\endcsname{9.98}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/cvvdp/lo\endcsname{9.98}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/exact_gate\endcsname{0.847}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/flip\endcsname{0.022}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/flip/hi\endcsname{0.023}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/flip/lo\endcsname{0.021}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/gate\endcsname{0.977}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/gpu\endcsname{45.1}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/lpips\endcsname{0.0017}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/lpips/hi\endcsname{0.0020}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/lpips/lo\endcsname{0.0014}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ms_ssim\endcsname{0.9992}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ms_ssim/hi\endcsname{0.9993}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ms_ssim/lo\endcsname{0.9992}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/psnr\endcsname{50.5}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/psnr/hi\endcsname{50.8}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/psnr/lo\endcsname{50.3}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/blur1\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/bright0.8\endcsname{0.993}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/bright1.2\endcsname{0.966}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/crop50\endcsname{0.498}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/crop70\endcsname{0.577}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/crop90\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/jpeg50\endcsname{0.923}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/jpeg60\endcsname{0.938}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/jpeg75\endcsname{0.977}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/jpeg90\endcsname{0.994}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/none\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/resize0.5\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/resize0.75\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/webp60\endcsname{0.958}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/rob/webp80\endcsname{0.981}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ssim\endcsname{0.9985}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ssim/hi\endcsname{0.9988}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/ssim/lo\endcsname{0.9982}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/worst\endcsname{0.952}
\expandafter\def\csname val@wm:image/trustmark-P@0.8/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/blind\endcsname{0.0206}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/blindhi\endcsname{0.0420}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/blindpct\endcsname{2.1}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/comb\endcsname{0.41}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/combq\endcsname{0.53}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/cost\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/costcpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/costgpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/cpu\endcsname{273}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/cvvdp\endcsname{9.93}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/cvvdp/hi\endcsname{9.94}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/cvvdp/lo\endcsname{9.91}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/flip\endcsname{0.029}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/flip/hi\endcsname{0.030}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/flip/lo\endcsname{0.028}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/gate\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/gpu\endcsname{45.1}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/lpips\endcsname{0.0049}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/lpips/hi\endcsname{0.0057}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/lpips/lo\endcsname{0.0042}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ms_ssim\endcsname{0.9978}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ms_ssim/hi\endcsname{0.9980}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ms_ssim/lo\endcsname{0.9977}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/psnr\endcsname{46.8}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/psnr/hi\endcsname{47.2}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/psnr/lo\endcsname{46.5}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/blur1\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/bright0.8\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/bright1.2\endcsname{0.982}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/crop50\endcsname{0.501}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/crop70\endcsname{0.639}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/jpeg50\endcsname{0.985}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/jpeg60\endcsname{0.993}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/jpeg75\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/jpeg90\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/none\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/resize0.5\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/resize0.75\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/webp60\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/rob/webp80\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ssim\endcsname{0.9964}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ssim/hi\endcsname{0.9971}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/ssim/lo\endcsname{0.9956}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/worst\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-P@1.5/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/trustmark-P@1/blind\endcsname{0.0206}
\expandafter\def\csname val@wm:image/trustmark-P@1/blindhi\endcsname{0.0420}
\expandafter\def\csname val@wm:image/trustmark-P@1/blindpct\endcsname{2.1}
\expandafter\def\csname val@wm:image/trustmark-P@1/comb\endcsname{0.43}
\expandafter\def\csname val@wm:image/trustmark-P@1/combq\endcsname{0.58}
\expandafter\def\csname val@wm:image/trustmark-P@1/cost\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1/costcpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1/costgpu\endcsname{0.013}
\expandafter\def\csname val@wm:image/trustmark-P@1/cpu\endcsname{273}
\expandafter\def\csname val@wm:image/trustmark-P@1/cvvdp\endcsname{9.97}
\expandafter\def\csname val@wm:image/trustmark-P@1/cvvdp/hi\endcsname{9.97}
\expandafter\def\csname val@wm:image/trustmark-P@1/cvvdp/lo\endcsname{9.96}
\expandafter\def\csname val@wm:image/trustmark-P@1/exact_gate\endcsname{0.976}
\expandafter\def\csname val@wm:image/trustmark-P@1/flip\endcsname{0.024}
\expandafter\def\csname val@wm:image/trustmark-P@1/flip/hi\endcsname{0.025}
\expandafter\def\csname val@wm:image/trustmark-P@1/flip/lo\endcsname{0.023}
\expandafter\def\csname val@wm:image/trustmark-P@1/gate\endcsname{0.990}
\expandafter\def\csname val@wm:image/trustmark-P@1/gpu\endcsname{45.1}
\expandafter\def\csname val@wm:image/trustmark-P@1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-P@1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-P@1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-P@1/lpips\endcsname{0.0024}
\expandafter\def\csname val@wm:image/trustmark-P@1/lpips/hi\endcsname{0.0028}
\expandafter\def\csname val@wm:image/trustmark-P@1/lpips/lo\endcsname{0.0020}
\expandafter\def\csname val@wm:image/trustmark-P@1/ms_ssim\endcsname{0.9989}
\expandafter\def\csname val@wm:image/trustmark-P@1/ms_ssim/hi\endcsname{0.9990}
\expandafter\def\csname val@wm:image/trustmark-P@1/ms_ssim/lo\endcsname{0.9988}
\expandafter\def\csname val@wm:image/trustmark-P@1/psnr\endcsname{49.4}
\expandafter\def\csname val@wm:image/trustmark-P@1/psnr/hi\endcsname{49.7}
\expandafter\def\csname val@wm:image/trustmark-P@1/psnr/lo\endcsname{49.1}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/blur1\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/bright0.8\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/bright1.2\endcsname{0.976}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/crop50\endcsname{0.498}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/crop70\endcsname{0.601}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/crop90\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/jpeg50\endcsname{0.955}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/jpeg60\endcsname{0.967}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/jpeg75\endcsname{0.990}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/jpeg90\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/none\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/resize0.5\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/resize0.75\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/webp60\endcsname{0.982}
\expandafter\def\csname val@wm:image/trustmark-P@1/rob/webp80\endcsname{0.992}
\expandafter\def\csname val@wm:image/trustmark-P@1/ssim\endcsname{0.9980}
\expandafter\def\csname val@wm:image/trustmark-P@1/ssim/hi\endcsname{0.9984}
\expandafter\def\csname val@wm:image/trustmark-P@1/ssim/lo\endcsname{0.9976}
\expandafter\def\csname val@wm:image/trustmark-P@1/worst\endcsname{0.977}
\expandafter\def\csname val@wm:image/trustmark-P@1/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/blind\endcsname{0.0265}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/blindhi\endcsname{0.0497}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/blindpct\endcsname{2.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/comb\endcsname{0.33}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/combq\endcsname{0.40}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/costgpu\endcsname{0.018}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/cvvdp\endcsname{9.33}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/cvvdp/hi\endcsname{9.38}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/cvvdp/lo\endcsname{9.28}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/flip\endcsname{0.045}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/flip/hi\endcsname{0.046}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/flip/lo\endcsname{0.043}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/gpu\endcsname{63.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/lpips\endcsname{0.0037}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/lpips/hi\endcsname{0.0040}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/lpips/lo\endcsname{0.0034}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ms_ssim\endcsname{0.9899}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ms_ssim/hi\endcsname{0.9904}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ms_ssim/lo\endcsname{0.9893}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/psnr\endcsname{40.7}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/psnr/hi\endcsname{41.1}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/psnr/lo\endcsname{40.3}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/bright1.2\endcsname{0.995}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/crop50\endcsname{0.510}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/crop70\endcsname{0.598}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/jpeg60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/webp60\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ssim\endcsname{0.9925}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ssim/hi\endcsname{0.9936}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/ssim/lo\endcsname{0.9912}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/worst\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.2/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/blind\endcsname{0.0265}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/blindhi\endcsname{0.0497}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/blindpct\endcsname{2.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/comb\endcsname{0.33}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/combq\endcsname{0.39}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/costgpu\endcsname{0.018}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/cvvdp\endcsname{9.25}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/cvvdp/hi\endcsname{9.31}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/cvvdp/lo\endcsname{9.20}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/flip\endcsname{0.047}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/flip/hi\endcsname{0.049}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/flip/lo\endcsname{0.045}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/gpu\endcsname{63.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/lpips\endcsname{0.0043}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/lpips/hi\endcsname{0.0046}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/lpips/lo\endcsname{0.0039}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ms_ssim\endcsname{0.9883}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ms_ssim/hi\endcsname{0.9889}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ms_ssim/lo\endcsname{0.9876}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/psnr\endcsname{40.0}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/psnr/hi\endcsname{40.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/psnr/lo\endcsname{39.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/bright1.2\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/crop50\endcsname{0.510}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/crop70\endcsname{0.613}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/jpeg60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/webp60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ssim\endcsname{0.9914}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ssim/hi\endcsname{0.9927}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/ssim/lo\endcsname{0.9901}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.3/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/blind\endcsname{0.0265}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/blindhi\endcsname{0.0497}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/blindpct\endcsname{2.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/comb\endcsname{0.32}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/combq\endcsname{0.38}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/costgpu\endcsname{0.018}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/cvvdp\endcsname{9.18}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/cvvdp/hi\endcsname{9.24}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/cvvdp/lo\endcsname{9.12}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/flip\endcsname{0.049}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/flip/hi\endcsname{0.051}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/flip/lo\endcsname{0.048}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/gpu\endcsname{63.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/lpips\endcsname{0.0049}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/lpips/hi\endcsname{0.0053}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/lpips/lo\endcsname{0.0045}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ms_ssim\endcsname{0.9866}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ms_ssim/hi\endcsname{0.9873}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ms_ssim/lo\endcsname{0.9859}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/psnr\endcsname{39.4}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/psnr/hi\endcsname{39.9}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/psnr/lo\endcsname{39.0}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/bright1.2\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/crop50\endcsname{0.509}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/crop70\endcsname{0.623}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/jpeg60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/webp60\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ssim\endcsname{0.9904}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ssim/hi\endcsname{0.9918}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/ssim/lo\endcsname{0.9889}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.4/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/blind\endcsname{0.0265}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/blindhi\endcsname{0.0497}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/blindpct\endcsname{2.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/comb\endcsname{0.32}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/combq\endcsname{0.38}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/costgpu\endcsname{0.018}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/cvvdp\endcsname{9.11}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/cvvdp/hi\endcsname{9.17}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/cvvdp/lo\endcsname{9.04}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/flip\endcsname{0.052}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/flip/hi\endcsname{0.054}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/flip/lo\endcsname{0.050}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/gpu\endcsname{63.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/lpips\endcsname{0.0056}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/lpips/hi\endcsname{0.0061}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/lpips/lo\endcsname{0.0052}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ms_ssim\endcsname{0.9848}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ms_ssim/hi\endcsname{0.9856}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ms_ssim/lo\endcsname{0.9840}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/psnr\endcsname{38.9}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/psnr/hi\endcsname{39.3}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/psnr/lo\endcsname{38.4}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/bright0.8\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/bright1.2\endcsname{0.996}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/crop50\endcsname{0.505}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/crop70\endcsname{0.626}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/jpeg50\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/jpeg60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/jpeg75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/webp60\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ssim\endcsname{0.9893}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ssim/hi\endcsname{0.9908}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/ssim/lo\endcsname{0.9876}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1.5/worstset\endcsname{div2k}
\expandafter\def\csname val@wm:image/trustmark-Q@1/blind\endcsname{0.0265}
\expandafter\def\csname val@wm:image/trustmark-Q@1/blindhi\endcsname{0.0497}
\expandafter\def\csname val@wm:image/trustmark-Q@1/blindpct\endcsname{2.6}
\expandafter\def\csname val@wm:image/trustmark-Q@1/comb\endcsname{0.34}
\expandafter\def\csname val@wm:image/trustmark-Q@1/combq\endcsname{0.43}
\expandafter\def\csname val@wm:image/trustmark-Q@1/cost\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1/costcpu\endcsname{0.014}
\expandafter\def\csname val@wm:image/trustmark-Q@1/costgpu\endcsname{0.018}
\expandafter\def\csname val@wm:image/trustmark-Q@1/cpu\endcsname{283}
\expandafter\def\csname val@wm:image/trustmark-Q@1/cvvdp\endcsname{9.48}
\expandafter\def\csname val@wm:image/trustmark-Q@1/cvvdp/hi\endcsname{9.52}
\expandafter\def\csname val@wm:image/trustmark-Q@1/cvvdp/lo\endcsname{9.44}
\expandafter\def\csname val@wm:image/trustmark-Q@1/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/flip\endcsname{0.040}
\expandafter\def\csname val@wm:image/trustmark-Q@1/flip/hi\endcsname{0.041}
\expandafter\def\csname val@wm:image/trustmark-Q@1/flip/lo\endcsname{0.039}
\expandafter\def\csname val@wm:image/trustmark-Q@1/gate\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1/gpu\endcsname{63.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:image/trustmark-Q@1/keyupper\endcsname{0.00017}
\expandafter\def\csname val@wm:image/trustmark-Q@1/lpips\endcsname{0.0027}
\expandafter\def\csname val@wm:image/trustmark-Q@1/lpips/hi\endcsname{0.0029}
\expandafter\def\csname val@wm:image/trustmark-Q@1/lpips/lo\endcsname{0.0024}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ms_ssim\endcsname{0.9928}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ms_ssim/hi\endcsname{0.9932}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ms_ssim/lo\endcsname{0.9924}
\expandafter\def\csname val@wm:image/trustmark-Q@1/psnr\endcsname{42.1}
\expandafter\def\csname val@wm:image/trustmark-Q@1/psnr/hi\endcsname{42.5}
\expandafter\def\csname val@wm:image/trustmark-Q@1/psnr/lo\endcsname{41.7}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/blur1\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/bright0.8\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/bright1.2\endcsname{0.992}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/crop50\endcsname{0.504}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/crop70\endcsname{0.570}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/crop90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/jpeg50\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/jpeg60\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/jpeg75\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/jpeg90\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/none\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/resize0.5\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/resize0.75\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/webp60\endcsname{0.998}
\expandafter\def\csname val@wm:image/trustmark-Q@1/rob/webp80\endcsname{1.000}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ssim\endcsname{0.9943}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ssim/hi\endcsname{0.9952}
\expandafter\def\csname val@wm:image/trustmark-Q@1/ssim/lo\endcsname{0.9934}
\expandafter\def\csname val@wm:image/trustmark-Q@1/worst\endcsname{0.999}
\expandafter\def\csname val@wm:image/trustmark-Q@1/worstset\endcsname{kodak}
\expandafter\def\csname val@wm:image/win/combined\endcsname{PixelSeal (0.15)}
\expandafter\def\csname val@wm:image/win/combined_q\endcsname{PixelSeal (0.15)}
\expandafter\def\csname val@wm:image/win/cost\endcsname{Video Seal (0.2)}
\expandafter\def\csname val@wm:image/win/speed\endcsname{Video Seal (0.2)}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/aac_64/aligned\endcsname{0.998}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/aac_64/unaligned\endcsname{0.999}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/all/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/all/exact_aligned\endcsname{0.978}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/all/exact_unaligned\endcsname{0.986}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/all/unaligned\endcsname{0.999}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/mp3_128/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/mp3_128/unaligned\endcsname{0.999}
\expandafter\def\csname val@wm:noalign/AudioSeal-base@1/n\endcsname{138}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/aac_64/aligned\endcsname{0.995}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/aac_64/unaligned\endcsname{0.998}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/all/aligned\endcsname{0.996}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/all/exact_aligned\endcsname{0.983}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/all/exact_unaligned\endcsname{0.990}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/all/unaligned\endcsname{0.999}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/mp3_128/aligned\endcsname{0.996}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/mp3_128/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@0.5/n\endcsname{138}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/aac_64/aligned\endcsname{0.996}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/aac_64/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/all/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/all/exact_aligned\endcsname{0.993}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/all/exact_unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/all/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/mp3_128/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/mp3_128/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1.1/n\endcsname{138}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/aac_64/aligned\endcsname{0.995}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/aac_64/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/all/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/all/exact_aligned\endcsname{0.993}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/all/exact_unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/all/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/mp3_128/aligned\endcsname{0.997}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/mp3_128/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/AudioSeal-streaming@1/n\endcsname{138}
\expandafter\def\csname val@wm:noalign/WavMark/aac_64/aligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/aac_64/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/all/aligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/all/exact_aligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/all/exact_unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/all/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/mp3_128/aligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/mp3_128/unaligned\endcsname{1.000}
\expandafter\def\csname val@wm:noalign/WavMark/n\endcsname{138}
\expandafter\def\csname val@wm:noalign/host\endcsname{Apple M5 Pro}
\expandafter\def\csname val@wm:price/cpu\endcsname{0.1728}
\expandafter\def\csname val@wm:price/date\endcsname{2026-09-01}
\expandafter\def\csname val@wm:price/gpu\endcsname{1.006}
\expandafter\def\csname val@wm:ps/flip\endcsname{0.024}
\expandafter\def\csname val@wm:ps/lpips\endcsname{0.0012}
\expandafter\def\csname val@wm:ratio/ps_tq/flip\endcsname{0.59}
\expandafter\def\csname val@wm:ratio/ps_tq/gpu\endcsname{6.9}
\expandafter\def\csname val@wm:ratio/ps_tq/lpips\endcsname{2.2}
\expandafter\def\csname val@wm:rgb/av\endcsname{18.1.0}
\expandafter\def\csname val@wm:rgb/backend_dlogit\endcsname{0.002}
\expandafter\def\csname val@wm:rgb/conv_dlogit\endcsname{0.92}
\expandafter\def\csname val@wm:rgb/flippairs\endcsname{8}
\expandafter\def\csname val@wm:rgb/maxflips\endcsname{2}
\expandafter\def\csname val@wm:rgb/model_dlogit\endcsname{$3\times10^{-5}$}
\expandafter\def\csname val@wm:rgb/nclips\endcsname{12}
\expandafter\def\csname val@wm:rgb/nframes\endcsname{16}
\expandafter\def\csname val@wm:rgb/rgb_equal\endcsname{0}
\expandafter\def\csname val@wm:rgb/same_libs\endcsname{yes}
\expandafter\def\csname val@wm:rgb/swscale\endcsname{9.5.102}
\expandafter\def\csname val@wm:rgb/yuv_equal\endcsname{12}
\expandafter\def\csname val@wm:stab/files\endcsname{13}
\expandafter\def\csname val@wm:stab/maxcross\endcsname{0.89}
\expandafter\def\csname val@wm:stab/maxflips\endcsname{2}
\expandafter\def\csname val@wm:stab/maxsame\endcsname{0.002}
\expandafter\def\csname val@wm:stab/nflipfiles\endcsname{2}
\expandafter\def\csname val@wm:stab/tm/cpu_dlogit\endcsname{$5\times10^{-5}$}
\expandafter\def\csname val@wm:stab/tm/flips\endcsname{0}
\expandafter\def\csname val@wm:stab/tm/maxcross\endcsname{0.070}
\expandafter\def\csname val@wm:stab/tm/maxsame\endcsname{0.070}
\expandafter\def\csname val@wm:stab/videofiles\endcsname{12}
\expandafter\def\csname val@wm:test/audio/AudioSeal-base@1/AudioSeal-streaming@0.5/pesq_speech/d\endcsname{-0.1072}
\expandafter\def\csname val@wm:test/audio/AudioSeal-base@1/AudioSeal-streaming@0.5/pesq_speech/n\endcsname{40}
\expandafter\def\csname val@wm:test/audio/AudioSeal-base@1/AudioSeal-streaming@0.5/pesq_speech/p\endcsname{$<$0.001}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/VideoSeal-1.0@default/flip/d\endcsname{-0.0099}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/VideoSeal-1.0@default/flip/n\endcsname{60}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/VideoSeal-1.0@default/flip/p\endcsname{$<$0.001}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-P@0.8/flip/d\endcsname{0.0019}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-P@0.8/flip/n\endcsname{60}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-P@0.8/flip/p\endcsname{0.062}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-Q@1.2/flip/d\endcsname{-0.0212}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-Q@1.2/flip/n\endcsname{60}
\expandafter\def\csname val@wm:test/image/PixelSeal@0.15/trustmark-Q@1.2/flip/p\endcsname{$<$0.001}
\expandafter\def\csname val@wm:test/video/PixelSeal@0.4/VideoSeal-1.0@0.4/vmaf/d\endcsname{3.6629}
\expandafter\def\csname val@wm:test/video/PixelSeal@0.4/VideoSeal-1.0@0.4/vmaf/n\endcsname{6}
\expandafter\def\csname val@wm:test/video/PixelSeal@0.4/VideoSeal-1.0@0.4/vmaf/p\endcsname{0.062}
\expandafter\def\csname val@wm:tm/blind/hdrk\endcsname{3}
\expandafter\def\csname val@wm:tm/blind/hdrmax\endcsname{37.5}
\expandafter\def\csname val@wm:tm/blind/hdrn\endcsname{8}
\expandafter\def\csname val@wm:tm/blind/max\endcsname{15.3}
\expandafter\def\csname val@wm:tm/blind/min\endcsname{5.9}
\expandafter\def\csname val@wm:tm/keytrials\endcsname{17{,}340}
\expandafter\def\csname val@wm:tq/flip\endcsname{0.040}
\expandafter\def\csname val@wm:tq/lpips\endcsname{0.0027}
\expandafter\def\csname val@wm:video/ChunkySeal@default/cost\endcsname{0.0066}
\expandafter\def\csname val@wm:video/ChunkySeal@default/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/ChunkySeal@default/costgpu\endcsname{0.0066}
\expandafter\def\csname val@wm:video/ChunkySeal@default/costhour\endcsname{1.48}
\expandafter\def\csname val@wm:video/ChunkySeal@default/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/ChunkySeal@default/embed_fps\endcsname{20.4}
\expandafter\def\csname val@wm:video/ChunkySeal@default/exact_gate\endcsname{0.000}
\expandafter\def\csname val@wm:video/ChunkySeal@default/flip\endcsname{0.048}
\expandafter\def\csname val@wm:video/ChunkySeal@default/flip/hi\endcsname{0.058}
\expandafter\def\csname val@wm:video/ChunkySeal@default/flip/lo\endcsname{0.039}
\expandafter\def\csname val@wm:video/ChunkySeal@default/fps\endcsname{20.4}
\expandafter\def\csname val@wm:video/ChunkySeal@default/gate\endcsname{0.891}
\expandafter\def\csname val@wm:video/ChunkySeal@default/gpu\endcsname{23.7}
\expandafter\def\csname val@wm:video/ChunkySeal@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/ChunkySeal@default/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/ChunkySeal@default/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/ChunkySeal@default/lpips\endcsname{0.0151}
\expandafter\def\csname val@wm:video/ChunkySeal@default/lpips/hi\endcsname{0.0270}
\expandafter\def\csname val@wm:video/ChunkySeal@default/lpips/lo\endcsname{0.0079}
\expandafter\def\csname val@wm:video/ChunkySeal@default/psnr\endcsname{44.5}
\expandafter\def\csname val@wm:video/ChunkySeal@default/psnr/hi\endcsname{45.6}
\expandafter\def\csname val@wm:video/ChunkySeal@default/psnr/lo\endcsname{43.3}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/crop75_h264_crf23\endcsname{0.535}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h264_crf18\endcsname{0.988}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h264_crf22\endcsname{0.925}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h264_crf23\endcsname{0.891}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h264_crf28\endcsname{0.763}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h265_crf23\endcsname{0.891}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/h265_crf28\endcsname{0.679}
\expandafter\def\csname val@wm:video/ChunkySeal@default/rob/resize0.5_h264_crf23\endcsname{0.790}
\expandafter\def\csname val@wm:video/ChunkySeal@default/ssim\endcsname{0.9734}
\expandafter\def\csname val@wm:video/ChunkySeal@default/ssim/hi\endcsname{0.9958}
\expandafter\def\csname val@wm:video/ChunkySeal@default/ssim/lo\endcsname{0.9293}
\expandafter\def\csname val@wm:video/ChunkySeal@default/vmaf\endcsname{96.4}
\expandafter\def\csname val@wm:video/ChunkySeal@default/vmaf/hi\endcsname{98.8}
\expandafter\def\csname val@wm:video/ChunkySeal@default/vmaf/lo\endcsname{94.1}
\expandafter\def\csname val@wm:video/ChunkySeal@default/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/ChunkySeal@default/worst\endcsname{0.652}
\expandafter\def\csname val@wm:video/ChunkySeal@default/worstset\endcsname{crowd\_run\_5s}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/comb\endcsname{1.00}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/combq\endcsname{1.00}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/cost\endcsname{0.0043}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/costgpu\endcsname{0.0043}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/costhour\endcsname{0.97}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/embed_fps\endcsname{31.7}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/exact_gate\endcsname{0.833}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/flip\endcsname{0.054}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/flip/hi\endcsname{0.066}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/flip/lo\endcsname{0.042}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/fps\endcsname{31.3}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/gate\endcsname{0.999}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/gpu\endcsname{15.4}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/lpips\endcsname{0.0130}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/lpips/hi\endcsname{0.0196}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/lpips/lo\endcsname{0.0079}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/psnr\endcsname{40.1}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/psnr/hi\endcsname{41.7}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/psnr/lo\endcsname{38.4}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/crop75_h264_crf23\endcsname{0.995}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h264_crf18\endcsname{0.998}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h264_crf22\endcsname{0.999}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h264_crf23\endcsname{0.999}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h264_crf28\endcsname{0.998}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h265_crf23\endcsname{0.999}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/h265_crf28\endcsname{0.998}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/rob/resize0.5_h264_crf23\endcsname{0.998}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/ssim\endcsname{0.9674}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/ssim/hi\endcsname{0.9913}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/ssim/lo\endcsname{0.9217}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/vmaf\endcsname{86.0}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/vmaf/hi\endcsname{91.7}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/vmaf/lo\endcsname{79.9}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/worst\endcsname{0.992}
\expandafter\def\csname val@wm:video/PixelSeal@0.4/worstset\endcsname{crowd\_run\_5s}
\expandafter\def\csname val@wm:video/PixelSeal@default/cost\endcsname{0.0043}
\expandafter\def\csname val@wm:video/PixelSeal@default/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/PixelSeal@default/costgpu\endcsname{0.0043}
\expandafter\def\csname val@wm:video/PixelSeal@default/costhour\endcsname{0.97}
\expandafter\def\csname val@wm:video/PixelSeal@default/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/PixelSeal@default/embed_fps\endcsname{30.9}
\expandafter\def\csname val@wm:video/PixelSeal@default/exact_gate\endcsname{0.667}
\expandafter\def\csname val@wm:video/PixelSeal@default/flip\endcsname{0.031}
\expandafter\def\csname val@wm:video/PixelSeal@default/flip/hi\endcsname{0.039}
\expandafter\def\csname val@wm:video/PixelSeal@default/flip/lo\endcsname{0.023}
\expandafter\def\csname val@wm:video/PixelSeal@default/fps\endcsname{31.3}
\expandafter\def\csname val@wm:video/PixelSeal@default/gate\endcsname{0.984}
\expandafter\def\csname val@wm:video/PixelSeal@default/gpu\endcsname{15.4}
\expandafter\def\csname val@wm:video/PixelSeal@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/PixelSeal@default/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/PixelSeal@default/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/PixelSeal@default/lpips\endcsname{0.0035}
\expandafter\def\csname val@wm:video/PixelSeal@default/lpips/hi\endcsname{0.0053}
\expandafter\def\csname val@wm:video/PixelSeal@default/lpips/lo\endcsname{0.0021}
\expandafter\def\csname val@wm:video/PixelSeal@default/psnr\endcsname{46.0}
\expandafter\def\csname val@wm:video/PixelSeal@default/psnr/hi\endcsname{47.5}
\expandafter\def\csname val@wm:video/PixelSeal@default/psnr/lo\endcsname{44.3}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/crop75_h264_crf23\endcsname{0.976}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h264_crf18\endcsname{0.988}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h264_crf22\endcsname{0.986}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h264_crf23\endcsname{0.984}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h264_crf28\endcsname{0.973}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h265_crf23\endcsname{0.984}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/h265_crf28\endcsname{0.969}
\expandafter\def\csname val@wm:video/PixelSeal@default/rob/resize0.5_h264_crf23\endcsname{0.978}
\expandafter\def\csname val@wm:video/PixelSeal@default/ssim\endcsname{0.9869}
\expandafter\def\csname val@wm:video/PixelSeal@default/ssim/hi\endcsname{0.9974}
\expandafter\def\csname val@wm:video/PixelSeal@default/ssim/lo\endcsname{0.9665}
\expandafter\def\csname val@wm:video/PixelSeal@default/vmaf\endcsname{95.5}
\expandafter\def\csname val@wm:video/PixelSeal@default/vmaf/hi\endcsname{97.9}
\expandafter\def\csname val@wm:video/PixelSeal@default/vmaf/lo\endcsname{92.7}
\expandafter\def\csname val@wm:video/PixelSeal@default/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/PixelSeal@default/worst\endcsname{0.949}
\expandafter\def\csname val@wm:video/PixelSeal@default/worstset\endcsname{crowd\_run\_5s}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/comb\endcsname{0.96}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/combq\endcsname{0.96}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/cost\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/costgpu\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/costhour\endcsname{1.02}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/embed_fps\endcsname{27.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/exact_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/flip\endcsname{0.055}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/flip/hi\endcsname{0.074}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/flip/lo\endcsname{0.034}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/fps\endcsname{29.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/gpu\endcsname{16.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/lpips\endcsname{0.0131}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/lpips/hi\endcsname{0.0210}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/lpips/lo\endcsname{0.0080}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/psnr\endcsname{40.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/psnr/hi\endcsname{43.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/psnr/lo\endcsname{37.5}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/crop75_h264_crf23\endcsname{0.968}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h264_crf18\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h264_crf22\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h264_crf23\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h264_crf28\endcsname{0.999}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h265_crf23\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/h265_crf28\endcsname{0.999}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/rob/resize0.5_h264_crf23\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/ssim\endcsname{0.9886}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/ssim/hi\endcsname{0.9920}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/ssim/lo\endcsname{0.9848}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/vmaf\endcsname{82.1}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/vmaf/hi\endcsname{88.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/vmaf/lo\endcsname{75.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/worst\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.4/worstset\endcsname{aspen\_5s}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/comb\endcsname{0.91}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/combq\endcsname{0.86}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/cost\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/costgpu\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/costhour\endcsname{1.02}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/embed_fps\endcsname{32.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/exact_gate\endcsname{0.500}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/flip\endcsname{0.083}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/flip/hi\endcsname{0.111}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/flip/lo\endcsname{0.052}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/fps\endcsname{29.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/gate\endcsname{0.997}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/gpu\endcsname{16.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/lpips\endcsname{0.0361}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/lpips/hi\endcsname{0.0508}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/lpips/lo\endcsname{0.0245}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/psnr\endcsname{35.5}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/psnr/hi\endcsname{38.5}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/psnr/lo\endcsname{32.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/crop75_h264_crf23\endcsname{0.938}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h264_crf18\endcsname{0.997}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h264_crf22\endcsname{0.997}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h264_crf23\endcsname{0.997}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h264_crf28\endcsname{0.992}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h265_crf23\endcsname{0.997}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/h265_crf28\endcsname{0.992}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/rob/resize0.5_h264_crf23\endcsname{0.993}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/ssim\endcsname{0.9710}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/ssim/hi\endcsname{0.9778}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/ssim/lo\endcsname{0.9638}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/vmaf\endcsname{66.6}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/vmaf/hi\endcsname{75.8}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/vmaf/lo\endcsname{57.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/worst\endcsname{0.992}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@0.7/worstset\endcsname{aspen\_5s}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/cost\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/costgpu\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/costhour\endcsname{1.02}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/embed_fps\endcsname{32.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/exact_gate\endcsname{0.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/flip\endcsname{0.116}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/flip/hi\endcsname{0.155}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/flip/lo\endcsname{0.074}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/fps\endcsname{29.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/gate\endcsname{0.954}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/gpu\endcsname{16.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/lpips\endcsname{0.0781}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/lpips/hi\endcsname{0.0977}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/lpips/lo\endcsname{0.0599}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/psnr\endcsname{31.6}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/psnr/hi\endcsname{34.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/psnr/lo\endcsname{28.8}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/crop75_h264_crf23\endcsname{0.788}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h264_crf18\endcsname{0.961}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h264_crf22\endcsname{0.958}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h264_crf23\endcsname{0.954}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h264_crf28\endcsname{0.941}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h265_crf23\endcsname{0.951}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/h265_crf28\endcsname{0.941}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/rob/resize0.5_h264_crf23\endcsname{0.951}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/ssim\endcsname{0.9403}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/ssim/hi\endcsname{0.9517}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/ssim/lo\endcsname{0.9281}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/vmaf\endcsname{54.6}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/vmaf/hi\endcsname{66.0}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/vmaf/lo\endcsname{45.1}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/worst\endcsname{0.902}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@1.1/worstset\endcsname{aspen\_5s}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/cost\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/costcpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/costgpu\endcsname{0.0045}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/costhour\endcsname{1.02}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/cpu\endcsname{--}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/embed_fps\endcsname{27.2}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/exact_gate\endcsname{0.667}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/flip\endcsname{0.032}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/flip/hi\endcsname{0.043}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/flip/lo\endcsname{0.019}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/fps\endcsname{29.7}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/gate\endcsname{0.986}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/gpu\endcsname{16.3}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/keymatch_gate\endcsname{1.000}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/keytrials\endcsname{1{,}206}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/keyupper\endcsname{0.0025}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/lpips\endcsname{0.0035}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/lpips/hi\endcsname{0.0057}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/lpips/lo\endcsname{0.0021}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/psnr\endcsname{46.2}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/psnr/hi\endcsname{49.2}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/psnr/lo\endcsname{43.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/crop75_h264_crf23\endcsname{0.898}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h264_crf18\endcsname{0.990}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h264_crf22\endcsname{0.986}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h264_crf23\endcsname{0.986}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h264_crf28\endcsname{0.985}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h265_crf23\endcsname{0.985}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/h265_crf28\endcsname{0.977}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/rob/resize0.5_h264_crf23\endcsname{0.975}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/ssim\endcsname{0.9964}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/ssim/hi\endcsname{0.9976}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/ssim/lo\endcsname{0.9949}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/vmaf\endcsname{94.0}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/vmaf/hi\endcsname{97.1}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/vmaf/lo\endcsname{91.0}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/vmaf_identical\endcsname{99.4}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/worst\endcsname{0.922}
\expandafter\def\csname val@wm:video/VideoSeal-1.0@default/worstset\endcsname{aspen\_5s}
\expandafter\def\csname val@wm:video/n_configs\endcsname{7}
\expandafter\def\csname val@wm:video/n_items\endcsname{6}
\expandafter\def\csname val@wm:video/n_qualify\endcsname{3}
\expandafter\def\csname val@wm:video/win/combined\endcsname{PixelSeal (0.4)}
\expandafter\def\csname val@wm:video/win/combined_q\endcsname{PixelSeal (0.4)}
\expandafter\def\csname val@wm:video/win/cost\endcsname{PixelSeal (0.4)}
\expandafter\def\csname val@wm:video/win/speed\endcsname{PixelSeal (0.4)}
\expandafter\def\csname val@fp:audio/CLAP/FPRq@query@0.01\endcsname{0.017}
\expandafter\def\csname val@fp:audio/CLAP/FPRq@query@0.01/pct\endcsname{1.7}
\expandafter\def\csname val@fp:audio/CLAP/R@1\endcsname{0.707}
\expandafter\def\csname val@fp:audio/CLAP/R@1/pct\endcsname{70.7}
\expandafter\def\csname val@fp:audio/CLAP/R@10\endcsname{0.800}
\expandafter\def\csname val@fp:audio/CLAP/R@10/pct\endcsname{80.0}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@0.0001\endcsname{0.569}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@0.0001/pct\endcsname{56.9}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@1e-05\endcsname{0.469}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@1e-05/pct\endcsname{46.9}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@1e-06\endcsname{0.328}
\expandafter\def\csname val@fp:audio/CLAP/TPR@pair@1e-06/pct\endcsname{32.8}
\expandafter\def\csname val@fp:audio/CLAP/TPR@query@0.01\endcsname{0.386}
\expandafter\def\csname val@fp:audio/CLAP/TPR@query@0.01/pct\endcsname{38.6}
\expandafter\def\csname val@fp:audio/CLAP/att/aac_64\endcsname{0.98}
\expandafter\def\csname val@fp:audio/CLAP/att/aac_64/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/CLAP/att/babble_0db\endcsname{0.12}
\expandafter\def\csname val@fp:audio/CLAP/att/babble_0db/pct\endcsname{12}
\expandafter\def\csname val@fp:audio/CLAP/att/babble_10db\endcsname{0.42}
\expandafter\def\csname val@fp:audio/CLAP/att/babble_10db/pct\endcsname{42}
\expandafter\def\csname val@fp:audio/CLAP/att/compressor\endcsname{0.98}
\expandafter\def\csname val@fp:audio/CLAP/att/compressor/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt10\endcsname{0.86}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt10/pct\endcsname{86}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt10_mp3_noise20\endcsname{0.41}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt10_mp3_noise20/pct\endcsname{41}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt5\endcsname{0.53}
\expandafter\def\csname val@fp:audio/CLAP/att/excerpt5/pct\endcsname{53}
\expandafter\def\csname val@fp:audio/CLAP/att/lowpass_2k\endcsname{0.88}
\expandafter\def\csname val@fp:audio/CLAP/att/lowpass_2k/pct\endcsname{88}
\expandafter\def\csname val@fp:audio/CLAP/att/mp3_64\endcsname{0.99}
\expandafter\def\csname val@fp:audio/CLAP/att/mp3_64/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/CLAP/att/noise_10db\endcsname{0.17}
\expandafter\def\csname val@fp:audio/CLAP/att/noise_10db/pct\endcsname{17}
\expandafter\def\csname val@fp:audio/CLAP/att/noise_20db\endcsname{0.49}
\expandafter\def\csname val@fp:audio/CLAP/att/noise_20db/pct\endcsname{49}
\expandafter\def\csname val@fp:audio/CLAP/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/att/opus_24\endcsname{0.96}
\expandafter\def\csname val@fp:audio/CLAP/att/opus_24/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/CLAP/att/phone\endcsname{0.85}
\expandafter\def\csname val@fp:audio/CLAP/att/phone/pct\endcsname{85}
\expandafter\def\csname val@fp:audio/CLAP/att/pitch+2\endcsname{0.91}
\expandafter\def\csname val@fp:audio/CLAP/att/pitch+2/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/CLAP/att/rerecord\endcsname{0.23}
\expandafter\def\csname val@fp:audio/CLAP/att/rerecord/pct\endcsname{23}
\expandafter\def\csname val@fp:audio/CLAP/att/resample_8k\endcsname{0.81}
\expandafter\def\csname val@fp:audio/CLAP/att/resample_8k/pct\endcsname{81}
\expandafter\def\csname val@fp:audio/CLAP/att/reverb\endcsname{0.65}
\expandafter\def\csname val@fp:audio/CLAP/att/reverb/pct\endcsname{65}
\expandafter\def\csname val@fp:audio/CLAP/att/speed_1.05\endcsname{0.90}
\expandafter\def\csname val@fp:audio/CLAP/att/speed_1.05/pct\endcsname{90}
\expandafter\def\csname val@fp:audio/CLAP/att/tempo_0.9\endcsname{0.84}
\expandafter\def\csname val@fp:audio/CLAP/att/tempo_0.9/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/CLAP/att/tempo_1.1\endcsname{0.86}
\expandafter\def\csname val@fp:audio/CLAP/att/tempo_1.1/pct\endcsname{86}
\expandafter\def\csname val@fp:audio/CLAP/bits\endcsname{16384}
\expandafter\def\csname val@fp:audio/CLAP/fam/chain\endcsname{0.32}
\expandafter\def\csname val@fp:audio/CLAP/fam/codec\endcsname{0.94}
\expandafter\def\csname val@fp:audio/CLAP/fam/excerpt\endcsname{0.70}
\expandafter\def\csname val@fp:audio/CLAP/fam/filter\endcsname{0.84}
\expandafter\def\csname val@fp:audio/CLAP/fam/noise\endcsname{0.30}
\expandafter\def\csname val@fp:audio/CLAP/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/fam/time-pitch\endcsname{0.88}
\expandafter\def\csname val@fp:audio/CLAP/ms\endcsname{1.1}
\expandafter\def\csname val@fp:audio/CLAP/muAP\endcsname{0.446}
\expandafter\def\csname val@fp:audio/CLAP/muAP/pct\endcsname{44.6}
\expandafter\def\csname val@fp:audio/CLAP/music/att/_all\endcsname{0.83}
\expandafter\def\csname val@fp:audio/CLAP/music/att/_all/pct\endcsname{83}
\expandafter\def\csname val@fp:audio/CLAP/music/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/babble_0db\endcsname{0.20}
\expandafter\def\csname val@fp:audio/CLAP/music/att/babble_0db/pct\endcsname{20}
\expandafter\def\csname val@fp:audio/CLAP/music/att/babble_10db\endcsname{0.69}
\expandafter\def\csname val@fp:audio/CLAP/music/att/babble_10db/pct\endcsname{69}
\expandafter\def\csname val@fp:audio/CLAP/music/att/compressor\endcsname{0.98}
\expandafter\def\csname val@fp:audio/CLAP/music/att/compressor/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt10\endcsname{0.96}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt10/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt10_mp3_noise20\endcsname{0.64}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt10_mp3_noise20/pct\endcsname{64}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt5\endcsname{0.79}
\expandafter\def\csname val@fp:audio/CLAP/music/att/excerpt5/pct\endcsname{79}
\expandafter\def\csname val@fp:audio/CLAP/music/att/lowpass_2k\endcsname{0.87}
\expandafter\def\csname val@fp:audio/CLAP/music/att/lowpass_2k/pct\endcsname{87}
\expandafter\def\csname val@fp:audio/CLAP/music/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/noise_10db\endcsname{0.28}
\expandafter\def\csname val@fp:audio/CLAP/music/att/noise_10db/pct\endcsname{28}
\expandafter\def\csname val@fp:audio/CLAP/music/att/noise_20db\endcsname{0.78}
\expandafter\def\csname val@fp:audio/CLAP/music/att/noise_20db/pct\endcsname{78}
\expandafter\def\csname val@fp:audio/CLAP/music/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/opus_24\endcsname{0.99}
\expandafter\def\csname val@fp:audio/CLAP/music/att/opus_24/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/CLAP/music/att/phone\endcsname{0.92}
\expandafter\def\csname val@fp:audio/CLAP/music/att/phone/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/CLAP/music/att/pitch+2\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/pitch+2/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/rerecord\endcsname{0.36}
\expandafter\def\csname val@fp:audio/CLAP/music/att/rerecord/pct\endcsname{36}
\expandafter\def\csname val@fp:audio/CLAP/music/att/resample_8k\endcsname{0.94}
\expandafter\def\csname val@fp:audio/CLAP/music/att/resample_8k/pct\endcsname{94}
\expandafter\def\csname val@fp:audio/CLAP/music/att/reverb\endcsname{0.98}
\expandafter\def\csname val@fp:audio/CLAP/music/att/reverb/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/CLAP/music/att/speed_1.05\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/speed_1.05/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/tempo_0.9\endcsname{0.99}
\expandafter\def\csname val@fp:audio/CLAP/music/att/tempo_0.9/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/att/tempo_1.1\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/music/att/tempo_1.1/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/music/tpr\endcsname{0.371}
\expandafter\def\csname val@fp:audio/CLAP/nodedup/tpr\endcsname{0.295}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/_all\endcsname{0.53}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/_all/pct\endcsname{53}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/aac_64\endcsname{0.94}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/aac_64/pct\endcsname{94}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/babble_0db\endcsname{0.00}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/babble_0db/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/babble_10db\endcsname{0.01}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/babble_10db/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/compressor\endcsname{0.99}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt10\endcsname{0.72}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt10/pct\endcsname{72}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt10_mp3_noise20\endcsname{0.07}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt10_mp3_noise20/pct\endcsname{7}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt5\endcsname{0.13}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/excerpt5/pct\endcsname{13}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/lowpass_2k\endcsname{0.89}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/lowpass_2k/pct\endcsname{89}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/mp3_64\endcsname{0.99}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/mp3_64/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/noise_10db\endcsname{0.01}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/noise_10db/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/noise_20db\endcsname{0.06}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/noise_20db/pct\endcsname{6}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/opus_24\endcsname{0.92}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/opus_24/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/phone\endcsname{0.76}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/phone/pct\endcsname{76}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/pitch+2\endcsname{0.78}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/pitch+2/pct\endcsname{78}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/rerecord\endcsname{0.02}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/rerecord/pct\endcsname{2}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/resample_8k\endcsname{0.61}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/resample_8k/pct\endcsname{61}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/reverb\endcsname{0.15}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/reverb/pct\endcsname{15}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/speed_1.05\endcsname{0.77}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/speed_1.05/pct\endcsname{76}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/tempo_0.9\endcsname{0.61}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/tempo_0.9/pct\endcsname{61}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/tempo_1.1\endcsname{0.64}
\expandafter\def\csname val@fp:audio/CLAP/speech/att/tempo_1.1/pct\endcsname{64}
\expandafter\def\csname val@fp:audio/CLAP/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/Chromaprint/FPRq@query@0.01\endcsname{0.016}
\expandafter\def\csname val@fp:audio/Chromaprint/FPRq@query@0.01/pct\endcsname{1.6}
\expandafter\def\csname val@fp:audio/Chromaprint/R@1\endcsname{0.805}
\expandafter\def\csname val@fp:audio/Chromaprint/R@1/pct\endcsname{80.5}
\expandafter\def\csname val@fp:audio/Chromaprint/R@10\endcsname{0.820}
\expandafter\def\csname val@fp:audio/Chromaprint/R@10/pct\endcsname{82.0}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@0.0001\endcsname{0.771}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@0.0001/pct\endcsname{77.1}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@1e-05\endcsname{0.727}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@1e-05/pct\endcsname{72.7}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@1e-06\endcsname{0.688}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@pair@1e-06/pct\endcsname{68.8}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@query@0.01\endcsname{0.704}
\expandafter\def\csname val@fp:audio/Chromaprint/TPR@query@0.01/pct\endcsname{70.4}
\expandafter\def\csname val@fp:audio/Chromaprint/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/babble_0db\endcsname{0.27}
\expandafter\def\csname val@fp:audio/Chromaprint/att/babble_0db/pct\endcsname{27}
\expandafter\def\csname val@fp:audio/Chromaprint/att/babble_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/Chromaprint/att/babble_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/Chromaprint/att/compressor\endcsname{0.96}
\expandafter\def\csname val@fp:audio/Chromaprint/att/compressor/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/phone\endcsname{0.61}
\expandafter\def\csname val@fp:audio/Chromaprint/att/phone/pct\endcsname{61}
\expandafter\def\csname val@fp:audio/Chromaprint/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/Chromaprint/att/pitch+2/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/Chromaprint/att/rerecord\endcsname{0.45}
\expandafter\def\csname val@fp:audio/Chromaprint/att/rerecord/pct\endcsname{45}
\expandafter\def\csname val@fp:audio/Chromaprint/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/att/reverb\endcsname{0.86}
\expandafter\def\csname val@fp:audio/Chromaprint/att/reverb/pct\endcsname{86}
\expandafter\def\csname val@fp:audio/Chromaprint/att/speed_1.05\endcsname{0.03}
\expandafter\def\csname val@fp:audio/Chromaprint/att/speed_1.05/pct\endcsname{3}
\expandafter\def\csname val@fp:audio/Chromaprint/att/tempo_0.9\endcsname{0.84}
\expandafter\def\csname val@fp:audio/Chromaprint/att/tempo_0.9/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/Chromaprint/att/tempo_1.1\endcsname{0.91}
\expandafter\def\csname val@fp:audio/Chromaprint/att/tempo_1.1/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/Chromaprint/bits\endcsname{7072}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/chain\endcsname{0.72}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/excerpt\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/filter\endcsname{0.86}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/noise\endcsname{0.81}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/fam/time-pitch\endcsname{0.45}
\expandafter\def\csname val@fp:audio/Chromaprint/ms\endcsname{2.0}
\expandafter\def\csname val@fp:audio/Chromaprint/muAP\endcsname{0.817}
\expandafter\def\csname val@fp:audio/Chromaprint/muAP/pct\endcsname{81.7}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/_all\endcsname{0.80}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/_all/pct\endcsname{80}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/babble_0db\endcsname{0.36}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/babble_0db/pct\endcsname{36}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/babble_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/babble_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/compressor\endcsname{0.98}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/compressor/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/phone\endcsname{0.52}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/phone/pct\endcsname{52}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/pitch+2/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/rerecord\endcsname{0.37}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/rerecord/pct\endcsname{37}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/reverb\endcsname{0.87}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/reverb/pct\endcsname{87}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/speed_1.05\endcsname{0.04}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/speed_1.05/pct\endcsname{4}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/tempo_0.9\endcsname{0.75}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/tempo_0.9/pct\endcsname{75}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/tempo_1.1\endcsname{0.86}
\expandafter\def\csname val@fp:audio/Chromaprint/music/att/tempo_1.1/pct\endcsname{86}
\expandafter\def\csname val@fp:audio/Chromaprint/music/tpr\endcsname{0.685}
\expandafter\def\csname val@fp:audio/Chromaprint/nodedup/tpr\endcsname{0.364}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/_all\endcsname{0.82}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/_all/pct\endcsname{82}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/babble_0db\endcsname{0.13}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/babble_0db/pct\endcsname{13}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/babble_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/babble_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/compressor\endcsname{0.92}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/compressor/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/phone\endcsname{0.74}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/phone/pct\endcsname{74}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/pitch+2\endcsname{0.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/rerecord\endcsname{0.57}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/rerecord/pct\endcsname{57}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/reverb\endcsname{0.84}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/reverb/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/speed_1.05\endcsname{0.00}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/speed_1.05/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/tempo_0.9\endcsname{0.98}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/tempo_0.9/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/tempo_1.1\endcsname{0.98}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/att/tempo_1.1/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/Chromaprint/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/FPRq@query@0.01\endcsname{0.019}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/FPRq@query@0.01/pct\endcsname{1.9}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/R@1\endcsname{0.749}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/R@1/pct\endcsname{74.9}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/R@10\endcsname{0.810}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/R@10/pct\endcsname{81.0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@0.0001\endcsname{0.588}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@0.0001/pct\endcsname{58.8}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@1e-05\endcsname{0.401}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@1e-05/pct\endcsname{40.1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@1e-06\endcsname{0.321}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@pair@1e-06/pct\endcsname{32.1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@query@0.01\endcsname{0.454}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/TPR@query@0.01/pct\endcsname{45.4}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/babble_0db\endcsname{0.20}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/babble_0db/pct\endcsname{20}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/babble_10db\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/babble_10db/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/compressor\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/compressor/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt10\endcsname{0.69}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt10/pct\endcsname{69}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt10_mp3_noise20\endcsname{0.68}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt10_mp3_noise20/pct\endcsname{68}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt5\endcsname{0.21}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/excerpt5/pct\endcsname{21}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/lowpass_2k\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/noise_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/noise_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/phone\endcsname{0.67}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/phone/pct\endcsname{67}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/pitch+2/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/rerecord\endcsname{0.34}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/rerecord/pct\endcsname{34}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/reverb\endcsname{0.94}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/reverb/pct\endcsname{94}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/speed_1.05\endcsname{0.09}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/speed_1.05/pct\endcsname{9}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/tempo_0.9\endcsname{0.97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/tempo_0.9/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/tempo_1.1\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/att/tempo_1.1/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/bits\endcsname{256}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/chain\endcsname{0.51}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/excerpt\endcsname{0.45}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/filter\endcsname{0.90}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/noise\endcsname{0.79}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/fam/time-pitch\endcsname{0.51}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/ms\endcsname{2.0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/muAP\endcsname{0.658}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/muAP/pct\endcsname{65.8}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/_all\endcsname{0.72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/_all/pct\endcsname{72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/babble_0db\endcsname{0.20}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/babble_0db/pct\endcsname{20}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/babble_10db\endcsname{0.97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/babble_10db/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/compressor\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/compressor/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt10\endcsname{0.56}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt10/pct\endcsname{56}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt10_mp3_noise20\endcsname{0.55}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt10_mp3_noise20/pct\endcsname{55}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt5\endcsname{0.23}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/excerpt5/pct\endcsname{22}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/lowpass_2k\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/lowpass_2k/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/noise_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/noise_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/phone\endcsname{0.50}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/phone/pct\endcsname{50}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/pitch+2/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/rerecord\endcsname{0.14}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/rerecord/pct\endcsname{14}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/reverb\endcsname{0.90}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/reverb/pct\endcsname{90}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/speed_1.05\endcsname{0.11}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/speed_1.05/pct\endcsname{11}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/tempo_0.9\endcsname{0.96}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/tempo_0.9/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/tempo_1.1\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/att/tempo_1.1/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/music/tpr\endcsname{0.458}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/nodedup/tpr\endcsname{0.279}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/_all\endcsname{0.80}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/_all/pct\endcsname{80}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/babble_0db\endcsname{0.21}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/babble_0db/pct\endcsname{21}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/babble_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/babble_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt10\endcsname{0.88}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt10/pct\endcsname{88}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt10_mp3_noise20\endcsname{0.88}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt10_mp3_noise20/pct\endcsname{88}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt5\endcsname{0.19}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/excerpt5/pct\endcsname{19}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/phone\endcsname{0.92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/phone/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/pitch+2\endcsname{0.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/rerecord\endcsname{0.64}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/rerecord/pct\endcsname{64}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/reverb\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/reverb/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/speed_1.05\endcsname{0.06}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/speed_1.05/pct\endcsname{6}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/tempo_0.9\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/tempo_0.9/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/tempo_1.1\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/att/tempo_1.1/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-256/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/FPRq@query@0.01\endcsname{0.017}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/FPRq@query@0.01/pct\endcsname{1.7}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/R@1\endcsname{0.662}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/R@1/pct\endcsname{66.2}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/R@10\endcsname{0.744}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/R@10/pct\endcsname{74.4}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@0.0001\endcsname{0.527}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@0.0001/pct\endcsname{52.7}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@1e-05\endcsname{0.359}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@1e-05/pct\endcsname{35.9}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@1e-06\endcsname{0.212}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@pair@1e-06/pct\endcsname{21.2}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@query@0.01\endcsname{0.409}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/TPR@query@0.01/pct\endcsname{40.9}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/aac_64\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/babble_0db\endcsname{0.08}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/babble_0db/pct\endcsname{8}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/babble_10db\endcsname{0.84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/babble_10db/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/compressor\endcsname{0.90}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/compressor/pct\endcsname{90}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt10\endcsname{0.41}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt10/pct\endcsname{41}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt10_mp3_noise20\endcsname{0.44}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt10_mp3_noise20/pct\endcsname{44}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt5\endcsname{0.10}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/excerpt5/pct\endcsname{10}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/lowpass_2k\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/lowpass_2k/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/noise_10db\endcsname{0.97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/noise_10db/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/noise_20db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/noise_20db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/opus_24\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/opus_24/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/phone\endcsname{0.49}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/phone/pct\endcsname{49}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/pitch+2\endcsname{0.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/rerecord\endcsname{0.18}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/rerecord/pct\endcsname{18}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/reverb\endcsname{0.72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/reverb/pct\endcsname{72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/speed_1.05\endcsname{0.03}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/speed_1.05/pct\endcsname{3}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/tempo_0.9\endcsname{0.89}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/tempo_0.9/pct\endcsname{89}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/tempo_1.1\endcsname{0.92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/att/tempo_1.1/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/chain\endcsname{0.31}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/codec\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/excerpt\endcsname{0.25}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/filter\endcsname{0.77}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/noise\endcsname{0.72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/fam/time-pitch\endcsname{0.46}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/ms\endcsname{2.0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/muAP\endcsname{0.581}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/muAP/pct\endcsname{58.1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/_all\endcsname{0.63}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/_all/pct\endcsname{63}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/aac_64\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/aac_64/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/babble_0db\endcsname{0.09}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/babble_0db/pct\endcsname{8}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/babble_10db\endcsname{0.84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/babble_10db/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/compressor\endcsname{0.92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/compressor/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt10\endcsname{0.25}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt10/pct\endcsname{25}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt10_mp3_noise20\endcsname{0.28}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt10_mp3_noise20/pct\endcsname{28}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt5\endcsname{0.12}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/excerpt5/pct\endcsname{12}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/lowpass_2k\endcsname{0.97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/lowpass_2k/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/mp3_64\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/mp3_64/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/noise_10db\endcsname{0.97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/noise_10db/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/noise_20db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/noise_20db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/none\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/none/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/opus_24\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/opus_24/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/phone\endcsname{0.34}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/phone/pct\endcsname{34}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/rerecord\endcsname{0.06}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/rerecord/pct\endcsname{6}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/resample_8k\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/resample_8k/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/reverb\endcsname{0.69}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/reverb/pct\endcsname{69}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/speed_1.05\endcsname{0.05}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/speed_1.05/pct\endcsname{5}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/tempo_0.9\endcsname{0.84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/tempo_0.9/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/tempo_1.1\endcsname{0.89}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/att/tempo_1.1/pct\endcsname{89}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/music/tpr\endcsname{0.406}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/nodedup/tpr\endcsname{0.209}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/_all\endcsname{0.71}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/_all/pct\endcsname{71}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/babble_0db\endcsname{0.08}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/babble_0db/pct\endcsname{8}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/babble_10db\endcsname{0.84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/babble_10db/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/compressor\endcsname{0.87}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/compressor/pct\endcsname{87}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt10\endcsname{0.66}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt10/pct\endcsname{66}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt10_mp3_noise20\endcsname{0.68}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt10_mp3_noise20/pct\endcsname{68}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt5\endcsname{0.07}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/excerpt5/pct\endcsname{7}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/lowpass_2k\endcsname{0.99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/lowpass_2k/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/noise_10db\endcsname{0.98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/noise_10db/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/phone\endcsname{0.71}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/phone/pct\endcsname{72}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/pitch+2\endcsname{0.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/rerecord\endcsname{0.38}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/rerecord/pct\endcsname{38}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/reverb\endcsname{0.76}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/reverb/pct\endcsname{76}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/speed_1.05\endcsname{0.01}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/speed_1.05/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/tempo_0.9\endcsname{0.96}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/tempo_0.9/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/tempo_1.1\endcsname{0.95}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/att/tempo_1.1/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/ISCC-Audio-64/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/NMFP-triplet/FPRq@query@0.01\endcsname{0.018}
\expandafter\def\csname val@fp:audio/NMFP-triplet/FPRq@query@0.01/pct\endcsname{1.8}
\expandafter\def\csname val@fp:audio/NMFP-triplet/R@1\endcsname{0.905}
\expandafter\def\csname val@fp:audio/NMFP-triplet/R@1/pct\endcsname{90.5}
\expandafter\def\csname val@fp:audio/NMFP-triplet/R@10\endcsname{0.924}
\expandafter\def\csname val@fp:audio/NMFP-triplet/R@10/pct\endcsname{92.4}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@0.0001\endcsname{0.902}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@0.0001/pct\endcsname{90.2}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@1e-05\endcsname{0.892}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@1e-05/pct\endcsname{89.2}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@1e-06\endcsname{0.846}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@pair@1e-06/pct\endcsname{84.6}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@query@0.01\endcsname{0.862}
\expandafter\def\csname val@fp:audio/NMFP-triplet/TPR@query@0.01/pct\endcsname{86.2}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/babble_0db\endcsname{0.91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/babble_0db/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/babble_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/babble_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/pitch+2\endcsname{0.06}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/pitch+2/pct\endcsname{6}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/rerecord\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/rerecord/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/speed_1.05\endcsname{0.06}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/speed_1.05/pct\endcsname{6}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/tempo_0.9\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/tempo_0.9/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/tempo_1.1\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/att/tempo_1.1/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/bits\endcsname{239108}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/chain\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/excerpt\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/filter\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/noise\endcsname{0.98}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/fam/time-pitch\endcsname{0.53}
\expandafter\def\csname val@fp:audio/NMFP-triplet/ms\endcsname{--}
\expandafter\def\csname val@fp:audio/NMFP-triplet/muAP\endcsname{0.937}
\expandafter\def\csname val@fp:audio/NMFP-triplet/muAP/pct\endcsname{93.7}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/_all\endcsname{0.91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/_all/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/babble_0db\endcsname{0.91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/babble_0db/pct\endcsname{90}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/babble_10db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/babble_10db/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/pitch+2\endcsname{0.09}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/pitch+2/pct\endcsname{9}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/rerecord\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/rerecord/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/speed_1.05\endcsname{0.04}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/speed_1.05/pct\endcsname{4}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/tempo_0.9\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/tempo_0.9/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/tempo_1.1\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/att/tempo_1.1/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/music/tpr\endcsname{0.858}
\expandafter\def\csname val@fp:audio/NMFP-triplet/nodedup/tpr\endcsname{0.281}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/_all\endcsname{0.91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/_all/pct\endcsname{90}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/babble_0db\endcsname{0.91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/babble_0db/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/babble_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/babble_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt10_mp3_noise20\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt5\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/excerpt5/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/pitch+2\endcsname{0.01}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/rerecord\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/rerecord/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/speed_1.05\endcsname{0.09}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/speed_1.05/pct\endcsname{9}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/tempo_0.9\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/tempo_0.9/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/tempo_1.1\endcsname{1.00}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/att/tempo_1.1/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/NMFP-triplet/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/audfprint/FPRq@query@0.01\endcsname{0.008}
\expandafter\def\csname val@fp:audio/audfprint/FPRq@query@0.01/pct\endcsname{0.8}
\expandafter\def\csname val@fp:audio/audfprint/R@1\endcsname{0.851}
\expandafter\def\csname val@fp:audio/audfprint/R@1/pct\endcsname{85.1}
\expandafter\def\csname val@fp:audio/audfprint/R@10\endcsname{0.871}
\expandafter\def\csname val@fp:audio/audfprint/R@10/pct\endcsname{87.1}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@0.0001\endcsname{0.801}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@0.0001/pct\endcsname{80.1}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@1e-05\endcsname{0.757}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@1e-05/pct\endcsname{75.7}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@1e-06\endcsname{0.599}
\expandafter\def\csname val@fp:audio/audfprint/TPR@pair@1e-06/pct\endcsname{59.9}
\expandafter\def\csname val@fp:audio/audfprint/TPR@query@0.01\endcsname{0.660}
\expandafter\def\csname val@fp:audio/audfprint/TPR@query@0.01/pct\endcsname{66.0}
\expandafter\def\csname val@fp:audio/audfprint/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/babble_0db\endcsname{0.88}
\expandafter\def\csname val@fp:audio/audfprint/att/babble_0db/pct\endcsname{88}
\expandafter\def\csname val@fp:audio/audfprint/att/babble_10db\endcsname{0.98}
\expandafter\def\csname val@fp:audio/audfprint/att/babble_10db/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/audfprint/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt10\endcsname{0.99}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt10/pct\endcsname{99}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt10_mp3_noise20\endcsname{0.94}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt10_mp3_noise20/pct\endcsname{94}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt5\endcsname{0.92}
\expandafter\def\csname val@fp:audio/audfprint/att/excerpt5/pct\endcsname{92}
\expandafter\def\csname val@fp:audio/audfprint/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/noise_10db\endcsname{0.98}
\expandafter\def\csname val@fp:audio/audfprint/att/noise_10db/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/audfprint/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/pitch+2\endcsname{0.07}
\expandafter\def\csname val@fp:audio/audfprint/att/pitch+2/pct\endcsname{7}
\expandafter\def\csname val@fp:audio/audfprint/att/rerecord\endcsname{0.85}
\expandafter\def\csname val@fp:audio/audfprint/att/rerecord/pct\endcsname{85}
\expandafter\def\csname val@fp:audio/audfprint/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/att/speed_1.05\endcsname{0.01}
\expandafter\def\csname val@fp:audio/audfprint/att/speed_1.05/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/audfprint/att/tempo_0.9\endcsname{0.61}
\expandafter\def\csname val@fp:audio/audfprint/att/tempo_0.9/pct\endcsname{61}
\expandafter\def\csname val@fp:audio/audfprint/att/tempo_1.1\endcsname{0.65}
\expandafter\def\csname val@fp:audio/audfprint/att/tempo_1.1/pct\endcsname{65}
\expandafter\def\csname val@fp:audio/audfprint/bits\endcsname{40397}
\expandafter\def\csname val@fp:audio/audfprint/fam/chain\endcsname{0.90}
\expandafter\def\csname val@fp:audio/audfprint/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/fam/excerpt\endcsname{0.95}
\expandafter\def\csname val@fp:audio/audfprint/fam/filter\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/fam/noise\endcsname{0.96}
\expandafter\def\csname val@fp:audio/audfprint/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/fam/time-pitch\endcsname{0.33}
\expandafter\def\csname val@fp:audio/audfprint/ms\endcsname{1.4}
\expandafter\def\csname val@fp:audio/audfprint/muAP\endcsname{0.851}
\expandafter\def\csname val@fp:audio/audfprint/muAP/pct\endcsname{85.1}
\expandafter\def\csname val@fp:audio/audfprint/music/att/_all\endcsname{0.84}
\expandafter\def\csname val@fp:audio/audfprint/music/att/_all/pct\endcsname{84}
\expandafter\def\csname val@fp:audio/audfprint/music/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/babble_0db\endcsname{0.82}
\expandafter\def\csname val@fp:audio/audfprint/music/att/babble_0db/pct\endcsname{82}
\expandafter\def\csname val@fp:audio/audfprint/music/att/babble_10db\endcsname{0.96}
\expandafter\def\csname val@fp:audio/audfprint/music/att/babble_10db/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/audfprint/music/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt10\endcsname{0.98}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt10/pct\endcsname{98}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt10_mp3_noise20\endcsname{0.91}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt10_mp3_noise20/pct\endcsname{91}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt5\endcsname{0.89}
\expandafter\def\csname val@fp:audio/audfprint/music/att/excerpt5/pct\endcsname{88}
\expandafter\def\csname val@fp:audio/audfprint/music/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/noise_10db\endcsname{0.96}
\expandafter\def\csname val@fp:audio/audfprint/music/att/noise_10db/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/audfprint/music/att/noise_20db\endcsname{0.99}
\expandafter\def\csname val@fp:audio/audfprint/music/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/pitch+2\endcsname{0.12}
\expandafter\def\csname val@fp:audio/audfprint/music/att/pitch+2/pct\endcsname{12}
\expandafter\def\csname val@fp:audio/audfprint/music/att/rerecord\endcsname{0.77}
\expandafter\def\csname val@fp:audio/audfprint/music/att/rerecord/pct\endcsname{77}
\expandafter\def\csname val@fp:audio/audfprint/music/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/music/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/music/att/speed_1.05\endcsname{0.01}
\expandafter\def\csname val@fp:audio/audfprint/music/att/speed_1.05/pct\endcsname{1}
\expandafter\def\csname val@fp:audio/audfprint/music/att/tempo_0.9\endcsname{0.60}
\expandafter\def\csname val@fp:audio/audfprint/music/att/tempo_0.9/pct\endcsname{60}
\expandafter\def\csname val@fp:audio/audfprint/music/att/tempo_1.1\endcsname{0.65}
\expandafter\def\csname val@fp:audio/audfprint/music/att/tempo_1.1/pct\endcsname{65}
\expandafter\def\csname val@fp:audio/audfprint/music/tpr\endcsname{0.649}
\expandafter\def\csname val@fp:audio/audfprint/nodedup/tpr\endcsname{0.224}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/_all\endcsname{0.87}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/_all/pct\endcsname{87}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/aac_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/aac_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/babble_0db\endcsname{0.97}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/babble_0db/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/babble_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/babble_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/compressor\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/compressor/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt10\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt10/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt10_mp3_noise20\endcsname{0.99}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt10_mp3_noise20/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt5\endcsname{0.96}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/excerpt5/pct\endcsname{96}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/lowpass_2k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/lowpass_2k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/mp3_64\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/mp3_64/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/noise_10db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/noise_10db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/noise_20db\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/noise_20db/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/opus_24\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/opus_24/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/phone\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/phone/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/pitch+2\endcsname{0.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/pitch+2/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/rerecord\endcsname{0.97}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/rerecord/pct\endcsname{97}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/resample_8k\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/resample_8k/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/reverb\endcsname{1.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/reverb/pct\endcsname{100}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/speed_1.05\endcsname{0.00}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/speed_1.05/pct\endcsname{0}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/tempo_0.9\endcsname{0.62}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/tempo_0.9/pct\endcsname{62}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/tempo_1.1\endcsname{0.66}
\expandafter\def\csname val@fp:audio/audfprint/speech/att/tempo_1.1/pct\endcsname{66}
\expandafter\def\csname val@fp:audio/audfprint/speech/tpr\endcsname{--}
\expandafter\def\csname val@fp:audio/cal_sources\endcsname{193}
\expandafter\def\csname val@fp:audio/dedup/items\endcsname{32}
\expandafter\def\csname val@fp:audio/dedup/neg\endcsname{17}
\expandafter\def\csname val@fp:audio/pos_sources\endcsname{1{,}000}
\expandafter\def\csname val@fp:c2pa/list_fingerprint\endcsname{9}
\expandafter\def\csname val@fp:c2pa/list_total\endcsname{53}
\expandafter\def\csname val@fp:c2pa/list_watermark\endcsname{44}
\expandafter\def\csname val@fp:corpus/abo/bg\endcsname{200}
\expandafter\def\csname val@fp:corpus/abo/dist\endcsname{100{,}000}
\expandafter\def\csname val@fp:corpus/abo/hard\endcsname{1{,}000}
\expandafter\def\csname val@fp:corpus/abo/neg\endcsname{2{,}000}
\expandafter\def\csname val@fp:corpus/abo/pos\endcsname{2{,}000}
\expandafter\def\csname val@fp:corpus/abo/reg\endcsname{5{,}000}
\expandafter\def\csname val@fp:corpus/audio/dist\endcsname{5{,}350}
\expandafter\def\csname val@fp:corpus/audio/music\endcsname{5{,}000}
\expandafter\def\csname val@fp:corpus/audio/neg\endcsname{400}
\expandafter\def\csname val@fp:corpus/audio/reg\endcsname{1{,}000}
\expandafter\def\csname val@fp:corpus/audio/speech\endcsname{1{,}750}
\expandafter\def\csname val@fp:corpus/disc/gt\endcsname{3{,}000}
\expandafter\def\csname val@fp:corpus/disc/negq\endcsname{3{,}000}
\expandafter\def\csname val@fp:corpus/disc/refs\endcsname{25{,}000}
\expandafter\def\csname val@fp:corpus/video/dist\endcsname{323}
\expandafter\def\csname val@fp:corpus/video/neg\endcsname{40}
\expandafter\def\csname val@fp:corpus/video/reg\endcsname{120}
\expandafter\def\csname val@fp:corpus/video/xiph\endcsname{23}
\expandafter\def\csname val@fp:count/attacks\endcsname{79}
\expandafter\def\csname val@fp:count/audio/attacks\endcsname{20}
\expandafter\def\csname val@fp:count/audio/methods\endcsname{6}
\expandafter\def\csname val@fp:count/audio/methods_p\endcsname{5}
\expandafter\def\csname val@fp:count/audio/neg_cal\endcsname{4{,}053}
\expandafter\def\csname val@fp:count/audio/neg_test\endcsname{3{,}990}
\expandafter\def\csname val@fp:count/audio/nref\endcsname{6{,}350}
\expandafter\def\csname val@fp:count/audio/pos\endcsname{21{,}000}
\expandafter\def\csname val@fp:count/image/attacks\endcsname{35}
\expandafter\def\csname val@fp:count/image/methods\endcsname{21}
\expandafter\def\csname val@fp:count/image/methods_p\endcsname{17}
\expandafter\def\csname val@fp:count/image/neg_cal\endcsname{27{,}684}
\expandafter\def\csname val@fp:count/image/neg_test\endcsname{26{,}820}
\expandafter\def\csname val@fp:count/image/nref\endcsname{98{,}985}
\expandafter\def\csname val@fp:count/image/pos\endcsname{72{,}000}
\expandafter\def\csname val@fp:count/methods\endcsname{35}
\expandafter\def\csname val@fp:count/video/attacks\endcsname{24}
\expandafter\def\csname val@fp:count/video/methods\endcsname{8}
\expandafter\def\csname val@fp:count/video/methods_p\endcsname{6}
\expandafter\def\csname val@fp:count/video/neg_cal\endcsname{500}
\expandafter\def\csname val@fp:count/video/neg_test\endcsname{500}
\expandafter\def\csname val@fp:count/video/nref\endcsname{443}
\expandafter\def\csname val@fp:count/video/pos\endcsname{3{,}000}
\expandafter\def\csname val@fp:dedup/n_dist\endcsname{100{,}000}
\expandafter\def\csname val@fp:dedup/n_dist_flagged\endcsname{6{,}015}
\expandafter\def\csname val@fp:dedup/n_hard\endcsname{1{,}000}
\expandafter\def\csname val@fp:dedup/n_hard_near_duplicate\endcsname{54}
\expandafter\def\csname val@fp:dedup/n_neg_flagged\endcsname{486}
\expandafter\def\csname val@fp:edit/n_edits\endcsname{6{,}000}
\expandafter\def\csname val@fp:edit/n_sources\endcsname{500}
\expandafter\def\csname val@fp:editret/BlockMean/R@1\endcsname{0.693}
\expandafter\def\csname val@fp:editret/BlockMean/area/0.01\endcsname{0.86}
\expandafter\def\csname val@fp:editret/BlockMean/area/0.03\endcsname{0.83}
\expandafter\def\csname val@fp:editret/BlockMean/area/0.1\endcsname{0.68}
\expandafter\def\csname val@fp:editret/BlockMean/area/0.25\endcsname{0.40}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/post/crop90\endcsname{0.37}
\expandafter\def\csname val@fp:editret/BlockMean/post/jpeg75\endcsname{0.79}
\expandafter\def\csname val@fp:editret/BlockMean/post/none\endcsname{0.80}
\expandafter\def\csname val@fp:editret/BlockMean/post/resize0.75_jpeg80\endcsname{0.81}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/area/0.01\endcsname{0.33}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/area/0.03\endcsname{0.16}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/area/0.1\endcsname{0.03}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/post/jpeg75\endcsname{0.17}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/post/none\endcsname{0.18}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/post/resize0.75_jpeg80\endcsname{0.18}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/tpr\endcsname{0.132}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/copymove\endcsname{0.06}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/inpaint-lama\endcsname{0.27}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/inpaint-telea\endcsname{0.19}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/recolor\endcsname{0.15}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/splice\endcsname{0.06}
\expandafter\def\csname val@fp:editret/BlockMean/query@0.01/type/textreplace\endcsname{0.07}
\expandafter\def\csname val@fp:editret/BlockMean/type/copymove\endcsname{0.73}
\expandafter\def\csname val@fp:editret/BlockMean/type/inpaint-lama\endcsname{0.77}
\expandafter\def\csname val@fp:editret/BlockMean/type/inpaint-telea\endcsname{0.79}
\expandafter\def\csname val@fp:editret/BlockMean/type/recolor\endcsname{0.69}
\expandafter\def\csname val@fp:editret/BlockMean/type/splice\endcsname{0.65}
\expandafter\def\csname val@fp:editret/BlockMean/type/textreplace\endcsname{0.53}
\expandafter\def\csname val@fp:editret/Blockhash-256/R@1\endcsname{0.727}
\expandafter\def\csname val@fp:editret/Blockhash-256/area/0.01\endcsname{0.87}
\expandafter\def\csname val@fp:editret/Blockhash-256/area/0.03\endcsname{0.85}
\expandafter\def\csname val@fp:editret/Blockhash-256/area/0.1\endcsname{0.74}
\expandafter\def\csname val@fp:editret/Blockhash-256/area/0.25\endcsname{0.46}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/post/crop90\endcsname{0.44}
\expandafter\def\csname val@fp:editret/Blockhash-256/post/jpeg75\endcsname{0.82}
\expandafter\def\csname val@fp:editret/Blockhash-256/post/none\endcsname{0.84}
\expandafter\def\csname val@fp:editret/Blockhash-256/post/resize0.75_jpeg80\endcsname{0.81}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/query@0.01/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/copymove\endcsname{0.75}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/inpaint-lama\endcsname{0.79}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/inpaint-telea\endcsname{0.80}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/recolor\endcsname{0.73}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/splice\endcsname{0.71}
\expandafter\def\csname val@fp:editret/Blockhash-256/type/textreplace\endcsname{0.59}
\expandafter\def\csname val@fp:editret/ColorMoment/R@1\endcsname{0.153}
\expandafter\def\csname val@fp:editret/ColorMoment/area/0.01\endcsname{0.29}
\expandafter\def\csname val@fp:editret/ColorMoment/area/0.03\endcsname{0.21}
\expandafter\def\csname val@fp:editret/ColorMoment/area/0.1\endcsname{0.09}
\expandafter\def\csname val@fp:editret/ColorMoment/area/0.25\endcsname{0.02}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/post/crop90\endcsname{0.11}
\expandafter\def\csname val@fp:editret/ColorMoment/post/jpeg75\endcsname{0.16}
\expandafter\def\csname val@fp:editret/ColorMoment/post/none\endcsname{0.22}
\expandafter\def\csname val@fp:editret/ColorMoment/post/resize0.75_jpeg80\endcsname{0.12}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/query@0.01/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/ColorMoment/type/copymove\endcsname{0.17}
\expandafter\def\csname val@fp:editret/ColorMoment/type/inpaint-lama\endcsname{0.24}
\expandafter\def\csname val@fp:editret/ColorMoment/type/inpaint-telea\endcsname{0.28}
\expandafter\def\csname val@fp:editret/ColorMoment/type/recolor\endcsname{0.07}
\expandafter\def\csname val@fp:editret/ColorMoment/type/splice\endcsname{0.11}
\expandafter\def\csname val@fp:editret/ColorMoment/type/textreplace\endcsname{0.04}
\expandafter\def\csname val@fp:editret/DINOHash-96/R@1\endcsname{0.771}
\expandafter\def\csname val@fp:editret/DINOHash-96/area/0.01\endcsname{0.93}
\expandafter\def\csname val@fp:editret/DINOHash-96/area/0.03\endcsname{0.89}
\expandafter\def\csname val@fp:editret/DINOHash-96/area/0.1\endcsname{0.74}
\expandafter\def\csname val@fp:editret/DINOHash-96/area/0.25\endcsname{0.51}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/area/0.01\endcsname{0.18}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/area/0.03\endcsname{0.09}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/area/0.1\endcsname{0.02}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/post/crop90\endcsname{0.01}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/post/jpeg75\endcsname{0.10}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/post/none\endcsname{0.08}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.10}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/tpr\endcsname{0.072}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/copymove\endcsname{0.05}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/inpaint-lama\endcsname{0.19}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/inpaint-telea\endcsname{0.08}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/recolor\endcsname{0.05}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/splice\endcsname{0.03}
\expandafter\def\csname val@fp:editret/DINOHash-96/pair@1e-07/type/textreplace\endcsname{0.03}
\expandafter\def\csname val@fp:editret/DINOHash-96/post/crop90\endcsname{0.73}
\expandafter\def\csname val@fp:editret/DINOHash-96/post/jpeg75\endcsname{0.77}
\expandafter\def\csname val@fp:editret/DINOHash-96/post/none\endcsname{0.79}
\expandafter\def\csname val@fp:editret/DINOHash-96/post/resize0.75_jpeg80\endcsname{0.79}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/area/0.01\endcsname{0.18}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/area/0.03\endcsname{0.09}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/area/0.1\endcsname{0.02}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/post/crop90\endcsname{0.01}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/post/jpeg75\endcsname{0.10}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/post/none\endcsname{0.08}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/post/resize0.75_jpeg80\endcsname{0.10}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/tpr\endcsname{0.072}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/copymove\endcsname{0.05}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/inpaint-lama\endcsname{0.19}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/inpaint-telea\endcsname{0.08}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/recolor\endcsname{0.05}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/splice\endcsname{0.03}
\expandafter\def\csname val@fp:editret/DINOHash-96/query@0.01/type/textreplace\endcsname{0.03}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/copymove\endcsname{0.78}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/inpaint-lama\endcsname{0.85}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/inpaint-telea\endcsname{0.79}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/recolor\endcsname{0.84}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/splice\endcsname{0.61}
\expandafter\def\csname val@fp:editret/DINOHash-96/type/textreplace\endcsname{0.75}
\expandafter\def\csname val@fp:editret/DINOv2-B/R@1\endcsname{0.932}
\expandafter\def\csname val@fp:editret/DINOv2-B/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/DINOv2-B/area/0.03\endcsname{0.99}
\expandafter\def\csname val@fp:editret/DINOv2-B/area/0.1\endcsname{0.95}
\expandafter\def\csname val@fp:editret/DINOv2-B/area/0.25\endcsname{0.80}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/area/0.01\endcsname{0.86}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/area/0.03\endcsname{0.73}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/area/0.1\endcsname{0.45}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/area/0.25\endcsname{0.15}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/post/crop90\endcsname{0.42}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/post/jpeg75\endcsname{0.59}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/post/none\endcsname{0.59}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.58}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/tpr\endcsname{0.546}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/copymove\endcsname{0.52}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/inpaint-lama\endcsname{0.63}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/inpaint-telea\endcsname{0.56}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/recolor\endcsname{0.67}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/splice\endcsname{0.33}
\expandafter\def\csname val@fp:editret/DINOv2-B/pair@1e-07/type/textreplace\endcsname{0.57}
\expandafter\def\csname val@fp:editret/DINOv2-B/post/crop90\endcsname{0.92}
\expandafter\def\csname val@fp:editret/DINOv2-B/post/jpeg75\endcsname{0.93}
\expandafter\def\csname val@fp:editret/DINOv2-B/post/none\endcsname{0.95}
\expandafter\def\csname val@fp:editret/DINOv2-B/post/resize0.75_jpeg80\endcsname{0.94}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/area/0.01\endcsname{0.87}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/area/0.03\endcsname{0.73}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/area/0.1\endcsname{0.45}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/area/0.25\endcsname{0.15}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/post/crop90\endcsname{0.43}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/post/jpeg75\endcsname{0.59}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/post/none\endcsname{0.60}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/post/resize0.75_jpeg80\endcsname{0.58}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/tpr\endcsname{0.550}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/copymove\endcsname{0.53}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/inpaint-lama\endcsname{0.63}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/inpaint-telea\endcsname{0.56}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/recolor\endcsname{0.68}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/splice\endcsname{0.33}
\expandafter\def\csname val@fp:editret/DINOv2-B/query@0.01/type/textreplace\endcsname{0.57}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/copymove\endcsname{0.96}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/inpaint-lama\endcsname{0.94}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/inpaint-telea\endcsname{0.93}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/recolor\endcsname{0.98}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/splice\endcsname{0.86}
\expandafter\def\csname val@fp:editret/DINOv2-B/type/textreplace\endcsname{0.93}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/R@1\endcsname{0.877}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/area/0.01\endcsname{0.97}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/area/0.03\endcsname{0.96}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/area/0.1\endcsname{0.88}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/area/0.25\endcsname{0.70}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/area/0.01\endcsname{0.65}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/area/0.03\endcsname{0.46}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/area/0.1\endcsname{0.21}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/area/0.25\endcsname{0.06}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/post/crop90\endcsname{0.15}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/post/jpeg75\endcsname{0.42}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/post/none\endcsname{0.41}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.40}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/tpr\endcsname{0.345}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/copymove\endcsname{0.32}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/inpaint-lama\endcsname{0.45}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/inpaint-telea\endcsname{0.35}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/recolor\endcsname{0.41}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/splice\endcsname{0.19}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/pair@1e-07/type/textreplace\endcsname{0.36}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/post/crop90\endcsname{0.85}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/post/jpeg75\endcsname{0.88}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/post/none\endcsname{0.89}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/post/resize0.75_jpeg80\endcsname{0.89}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/area/0.01\endcsname{0.68}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/area/0.03\endcsname{0.49}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/area/0.1\endcsname{0.24}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/area/0.25\endcsname{0.07}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/post/crop90\endcsname{0.18}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/post/jpeg75\endcsname{0.45}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/post/none\endcsname{0.43}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/post/resize0.75_jpeg80\endcsname{0.43}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/tpr\endcsname{0.371}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/copymove\endcsname{0.34}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/inpaint-lama\endcsname{0.48}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/inpaint-telea\endcsname{0.37}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/recolor\endcsname{0.44}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/splice\endcsname{0.21}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/query@0.01/type/textreplace\endcsname{0.38}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/copymove\endcsname{0.91}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/inpaint-lama\endcsname{0.90}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/inpaint-telea\endcsname{0.87}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/recolor\endcsname{0.95}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/splice\endcsname{0.75}
\expandafter\def\csname val@fp:editret/DINOv2-S-LSH256/type/textreplace\endcsname{0.88}
\expandafter\def\csname val@fp:editret/DINOv2-S/R@1\endcsname{0.934}
\expandafter\def\csname val@fp:editret/DINOv2-S/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/DINOv2-S/area/0.03\endcsname{0.98}
\expandafter\def\csname val@fp:editret/DINOv2-S/area/0.1\endcsname{0.95}
\expandafter\def\csname val@fp:editret/DINOv2-S/area/0.25\endcsname{0.82}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/area/0.01\endcsname{0.81}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/area/0.03\endcsname{0.63}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/area/0.1\endcsname{0.34}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/area/0.25\endcsname{0.10}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/post/crop90\endcsname{0.29}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/post/jpeg75\endcsname{0.54}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/post/none\endcsname{0.54}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.52}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/tpr\endcsname{0.470}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/copymove\endcsname{0.44}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/inpaint-lama\endcsname{0.57}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/inpaint-telea\endcsname{0.47}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/recolor\endcsname{0.57}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/splice\endcsname{0.28}
\expandafter\def\csname val@fp:editret/DINOv2-S/pair@1e-07/type/textreplace\endcsname{0.49}
\expandafter\def\csname val@fp:editret/DINOv2-S/post/crop90\endcsname{0.92}
\expandafter\def\csname val@fp:editret/DINOv2-S/post/jpeg75\endcsname{0.93}
\expandafter\def\csname val@fp:editret/DINOv2-S/post/none\endcsname{0.95}
\expandafter\def\csname val@fp:editret/DINOv2-S/post/resize0.75_jpeg80\endcsname{0.94}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/area/0.01\endcsname{0.83}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/area/0.03\endcsname{0.66}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/area/0.1\endcsname{0.36}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/area/0.25\endcsname{0.11}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/post/crop90\endcsname{0.32}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/post/jpeg75\endcsname{0.56}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/post/none\endcsname{0.55}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/post/resize0.75_jpeg80\endcsname{0.54}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/tpr\endcsname{0.492}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/copymove\endcsname{0.47}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/inpaint-lama\endcsname{0.59}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/inpaint-telea\endcsname{0.49}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/recolor\endcsname{0.60}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/splice\endcsname{0.30}
\expandafter\def\csname val@fp:editret/DINOv2-S/query@0.01/type/textreplace\endcsname{0.50}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/copymove\endcsname{0.96}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/inpaint-lama\endcsname{0.94}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/inpaint-telea\endcsname{0.94}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/recolor\endcsname{0.97}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/splice\endcsname{0.86}
\expandafter\def\csname val@fp:editret/DINOv2-S/type/textreplace\endcsname{0.93}
\expandafter\def\csname val@fp:editret/ISC21-1st/R@1\endcsname{0.931}
\expandafter\def\csname val@fp:editret/ISC21-1st/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/ISC21-1st/area/0.03\endcsname{0.98}
\expandafter\def\csname val@fp:editret/ISC21-1st/area/0.1\endcsname{0.94}
\expandafter\def\csname val@fp:editret/ISC21-1st/area/0.25\endcsname{0.82}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/area/0.01\endcsname{0.91}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/area/0.03\endcsname{0.78}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/area/0.1\endcsname{0.51}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/area/0.25\endcsname{0.22}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/post/crop90\endcsname{0.57}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/post/jpeg75\endcsname{0.62}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/post/none\endcsname{0.61}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.61}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/tpr\endcsname{0.602}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/copymove\endcsname{0.55}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/inpaint-lama\endcsname{0.65}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/inpaint-telea\endcsname{0.54}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/recolor\endcsname{0.81}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/splice\endcsname{0.37}
\expandafter\def\csname val@fp:editret/ISC21-1st/pair@1e-07/type/textreplace\endcsname{0.70}
\expandafter\def\csname val@fp:editret/ISC21-1st/post/crop90\endcsname{0.93}
\expandafter\def\csname val@fp:editret/ISC21-1st/post/jpeg75\endcsname{0.92}
\expandafter\def\csname val@fp:editret/ISC21-1st/post/none\endcsname{0.94}
\expandafter\def\csname val@fp:editret/ISC21-1st/post/resize0.75_jpeg80\endcsname{0.94}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/area/0.01\endcsname{0.91}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/area/0.03\endcsname{0.79}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/area/0.1\endcsname{0.53}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/area/0.25\endcsname{0.24}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/post/crop90\endcsname{0.59}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/post/jpeg75\endcsname{0.63}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/post/none\endcsname{0.63}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/post/resize0.75_jpeg80\endcsname{0.62}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/tpr\endcsname{0.617}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/copymove\endcsname{0.56}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/inpaint-lama\endcsname{0.67}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/inpaint-telea\endcsname{0.56}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/recolor\endcsname{0.82}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/splice\endcsname{0.39}
\expandafter\def\csname val@fp:editret/ISC21-1st/query@0.01/type/textreplace\endcsname{0.71}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/copymove\endcsname{0.96}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/inpaint-lama\endcsname{0.94}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/inpaint-telea\endcsname{0.93}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/recolor\endcsname{0.99}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/splice\endcsname{0.81}
\expandafter\def\csname val@fp:editret/ISC21-1st/type/textreplace\endcsname{0.95}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/R@1\endcsname{0.516}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/area/0.01\endcsname{0.81}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/area/0.03\endcsname{0.67}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/area/0.1\endcsname{0.41}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/area/0.25\endcsname{0.18}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/area/0.01\endcsname{0.40}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/area/0.03\endcsname{0.20}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/area/0.1\endcsname{0.05}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/post/crop90\endcsname{0.06}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/post/jpeg75\endcsname{0.21}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/post/none\endcsname{0.20}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.19}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/tpr\endcsname{0.167}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/copymove\endcsname{0.13}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/inpaint-lama\endcsname{0.30}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/inpaint-telea\endcsname{0.24}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/recolor\endcsname{0.18}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/splice\endcsname{0.09}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/pair@1e-07/type/textreplace\endcsname{0.06}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/post/crop90\endcsname{0.42}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/post/jpeg75\endcsname{0.56}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/post/none\endcsname{0.54}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/post/resize0.75_jpeg80\endcsname{0.55}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/area/0.01\endcsname{0.43}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/area/0.03\endcsname{0.22}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/area/0.1\endcsname{0.06}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/post/crop90\endcsname{0.07}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/post/jpeg75\endcsname{0.23}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/post/none\endcsname{0.21}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/post/resize0.75_jpeg80\endcsname{0.22}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/tpr\endcsname{0.181}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/copymove\endcsname{0.14}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/inpaint-lama\endcsname{0.32}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/inpaint-telea\endcsname{0.26}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/recolor\endcsname{0.21}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/splice\endcsname{0.10}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/query@0.01/type/textreplace\endcsname{0.07}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/copymove\endcsname{0.52}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/inpaint-lama\endcsname{0.61}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/inpaint-telea\endcsname{0.62}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/recolor\endcsname{0.56}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/splice\endcsname{0.41}
\expandafter\def\csname val@fp:editret/ISCC-Image-256/type/textreplace\endcsname{0.38}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/R@1\endcsname{0.502}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/area/0.01\endcsname{0.80}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/area/0.03\endcsname{0.65}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/area/0.1\endcsname{0.39}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/area/0.25\endcsname{0.17}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/area/0.01\endcsname{0.33}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/area/0.03\endcsname{0.15}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/area/0.1\endcsname{0.03}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/post/crop90\endcsname{0.04}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/post/jpeg75\endcsname{0.17}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/post/none\endcsname{0.16}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.15}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/tpr\endcsname{0.130}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/copymove\endcsname{0.10}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/inpaint-lama\endcsname{0.25}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/inpaint-telea\endcsname{0.19}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/recolor\endcsname{0.14}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/splice\endcsname{0.06}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/pair@1e-07/type/textreplace\endcsname{0.04}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/post/crop90\endcsname{0.41}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/post/jpeg75\endcsname{0.53}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/post/none\endcsname{0.53}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/post/resize0.75_jpeg80\endcsname{0.54}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/area/0.01\endcsname{0.33}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/area/0.03\endcsname{0.15}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/area/0.1\endcsname{0.03}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/post/crop90\endcsname{0.04}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/post/jpeg75\endcsname{0.17}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/post/none\endcsname{0.16}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/post/resize0.75_jpeg80\endcsname{0.15}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/tpr\endcsname{0.130}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/copymove\endcsname{0.10}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/inpaint-lama\endcsname{0.25}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/inpaint-telea\endcsname{0.19}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/recolor\endcsname{0.14}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/splice\endcsname{0.06}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/query@0.01/type/textreplace\endcsname{0.04}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/copymove\endcsname{0.51}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/inpaint-lama\endcsname{0.60}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/inpaint-telea\endcsname{0.63}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/recolor\endcsname{0.53}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/splice\endcsname{0.39}
\expandafter\def\csname val@fp:editret/ISCC-Image-64/type/textreplace\endcsname{0.35}
\expandafter\def\csname val@fp:editret/MarrHildreth/R@1\endcsname{0.803}
\expandafter\def\csname val@fp:editret/MarrHildreth/area/0.01\endcsname{0.87}
\expandafter\def\csname val@fp:editret/MarrHildreth/area/0.03\endcsname{0.85}
\expandafter\def\csname val@fp:editret/MarrHildreth/area/0.1\endcsname{0.81}
\expandafter\def\csname val@fp:editret/MarrHildreth/area/0.25\endcsname{0.69}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/area/0.01\endcsname{0.32}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/area/0.03\endcsname{0.24}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/area/0.1\endcsname{0.07}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/post/jpeg75\endcsname{0.22}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/post/none\endcsname{0.24}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.18}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/tpr\endcsname{0.160}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/copymove\endcsname{0.13}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/inpaint-lama\endcsname{0.22}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/inpaint-telea\endcsname{0.21}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/recolor\endcsname{0.18}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/splice\endcsname{0.12}
\expandafter\def\csname val@fp:editret/MarrHildreth/pair@1e-07/type/textreplace\endcsname{0.10}
\expandafter\def\csname val@fp:editret/MarrHildreth/post/crop90\endcsname{0.52}
\expandafter\def\csname val@fp:editret/MarrHildreth/post/jpeg75\endcsname{0.89}
\expandafter\def\csname val@fp:editret/MarrHildreth/post/none\endcsname{0.90}
\expandafter\def\csname val@fp:editret/MarrHildreth/post/resize0.75_jpeg80\endcsname{0.90}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/area/0.01\endcsname{0.43}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/area/0.03\endcsname{0.35}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/area/0.1\endcsname{0.12}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/post/jpeg75\endcsname{0.31}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/post/none\endcsname{0.34}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/post/resize0.75_jpeg80\endcsname{0.27}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/tpr\endcsname{0.231}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/copymove\endcsname{0.19}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/inpaint-lama\endcsname{0.29}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/inpaint-telea\endcsname{0.28}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/recolor\endcsname{0.27}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/splice\endcsname{0.19}
\expandafter\def\csname val@fp:editret/MarrHildreth/query@0.01/type/textreplace\endcsname{0.16}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/copymove\endcsname{0.78}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/inpaint-lama\endcsname{0.83}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/inpaint-telea\endcsname{0.84}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/recolor\endcsname{0.84}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/splice\endcsname{0.78}
\expandafter\def\csname val@fp:editret/MarrHildreth/type/textreplace\endcsname{0.74}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/R@1\endcsname{0.933}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/area/0.03\endcsname{0.99}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/area/0.1\endcsname{0.95}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/area/0.25\endcsname{0.80}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/area/0.01\endcsname{0.61}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/area/0.03\endcsname{0.43}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/area/0.1\endcsname{0.18}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/area/0.25\endcsname{0.03}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/post/crop90\endcsname{0.14}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/post/jpeg75\endcsname{0.39}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/post/none\endcsname{0.42}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.31}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/tpr\endcsname{0.314}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/copymove\endcsname{0.40}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/inpaint-lama\endcsname{0.51}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/inpaint-telea\endcsname{0.45}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/recolor\endcsname{0.21}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/splice\endcsname{0.23}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/pair@1e-07/type/textreplace\endcsname{0.09}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/post/crop90\endcsname{0.91}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/post/jpeg75\endcsname{0.93}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/post/none\endcsname{0.95}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/post/resize0.75_jpeg80\endcsname{0.94}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/area/0.01\endcsname{0.70}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/area/0.03\endcsname{0.52}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/area/0.1\endcsname{0.24}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/area/0.25\endcsname{0.06}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/post/crop90\endcsname{0.21}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/post/jpeg75\endcsname{0.44}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/post/none\endcsname{0.48}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/post/resize0.75_jpeg80\endcsname{0.38}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/tpr\endcsname{0.379}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/copymove\endcsname{0.48}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/inpaint-lama\endcsname{0.57}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/inpaint-telea\endcsname{0.52}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/recolor\endcsname{0.28}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/splice\endcsname{0.30}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/query@0.01/type/textreplace\endcsname{0.13}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/copymove\endcsname{0.95}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/inpaint-lama\endcsname{0.94}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/inpaint-telea\endcsname{0.94}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/recolor\endcsname{0.97}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/splice\endcsname{0.89}
\expandafter\def\csname val@fp:editret/OpenCLIP-B32/type/textreplace\endcsname{0.90}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/R@1\endcsname{0.710}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/area/0.01\endcsname{0.80}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/area/0.03\endcsname{0.77}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/area/0.1\endcsname{0.69}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/area/0.25\endcsname{0.58}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/area/0.01\endcsname{0.55}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/area/0.03\endcsname{0.41}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/area/0.1\endcsname{0.22}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/area/0.25\endcsname{0.09}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/post/jpeg75\endcsname{0.42}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/post/none\endcsname{0.42}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.43}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/tpr\endcsname{0.317}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/copymove\endcsname{0.22}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/inpaint-lama\endcsname{0.47}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/inpaint-telea\endcsname{0.37}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/recolor\endcsname{0.50}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/splice\endcsname{0.16}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/pair@1e-07/type/textreplace\endcsname{0.18}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/post/crop90\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/post/jpeg75\endcsname{0.86}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/post/none\endcsname{0.87}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/post/resize0.75_jpeg80\endcsname{0.87}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/area/0.01\endcsname{0.57}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/area/0.03\endcsname{0.42}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/area/0.1\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/area/0.25\endcsname{0.09}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/post/jpeg75\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/post/none\endcsname{0.45}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/post/resize0.75_jpeg80\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/tpr\endcsname{0.333}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/copymove\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/inpaint-lama\endcsname{0.48}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/inpaint-telea\endcsname{0.39}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/recolor\endcsname{0.51}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/splice\endcsname{0.18}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/query@0.01/type/textreplace\endcsname{0.19}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/copymove\endcsname{0.69}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/inpaint-lama\endcsname{0.78}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/inpaint-telea\endcsname{0.75}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/recolor\endcsname{0.80}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/splice\endcsname{0.59}
\expandafter\def\csname val@fp:editret/PDQ-dihedral/type/textreplace\endcsname{0.65}
\expandafter\def\csname val@fp:editret/PDQ/R@1\endcsname{0.746}
\expandafter\def\csname val@fp:editret/PDQ/area/0.01\endcsname{0.82}
\expandafter\def\csname val@fp:editret/PDQ/area/0.03\endcsname{0.80}
\expandafter\def\csname val@fp:editret/PDQ/area/0.1\endcsname{0.73}
\expandafter\def\csname val@fp:editret/PDQ/area/0.25\endcsname{0.63}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/area/0.01\endcsname{0.57}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/area/0.03\endcsname{0.42}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/area/0.1\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/area/0.25\endcsname{0.09}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/post/jpeg75\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/post/none\endcsname{0.45}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/tpr\endcsname{0.333}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/copymove\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/inpaint-lama\endcsname{0.48}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/inpaint-telea\endcsname{0.39}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/recolor\endcsname{0.51}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/splice\endcsname{0.18}
\expandafter\def\csname val@fp:editret/PDQ/pair@1e-07/type/textreplace\endcsname{0.19}
\expandafter\def\csname val@fp:editret/PDQ/post/crop90\endcsname{0.30}
\expandafter\def\csname val@fp:editret/PDQ/post/jpeg75\endcsname{0.88}
\expandafter\def\csname val@fp:editret/PDQ/post/none\endcsname{0.90}
\expandafter\def\csname val@fp:editret/PDQ/post/resize0.75_jpeg80\endcsname{0.90}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/area/0.01\endcsname{0.57}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/area/0.03\endcsname{0.42}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/area/0.1\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/area/0.25\endcsname{0.09}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/post/jpeg75\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/post/none\endcsname{0.45}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/post/resize0.75_jpeg80\endcsname{0.44}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/tpr\endcsname{0.333}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/copymove\endcsname{0.24}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/inpaint-lama\endcsname{0.48}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/inpaint-telea\endcsname{0.39}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/recolor\endcsname{0.51}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/splice\endcsname{0.18}
\expandafter\def\csname val@fp:editret/PDQ/query@0.01/type/textreplace\endcsname{0.19}
\expandafter\def\csname val@fp:editret/PDQ/type/copymove\endcsname{0.74}
\expandafter\def\csname val@fp:editret/PDQ/type/inpaint-lama\endcsname{0.80}
\expandafter\def\csname val@fp:editret/PDQ/type/inpaint-telea\endcsname{0.78}
\expandafter\def\csname val@fp:editret/PDQ/type/recolor\endcsname{0.82}
\expandafter\def\csname val@fp:editret/PDQ/type/splice\endcsname{0.63}
\expandafter\def\csname val@fp:editret/PDQ/type/textreplace\endcsname{0.71}
\expandafter\def\csname val@fp:editret/SSCD-large/R@1\endcsname{0.983}
\expandafter\def\csname val@fp:editret/SSCD-large/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/area/0.03\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/area/0.1\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/area/0.25\endcsname{0.96}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/area/0.01\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/area/0.03\endcsname{0.89}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/area/0.1\endcsname{0.57}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/area/0.25\endcsname{0.20}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/post/crop90\endcsname{0.61}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/post/jpeg75\endcsname{0.69}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/post/none\endcsname{0.70}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.64}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/tpr\endcsname{0.659}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/copymove\endcsname{0.75}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/inpaint-lama\endcsname{0.71}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/inpaint-telea\endcsname{0.69}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/recolor\endcsname{0.79}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/splice\endcsname{0.54}
\expandafter\def\csname val@fp:editret/SSCD-large/pair@1e-07/type/textreplace\endcsname{0.48}
\expandafter\def\csname val@fp:editret/SSCD-large/post/crop90\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/post/jpeg75\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-large/post/none\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/post/resize0.75_jpeg80\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/area/0.03\endcsname{0.95}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/area/0.1\endcsname{0.72}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/area/0.25\endcsname{0.32}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/post/crop90\endcsname{0.71}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/post/jpeg75\endcsname{0.76}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/post/none\endcsname{0.79}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/post/resize0.75_jpeg80\endcsname{0.73}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/tpr\endcsname{0.747}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/copymove\endcsname{0.86}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/inpaint-lama\endcsname{0.77}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/inpaint-telea\endcsname{0.78}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/recolor\endcsname{0.88}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/splice\endcsname{0.62}
\expandafter\def\csname val@fp:editret/SSCD-large/query@0.01/type/textreplace\endcsname{0.58}
\expandafter\def\csname val@fp:editret/SSCD-large/type/copymove\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/type/inpaint-lama\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/type/inpaint-telea\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/type/recolor\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-large/type/splice\endcsname{0.97}
\expandafter\def\csname val@fp:editret/SSCD-large/type/textreplace\endcsname{0.96}
\expandafter\def\csname val@fp:editret/SSCD-mixup/R@1\endcsname{0.979}
\expandafter\def\csname val@fp:editret/SSCD-mixup/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/area/0.03\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/area/0.1\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/area/0.25\endcsname{0.94}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/area/0.01\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/area/0.03\endcsname{0.92}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/area/0.1\endcsname{0.64}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/area/0.25\endcsname{0.29}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/post/crop90\endcsname{0.63}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/post/jpeg75\endcsname{0.74}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/post/none\endcsname{0.74}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.73}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/tpr\endcsname{0.712}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/copymove\endcsname{0.84}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/inpaint-lama\endcsname{0.74}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/inpaint-telea\endcsname{0.71}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/recolor\endcsname{0.86}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/splice\endcsname{0.58}
\expandafter\def\csname val@fp:editret/SSCD-mixup/pair@1e-07/type/textreplace\endcsname{0.52}
\expandafter\def\csname val@fp:editret/SSCD-mixup/post/crop90\endcsname{0.97}
\expandafter\def\csname val@fp:editret/SSCD-mixup/post/jpeg75\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-mixup/post/none\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/post/resize0.75_jpeg80\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/area/0.01\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/area/0.03\endcsname{0.94}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/area/0.1\endcsname{0.67}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/area/0.25\endcsname{0.33}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/post/crop90\endcsname{0.66}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/post/jpeg75\endcsname{0.76}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/post/none\endcsname{0.76}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/post/resize0.75_jpeg80\endcsname{0.75}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/tpr\endcsname{0.732}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/copymove\endcsname{0.86}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/inpaint-lama\endcsname{0.76}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/inpaint-telea\endcsname{0.73}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/recolor\endcsname{0.89}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/splice\endcsname{0.60}
\expandafter\def\csname val@fp:editret/SSCD-mixup/query@0.01/type/textreplace\endcsname{0.55}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/copymove\endcsname{0.99}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/inpaint-lama\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/inpaint-telea\endcsname{0.98}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/recolor\endcsname{1.00}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/splice\endcsname{0.95}
\expandafter\def\csname val@fp:editret/SSCD-mixup/type/textreplace\endcsname{0.97}
\expandafter\def\csname val@fp:editret/aHash-64/R@1\endcsname{0.535}
\expandafter\def\csname val@fp:editret/aHash-64/area/0.01\endcsname{0.74}
\expandafter\def\csname val@fp:editret/aHash-64/area/0.03\endcsname{0.67}
\expandafter\def\csname val@fp:editret/aHash-64/area/0.1\endcsname{0.49}
\expandafter\def\csname val@fp:editret/aHash-64/area/0.25\endcsname{0.24}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/post/crop90\endcsname{0.28}
\expandafter\def\csname val@fp:editret/aHash-64/post/jpeg75\endcsname{0.62}
\expandafter\def\csname val@fp:editret/aHash-64/post/none\endcsname{0.61}
\expandafter\def\csname val@fp:editret/aHash-64/post/resize0.75_jpeg80\endcsname{0.62}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/query@0.01/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/aHash-64/type/copymove\endcsname{0.55}
\expandafter\def\csname val@fp:editret/aHash-64/type/inpaint-lama\endcsname{0.64}
\expandafter\def\csname val@fp:editret/aHash-64/type/inpaint-telea\endcsname{0.65}
\expandafter\def\csname val@fp:editret/aHash-64/type/recolor\endcsname{0.54}
\expandafter\def\csname val@fp:editret/aHash-64/type/splice\endcsname{0.46}
\expandafter\def\csname val@fp:editret/aHash-64/type/textreplace\endcsname{0.36}
\expandafter\def\csname val@fp:editret/dHash-64/R@1\endcsname{0.712}
\expandafter\def\csname val@fp:editret/dHash-64/area/0.01\endcsname{0.85}
\expandafter\def\csname val@fp:editret/dHash-64/area/0.03\endcsname{0.82}
\expandafter\def\csname val@fp:editret/dHash-64/area/0.1\endcsname{0.72}
\expandafter\def\csname val@fp:editret/dHash-64/area/0.25\endcsname{0.46}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/post/crop90\endcsname{0.36}
\expandafter\def\csname val@fp:editret/dHash-64/post/jpeg75\endcsname{0.83}
\expandafter\def\csname val@fp:editret/dHash-64/post/none\endcsname{0.83}
\expandafter\def\csname val@fp:editret/dHash-64/post/resize0.75_jpeg80\endcsname{0.83}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/area/0.01\endcsname{0.36}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/area/0.03\endcsname{0.19}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/area/0.1\endcsname{0.05}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/area/0.25\endcsname{0.01}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/post/jpeg75\endcsname{0.20}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/post/none\endcsname{0.20}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/post/resize0.75_jpeg80\endcsname{0.19}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/tpr\endcsname{0.149}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/copymove\endcsname{0.11}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/inpaint-lama\endcsname{0.27}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/inpaint-telea\endcsname{0.22}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/recolor\endcsname{0.17}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/splice\endcsname{0.07}
\expandafter\def\csname val@fp:editret/dHash-64/query@0.01/type/textreplace\endcsname{0.06}
\expandafter\def\csname val@fp:editret/dHash-64/type/copymove\endcsname{0.68}
\expandafter\def\csname val@fp:editret/dHash-64/type/inpaint-lama\endcsname{0.80}
\expandafter\def\csname val@fp:editret/dHash-64/type/inpaint-telea\endcsname{0.79}
\expandafter\def\csname val@fp:editret/dHash-64/type/recolor\endcsname{0.76}
\expandafter\def\csname val@fp:editret/dHash-64/type/splice\endcsname{0.64}
\expandafter\def\csname val@fp:editret/dHash-64/type/textreplace\endcsname{0.60}
\expandafter\def\csname val@fp:editret/pHash-256/R@1\endcsname{0.758}
\expandafter\def\csname val@fp:editret/pHash-256/area/0.01\endcsname{0.85}
\expandafter\def\csname val@fp:editret/pHash-256/area/0.03\endcsname{0.83}
\expandafter\def\csname val@fp:editret/pHash-256/area/0.1\endcsname{0.74}
\expandafter\def\csname val@fp:editret/pHash-256/area/0.25\endcsname{0.61}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/area/0.01\endcsname{0.55}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/area/0.03\endcsname{0.40}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/area/0.1\endcsname{0.21}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/area/0.25\endcsname{0.08}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/post/jpeg75\endcsname{0.41}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/post/none\endcsname{0.41}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.42}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/tpr\endcsname{0.311}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/copymove\endcsname{0.23}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/inpaint-lama\endcsname{0.47}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/inpaint-telea\endcsname{0.37}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/recolor\endcsname{0.47}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/splice\endcsname{0.16}
\expandafter\def\csname val@fp:editret/pHash-256/pair@1e-07/type/textreplace\endcsname{0.16}
\expandafter\def\csname val@fp:editret/pHash-256/post/crop90\endcsname{0.39}
\expandafter\def\csname val@fp:editret/pHash-256/post/jpeg75\endcsname{0.87}
\expandafter\def\csname val@fp:editret/pHash-256/post/none\endcsname{0.88}
\expandafter\def\csname val@fp:editret/pHash-256/post/resize0.75_jpeg80\endcsname{0.89}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/area/0.01\endcsname{0.57}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/area/0.03\endcsname{0.42}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/area/0.1\endcsname{0.23}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/area/0.25\endcsname{0.09}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/post/jpeg75\endcsname{0.44}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/post/none\endcsname{0.44}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/post/resize0.75_jpeg80\endcsname{0.43}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/tpr\endcsname{0.328}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/copymove\endcsname{0.25}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/inpaint-lama\endcsname{0.48}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/inpaint-telea\endcsname{0.39}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/recolor\endcsname{0.49}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/splice\endcsname{0.18}
\expandafter\def\csname val@fp:editret/pHash-256/query@0.01/type/textreplace\endcsname{0.18}
\expandafter\def\csname val@fp:editret/pHash-256/type/copymove\endcsname{0.76}
\expandafter\def\csname val@fp:editret/pHash-256/type/inpaint-lama\endcsname{0.82}
\expandafter\def\csname val@fp:editret/pHash-256/type/inpaint-telea\endcsname{0.80}
\expandafter\def\csname val@fp:editret/pHash-256/type/recolor\endcsname{0.84}
\expandafter\def\csname val@fp:editret/pHash-256/type/splice\endcsname{0.65}
\expandafter\def\csname val@fp:editret/pHash-256/type/textreplace\endcsname{0.69}
\expandafter\def\csname val@fp:editret/pHash-64/R@1\endcsname{0.529}
\expandafter\def\csname val@fp:editret/pHash-64/area/0.01\endcsname{0.76}
\expandafter\def\csname val@fp:editret/pHash-64/area/0.03\endcsname{0.65}
\expandafter\def\csname val@fp:editret/pHash-64/area/0.1\endcsname{0.45}
\expandafter\def\csname val@fp:editret/pHash-64/area/0.25\endcsname{0.25}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/area/0.01\endcsname{0.23}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/area/0.03\endcsname{0.08}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/area/0.1\endcsname{0.02}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/post/jpeg75\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/post/none\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/tpr\endcsname{0.085}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/copymove\endcsname{0.05}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/inpaint-lama\endcsname{0.21}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/inpaint-telea\endcsname{0.14}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/recolor\endcsname{0.08}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/splice\endcsname{0.03}
\expandafter\def\csname val@fp:editret/pHash-64/pair@1e-07/type/textreplace\endcsname{0.01}
\expandafter\def\csname val@fp:editret/pHash-64/post/crop90\endcsname{0.32}
\expandafter\def\csname val@fp:editret/pHash-64/post/jpeg75\endcsname{0.60}
\expandafter\def\csname val@fp:editret/pHash-64/post/none\endcsname{0.60}
\expandafter\def\csname val@fp:editret/pHash-64/post/resize0.75_jpeg80\endcsname{0.61}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/area/0.01\endcsname{0.23}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/area/0.03\endcsname{0.08}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/area/0.1\endcsname{0.02}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/post/jpeg75\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/post/none\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/post/resize0.75_jpeg80\endcsname{0.11}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/tpr\endcsname{0.085}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/copymove\endcsname{0.05}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/inpaint-lama\endcsname{0.21}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/inpaint-telea\endcsname{0.14}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/recolor\endcsname{0.08}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/splice\endcsname{0.03}
\expandafter\def\csname val@fp:editret/pHash-64/query@0.01/type/textreplace\endcsname{0.01}
\expandafter\def\csname val@fp:editret/pHash-64/type/copymove\endcsname{0.49}
\expandafter\def\csname val@fp:editret/pHash-64/type/inpaint-lama\endcsname{0.67}
\expandafter\def\csname val@fp:editret/pHash-64/type/inpaint-telea\endcsname{0.65}
\expandafter\def\csname val@fp:editret/pHash-64/type/recolor\endcsname{0.65}
\expandafter\def\csname val@fp:editret/pHash-64/type/splice\endcsname{0.37}
\expandafter\def\csname val@fp:editret/pHash-64/type/textreplace\endcsname{0.35}
\expandafter\def\csname val@fp:editret/wHash-64/R@1\endcsname{0.436}
\expandafter\def\csname val@fp:editret/wHash-64/area/0.01\endcsname{0.59}
\expandafter\def\csname val@fp:editret/wHash-64/area/0.03\endcsname{0.55}
\expandafter\def\csname val@fp:editret/wHash-64/area/0.1\endcsname{0.42}
\expandafter\def\csname val@fp:editret/wHash-64/area/0.25\endcsname{0.18}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/pair@1e-07/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/post/crop90\endcsname{0.23}
\expandafter\def\csname val@fp:editret/wHash-64/post/jpeg75\endcsname{0.51}
\expandafter\def\csname val@fp:editret/wHash-64/post/none\endcsname{0.53}
\expandafter\def\csname val@fp:editret/wHash-64/post/resize0.75_jpeg80\endcsname{0.48}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/area/0.01\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/area/0.03\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/area/0.1\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/area/0.25\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/post/crop90\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/post/jpeg75\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/post/none\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/post/resize0.75_jpeg80\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/tpr\endcsname{0.000}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/copymove\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/inpaint-lama\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/inpaint-telea\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/recolor\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/splice\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/query@0.01/type/textreplace\endcsname{0.00}
\expandafter\def\csname val@fp:editret/wHash-64/type/copymove\endcsname{0.45}
\expandafter\def\csname val@fp:editret/wHash-64/type/inpaint-lama\endcsname{0.50}
\expandafter\def\csname val@fp:editret/wHash-64/type/inpaint-telea\endcsname{0.51}
\expandafter\def\csname val@fp:editret/wHash-64/type/recolor\endcsname{0.43}
\expandafter\def\csname val@fp:editret/wHash-64/type/splice\endcsname{0.40}
\expandafter\def\csname val@fp:editret/wHash-64/type/textreplace\endcsname{0.34}
\expandafter\def\csname val@fp:image/BlockMean/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/BlockMean/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/BlockMean/FPRq@query@0.01\endcsname{0.009}
\expandafter\def\csname val@fp:image/BlockMean/FPRq@query@0.01/pct\endcsname{0.9}
\expandafter\def\csname val@fp:image/BlockMean/R@1\endcsname{0.562}
\expandafter\def\csname val@fp:image/BlockMean/R@1/pct\endcsname{56.2}
\expandafter\def\csname val@fp:image/BlockMean/R@10\endcsname{0.619}
\expandafter\def\csname val@fp:image/BlockMean/R@10/pct\endcsname{61.9}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@0.0001\endcsname{0.507}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@0.0001/pct\endcsname{50.7}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-05\endcsname{0.463}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-05/pct\endcsname{46.3}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-06\endcsname{0.337}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-06/pct\endcsname{33.7}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/BlockMean/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/BlockMean/TPR@query@0.01\endcsname{0.337}
\expandafter\def\csname val@fp:image/BlockMean/TPR@query@0.01/pct\endcsname{33.7}
\expandafter\def\csname val@fp:image/BlockMean/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/blur2\endcsname{0.96}
\expandafter\def\csname val@fp:image/BlockMean/att/blur2/pct\endcsname{96}
\expandafter\def\csname val@fp:image/BlockMean/att/bright0.6\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/bright0.6/pct\endcsname{98}
\expandafter\def\csname val@fp:image/BlockMean/att/bright1.4\endcsname{0.70}
\expandafter\def\csname val@fp:image/BlockMean/att/bright1.4/pct\endcsname{70}
\expandafter\def\csname val@fp:image/BlockMean/att/contrast0.5\endcsname{0.98}
\expandafter\def\csname val@fp:image/BlockMean/att/contrast0.5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/BlockMean/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/crop70\endcsname{0.01}
\expandafter\def\csname val@fp:image/BlockMean/att/crop70/pct\endcsname{1}
\expandafter\def\csname val@fp:image/BlockMean/att/crop90\endcsname{0.45}
\expandafter\def\csname val@fp:image/BlockMean/att/crop90/pct\endcsname{45}
\expandafter\def\csname val@fp:image/BlockMean/att/emoji0.3\endcsname{0.85}
\expandafter\def\csname val@fp:image/BlockMean/att/emoji0.3/pct\endcsname{85}
\expandafter\def\csname val@fp:image/BlockMean/att/gamma0.6\endcsname{0.94}
\expandafter\def\csname val@fp:image/BlockMean/att/gamma0.6/pct\endcsname{94}
\expandafter\def\csname val@fp:image/BlockMean/att/gray\endcsname{0.98}
\expandafter\def\csname val@fp:image/BlockMean/att/gray/pct\endcsname{98}
\expandafter\def\csname val@fp:image/BlockMean/att/hflip\endcsname{0.17}
\expandafter\def\csname val@fp:image/BlockMean/att/hflip/pct\endcsname{17}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg30\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg30/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg50\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg50/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg75\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/jpeg75/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/att/meme\endcsname{0.08}
\expandafter\def\csname val@fp:image/BlockMean/att/meme/pct\endcsname{8}
\expandafter\def\csname val@fp:image/BlockMean/att/noise0.05\endcsname{0.96}
\expandafter\def\csname val@fp:image/BlockMean/att/noise0.05/pct\endcsname{96}
\expandafter\def\csname val@fp:image/BlockMean/att/none\endcsname{0.98}
\expandafter\def\csname val@fp:image/BlockMean/att/none/pct\endcsname{98}
\expandafter\def\csname val@fp:image/BlockMean/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/perspective\endcsname{0.34}
\expandafter\def\csname val@fp:image/BlockMean/att/perspective/pct\endcsname{34}
\expandafter\def\csname val@fp:image/BlockMean/att/pixelize0.3\endcsname{0.96}
\expandafter\def\csname val@fp:image/BlockMean/att/pixelize0.3/pct\endcsname{96}
\expandafter\def\csname val@fp:image/BlockMean/att/recapture\endcsname{0.56}
\expandafter\def\csname val@fp:image/BlockMean/att/recapture/pct\endcsname{56}
\expandafter\def\csname val@fp:image/BlockMean/att/resize0.25\endcsname{0.96}
\expandafter\def\csname val@fp:image/BlockMean/att/resize0.25/pct\endcsname{96}
\expandafter\def\csname val@fp:image/BlockMean/att/resize0.5\endcsname{0.96}
\expandafter\def\csname val@fp:image/BlockMean/att/resize0.5/pct\endcsname{96}
\expandafter\def\csname val@fp:image/BlockMean/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/rot5\endcsname{0.05}
\expandafter\def\csname val@fp:image/BlockMean/att/rot5/pct\endcsname{5}
\expandafter\def\csname val@fp:image/BlockMean/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/sat2\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/sat2/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/BlockMean/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/BlockMean/att/skew\endcsname{0.12}
\expandafter\def\csname val@fp:image/BlockMean/att/skew/pct\endcsname{12}
\expandafter\def\csname val@fp:image/BlockMean/att/social\endcsname{0.45}
\expandafter\def\csname val@fp:image/BlockMean/att/social/pct\endcsname{45}
\expandafter\def\csname val@fp:image/BlockMean/att/squash0.75\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/squash0.75/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/att/text\endcsname{0.93}
\expandafter\def\csname val@fp:image/BlockMean/att/text/pct\endcsname{93}
\expandafter\def\csname val@fp:image/BlockMean/att/webp50\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/att/webp50/pct\endcsname{97}
\expandafter\def\csname val@fp:image/BlockMean/bits\endcsname{256}
\expandafter\def\csname val@fp:image/BlockMean/disc\endcsname{0.069}
\expandafter\def\csname val@fp:image/BlockMean/fam/chain\endcsname{0.50}
\expandafter\def\csname val@fp:image/BlockMean/fam/compression\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/fam/crop\endcsname{0.09}
\expandafter\def\csname val@fp:image/BlockMean/fam/geometric\endcsname{0.10}
\expandafter\def\csname val@fp:image/BlockMean/fam/none\endcsname{0.98}
\expandafter\def\csname val@fp:image/BlockMean/fam/overlay\endcsname{0.37}
\expandafter\def\csname val@fp:image/BlockMean/fam/photometric\endcsname{0.94}
\expandafter\def\csname val@fp:image/BlockMean/fam/scale\endcsname{0.97}
\expandafter\def\csname val@fp:image/BlockMean/hard\endcsname{0.001}
\expandafter\def\csname val@fp:image/BlockMean/hard/pct\endcsname{0.1}
\expandafter\def\csname val@fp:image/BlockMean/ms\endcsname{1.0}
\expandafter\def\csname val@fp:image/BlockMean/muAP\endcsname{0.338}
\expandafter\def\csname val@fp:image/BlockMean/muAP/pct\endcsname{33.8}
\expandafter\def\csname val@fp:image/Blockhash-256/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/FPRq@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/FPRq@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/R@1\endcsname{0.560}
\expandafter\def\csname val@fp:image/Blockhash-256/R@1/pct\endcsname{56.0}
\expandafter\def\csname val@fp:image/Blockhash-256/R@10\endcsname{0.618}
\expandafter\def\csname val@fp:image/Blockhash-256/R@10/pct\endcsname{61.8}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@0.0001\endcsname{0.493}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@0.0001/pct\endcsname{49.3}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-05\endcsname{0.401}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-05/pct\endcsname{40.1}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-06\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-06/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/TPR@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/blur2\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/blur2/pct\endcsname{93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/bright0.6\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/bright0.6/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/bright1.4\endcsname{0.77}
\expandafter\def\csname val@fp:image/Blockhash-256/att/bright1.4/pct\endcsname{77}
\expandafter\def\csname val@fp:image/Blockhash-256/att/contrast0.5\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/contrast0.5/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop70\endcsname{0.01}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop70/pct\endcsname{1}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop90\endcsname{0.58}
\expandafter\def\csname val@fp:image/Blockhash-256/att/crop90/pct\endcsname{58}
\expandafter\def\csname val@fp:image/Blockhash-256/att/emoji0.3\endcsname{0.90}
\expandafter\def\csname val@fp:image/Blockhash-256/att/emoji0.3/pct\endcsname{90}
\expandafter\def\csname val@fp:image/Blockhash-256/att/gamma0.6\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/gamma0.6/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/gray\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/gray/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/hflip\endcsname{0.13}
\expandafter\def\csname val@fp:image/Blockhash-256/att/hflip/pct\endcsname{13}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg30\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg30/pct\endcsname{93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg50\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg50/pct\endcsname{93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg75\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/jpeg75/pct\endcsname{93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/meme\endcsname{0.15}
\expandafter\def\csname val@fp:image/Blockhash-256/att/meme/pct\endcsname{15}
\expandafter\def\csname val@fp:image/Blockhash-256/att/noise0.05\endcsname{0.88}
\expandafter\def\csname val@fp:image/Blockhash-256/att/noise0.05/pct\endcsname{88}
\expandafter\def\csname val@fp:image/Blockhash-256/att/none\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/none/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/perspective\endcsname{0.39}
\expandafter\def\csname val@fp:image/Blockhash-256/att/perspective/pct\endcsname{39}
\expandafter\def\csname val@fp:image/Blockhash-256/att/pixelize0.3\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/pixelize0.3/pct\endcsname{93}
\expandafter\def\csname val@fp:image/Blockhash-256/att/recapture\endcsname{0.55}
\expandafter\def\csname val@fp:image/Blockhash-256/att/recapture/pct\endcsname{55}
\expandafter\def\csname val@fp:image/Blockhash-256/att/resize0.25\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/resize0.25/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/resize0.5\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/resize0.5/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot5\endcsname{0.05}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot5/pct\endcsname{5}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/sat2\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/sat2/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/Blockhash-256/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/Blockhash-256/att/skew\endcsname{0.24}
\expandafter\def\csname val@fp:image/Blockhash-256/att/skew/pct\endcsname{24}
\expandafter\def\csname val@fp:image/Blockhash-256/att/social\endcsname{0.55}
\expandafter\def\csname val@fp:image/Blockhash-256/att/social/pct\endcsname{55}
\expandafter\def\csname val@fp:image/Blockhash-256/att/squash0.75\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/squash0.75/pct\endcsname{94}
\expandafter\def\csname val@fp:image/Blockhash-256/att/text\endcsname{0.91}
\expandafter\def\csname val@fp:image/Blockhash-256/att/text/pct\endcsname{91}
\expandafter\def\csname val@fp:image/Blockhash-256/att/webp50\endcsname{0.92}
\expandafter\def\csname val@fp:image/Blockhash-256/att/webp50/pct\endcsname{92}
\expandafter\def\csname val@fp:image/Blockhash-256/bits\endcsname{256}
\expandafter\def\csname val@fp:image/Blockhash-256/disc\endcsname{0.182}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/chain\endcsname{0.55}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/compression\endcsname{0.93}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/crop\endcsname{0.12}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/geometric\endcsname{0.12}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/none\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/overlay\endcsname{0.39}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/photometric\endcsname{0.91}
\expandafter\def\csname val@fp:image/Blockhash-256/fam/scale\endcsname{0.94}
\expandafter\def\csname val@fp:image/Blockhash-256/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/Blockhash-256/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/Blockhash-256/ms\endcsname{19}
\expandafter\def\csname val@fp:image/Blockhash-256/muAP\endcsname{0.250}
\expandafter\def\csname val@fp:image/Blockhash-256/muAP/pct\endcsname{25.0}
\expandafter\def\csname val@fp:image/ColorMoment/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/FPRq@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/FPRq@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/R@1\endcsname{0.281}
\expandafter\def\csname val@fp:image/ColorMoment/R@1/pct\endcsname{28.1}
\expandafter\def\csname val@fp:image/ColorMoment/R@10\endcsname{0.379}
\expandafter\def\csname val@fp:image/ColorMoment/R@10/pct\endcsname{37.9}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@0.0001\endcsname{0.257}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@0.0001/pct\endcsname{25.7}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-05\endcsname{0.104}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-05/pct\endcsname{10.4}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-06\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-06/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/TPR@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ColorMoment/att/blur2\endcsname{0.40}
\expandafter\def\csname val@fp:image/ColorMoment/att/blur2/pct\endcsname{40}
\expandafter\def\csname val@fp:image/ColorMoment/att/bright0.6\endcsname{0.04}
\expandafter\def\csname val@fp:image/ColorMoment/att/bright0.6/pct\endcsname{4}
\expandafter\def\csname val@fp:image/ColorMoment/att/bright1.4\endcsname{0.05}
\expandafter\def\csname val@fp:image/ColorMoment/att/bright1.4/pct\endcsname{5}
\expandafter\def\csname val@fp:image/ColorMoment/att/contrast0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/contrast0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop30\endcsname{0.01}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop30/pct\endcsname{1}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop50\endcsname{0.01}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop50/pct\endcsname{1}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop50off\endcsname{0.01}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop50off/pct\endcsname{2}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop70\endcsname{0.04}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop70/pct\endcsname{4}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop90\endcsname{0.35}
\expandafter\def\csname val@fp:image/ColorMoment/att/crop90/pct\endcsname{35}
\expandafter\def\csname val@fp:image/ColorMoment/att/emoji0.3\endcsname{0.05}
\expandafter\def\csname val@fp:image/ColorMoment/att/emoji0.3/pct\endcsname{5}
\expandafter\def\csname val@fp:image/ColorMoment/att/gamma0.6\endcsname{0.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/gamma0.6/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ColorMoment/att/gray\endcsname{0.02}
\expandafter\def\csname val@fp:image/ColorMoment/att/gray/pct\endcsname{2}
\expandafter\def\csname val@fp:image/ColorMoment/att/hflip\endcsname{1.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/hflip/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg30\endcsname{0.18}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg30/pct\endcsname{18}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg50\endcsname{0.25}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg50/pct\endcsname{25}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg75\endcsname{0.40}
\expandafter\def\csname val@fp:image/ColorMoment/att/jpeg75/pct\endcsname{40}
\expandafter\def\csname val@fp:image/ColorMoment/att/meme\endcsname{0.08}
\expandafter\def\csname val@fp:image/ColorMoment/att/meme/pct\endcsname{8}
\expandafter\def\csname val@fp:image/ColorMoment/att/noise0.05\endcsname{0.06}
\expandafter\def\csname val@fp:image/ColorMoment/att/noise0.05/pct\endcsname{6}
\expandafter\def\csname val@fp:image/ColorMoment/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ColorMoment/att/pad25\endcsname{0.14}
\expandafter\def\csname val@fp:image/ColorMoment/att/pad25/pct\endcsname{14}
\expandafter\def\csname val@fp:image/ColorMoment/att/perspective\endcsname{0.30}
\expandafter\def\csname val@fp:image/ColorMoment/att/perspective/pct\endcsname{30}
\expandafter\def\csname val@fp:image/ColorMoment/att/pixelize0.3\endcsname{0.65}
\expandafter\def\csname val@fp:image/ColorMoment/att/pixelize0.3/pct\endcsname{65}
\expandafter\def\csname val@fp:image/ColorMoment/att/recapture\endcsname{0.02}
\expandafter\def\csname val@fp:image/ColorMoment/att/recapture/pct\endcsname{2}
\expandafter\def\csname val@fp:image/ColorMoment/att/resize0.25\endcsname{0.61}
\expandafter\def\csname val@fp:image/ColorMoment/att/resize0.25/pct\endcsname{61}
\expandafter\def\csname val@fp:image/ColorMoment/att/resize0.5\endcsname{0.87}
\expandafter\def\csname val@fp:image/ColorMoment/att/resize0.5/pct\endcsname{87}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot15\endcsname{0.40}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot15/pct\endcsname{40}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot5\endcsname{0.60}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot5/pct\endcsname{60}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot90\endcsname{1.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/rot90/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ColorMoment/att/sat2\endcsname{0.03}
\expandafter\def\csname val@fp:image/ColorMoment/att/sat2/pct\endcsname{3}
\expandafter\def\csname val@fp:image/ColorMoment/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/ColorMoment/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ColorMoment/att/skew\endcsname{0.11}
\expandafter\def\csname val@fp:image/ColorMoment/att/skew/pct\endcsname{11}
\expandafter\def\csname val@fp:image/ColorMoment/att/social\endcsname{0.09}
\expandafter\def\csname val@fp:image/ColorMoment/att/social/pct\endcsname{9}
\expandafter\def\csname val@fp:image/ColorMoment/att/squash0.75\endcsname{0.96}
\expandafter\def\csname val@fp:image/ColorMoment/att/squash0.75/pct\endcsname{96}
\expandafter\def\csname val@fp:image/ColorMoment/att/text\endcsname{0.13}
\expandafter\def\csname val@fp:image/ColorMoment/att/text/pct\endcsname{13}
\expandafter\def\csname val@fp:image/ColorMoment/att/webp50\endcsname{0.24}
\expandafter\def\csname val@fp:image/ColorMoment/att/webp50/pct\endcsname{24}
\expandafter\def\csname val@fp:image/ColorMoment/bits\endcsname{1344}
\expandafter\def\csname val@fp:image/ColorMoment/disc\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/fam/chain\endcsname{0.06}
\expandafter\def\csname val@fp:image/ColorMoment/fam/compression\endcsname{0.27}
\expandafter\def\csname val@fp:image/ColorMoment/fam/crop\endcsname{0.08}
\expandafter\def\csname val@fp:image/ColorMoment/fam/geometric\endcsname{0.51}
\expandafter\def\csname val@fp:image/ColorMoment/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ColorMoment/fam/overlay\endcsname{0.05}
\expandafter\def\csname val@fp:image/ColorMoment/fam/photometric\endcsname{0.14}
\expandafter\def\csname val@fp:image/ColorMoment/fam/scale\endcsname{0.81}
\expandafter\def\csname val@fp:image/ColorMoment/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/ColorMoment/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ColorMoment/ms\endcsname{3.6}
\expandafter\def\csname val@fp:image/ColorMoment/muAP\endcsname{0.101}
\expandafter\def\csname val@fp:image/ColorMoment/muAP/pct\endcsname{10.1}
\expandafter\def\csname val@fp:image/DINOHash-96/FPRq@pair@1e-07\endcsname{0.002}
\expandafter\def\csname val@fp:image/DINOHash-96/FPRq@pair@1e-07/pct\endcsname{0.2}
\expandafter\def\csname val@fp:image/DINOHash-96/FPRq@query@0.01\endcsname{0.002}
\expandafter\def\csname val@fp:image/DINOHash-96/FPRq@query@0.01/pct\endcsname{0.2}
\expandafter\def\csname val@fp:image/DINOHash-96/R@1\endcsname{0.769}
\expandafter\def\csname val@fp:image/DINOHash-96/R@1/pct\endcsname{76.9}
\expandafter\def\csname val@fp:image/DINOHash-96/R@10\endcsname{0.872}
\expandafter\def\csname val@fp:image/DINOHash-96/R@10/pct\endcsname{87.2}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@0.0001\endcsname{0.733}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@0.0001/pct\endcsname{73.3}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-05\endcsname{0.502}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-05/pct\endcsname{50.2}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-06\endcsname{0.388}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-06/pct\endcsname{38.8}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-07\endcsname{0.237}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-07/pct\endcsname{23.7}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-08\endcsname{0.145}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@pair@1e-08/pct\endcsname{14.5}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@query@0.01\endcsname{0.237}
\expandafter\def\csname val@fp:image/DINOHash-96/TPR@query@0.01/pct\endcsname{23.7}
\expandafter\def\csname val@fp:image/DINOHash-96/att/background0.5\endcsname{0.05}
\expandafter\def\csname val@fp:image/DINOHash-96/att/background0.5/pct\endcsname{5}
\expandafter\def\csname val@fp:image/DINOHash-96/att/blur2\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/blur2/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/bright0.6\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/bright0.6/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/bright1.4\endcsname{0.78}
\expandafter\def\csname val@fp:image/DINOHash-96/att/bright1.4/pct\endcsname{78}
\expandafter\def\csname val@fp:image/DINOHash-96/att/contrast0.5\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOHash-96/att/contrast0.5/pct\endcsname{93}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop30\endcsname{0.12}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop30/pct\endcsname{12}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop50\endcsname{0.39}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop50/pct\endcsname{39}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop50off\endcsname{0.35}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop50off/pct\endcsname{35}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop70\endcsname{0.70}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop70/pct\endcsname{70}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop90\endcsname{0.89}
\expandafter\def\csname val@fp:image/DINOHash-96/att/crop90/pct\endcsname{89}
\expandafter\def\csname val@fp:image/DINOHash-96/att/emoji0.3\endcsname{0.77}
\expandafter\def\csname val@fp:image/DINOHash-96/att/emoji0.3/pct\endcsname{77}
\expandafter\def\csname val@fp:image/DINOHash-96/att/gamma0.6\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOHash-96/att/gamma0.6/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOHash-96/att/gray\endcsname{0.85}
\expandafter\def\csname val@fp:image/DINOHash-96/att/gray/pct\endcsname{85}
\expandafter\def\csname val@fp:image/DINOHash-96/att/hflip\endcsname{0.88}
\expandafter\def\csname val@fp:image/DINOHash-96/att/hflip/pct\endcsname{88}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg30\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg30/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOHash-96/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOHash-96/att/meme\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOHash-96/att/meme/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOHash-96/att/noise0.05\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/noise0.05/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOHash-96/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOHash-96/att/pad25\endcsname{0.74}
\expandafter\def\csname val@fp:image/DINOHash-96/att/pad25/pct\endcsname{74}
\expandafter\def\csname val@fp:image/DINOHash-96/att/perspective\endcsname{0.80}
\expandafter\def\csname val@fp:image/DINOHash-96/att/perspective/pct\endcsname{80}
\expandafter\def\csname val@fp:image/DINOHash-96/att/pixelize0.3\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/pixelize0.3/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOHash-96/att/recapture\endcsname{0.81}
\expandafter\def\csname val@fp:image/DINOHash-96/att/recapture/pct\endcsname{81}
\expandafter\def\csname val@fp:image/DINOHash-96/att/resize0.25\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOHash-96/att/resize0.25/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOHash-96/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOHash-96/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot15\endcsname{0.55}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot15/pct\endcsname{55}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot5\endcsname{0.79}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot5/pct\endcsname{79}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot90\endcsname{0.29}
\expandafter\def\csname val@fp:image/DINOHash-96/att/rot90/pct\endcsname{29}
\expandafter\def\csname val@fp:image/DINOHash-96/att/sat2\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/sat2/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOHash-96/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/DINOHash-96/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/DINOHash-96/att/skew\endcsname{0.57}
\expandafter\def\csname val@fp:image/DINOHash-96/att/skew/pct\endcsname{57}
\expandafter\def\csname val@fp:image/DINOHash-96/att/social\endcsname{0.88}
\expandafter\def\csname val@fp:image/DINOHash-96/att/social/pct\endcsname{88}
\expandafter\def\csname val@fp:image/DINOHash-96/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOHash-96/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOHash-96/att/text\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOHash-96/att/text/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOHash-96/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOHash-96/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOHash-96/bits\endcsname{96.0}
\expandafter\def\csname val@fp:image/DINOHash-96/disc\endcsname{0.212}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/chain\endcsname{0.85}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/crop\endcsname{0.49}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/geometric\endcsname{0.66}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/overlay\endcsname{0.52}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/photometric\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOHash-96/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOHash-96/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/DINOHash-96/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/DINOHash-96/ms\endcsname{3.6}
\expandafter\def\csname val@fp:image/DINOHash-96/muAP\endcsname{0.533}
\expandafter\def\csname val@fp:image/DINOHash-96/muAP/pct\endcsname{53.3}
\expandafter\def\csname val@fp:image/DINOv2-B/FPRq@pair@1e-07\endcsname{0.009}
\expandafter\def\csname val@fp:image/DINOv2-B/FPRq@pair@1e-07/pct\endcsname{0.9}
\expandafter\def\csname val@fp:image/DINOv2-B/FPRq@query@0.01\endcsname{0.012}
\expandafter\def\csname val@fp:image/DINOv2-B/FPRq@query@0.01/pct\endcsname{1.2}
\expandafter\def\csname val@fp:image/DINOv2-B/R@1\endcsname{0.872}
\expandafter\def\csname val@fp:image/DINOv2-B/R@1/pct\endcsname{87.2}
\expandafter\def\csname val@fp:image/DINOv2-B/R@10\endcsname{0.926}
\expandafter\def\csname val@fp:image/DINOv2-B/R@10/pct\endcsname{92.6}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@0.0001\endcsname{0.829}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@0.0001/pct\endcsname{82.9}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-05\endcsname{0.754}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-05/pct\endcsname{75.4}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-06\endcsname{0.685}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-06/pct\endcsname{68.5}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-07\endcsname{0.650}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-07/pct\endcsname{65.0}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-08\endcsname{0.623}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@pair@1e-08/pct\endcsname{62.3}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@query@0.01\endcsname{0.653}
\expandafter\def\csname val@fp:image/DINOv2-B/TPR@query@0.01/pct\endcsname{65.3}
\expandafter\def\csname val@fp:image/DINOv2-B/att/background0.5\endcsname{0.13}
\expandafter\def\csname val@fp:image/DINOv2-B/att/background0.5/pct\endcsname{13}
\expandafter\def\csname val@fp:image/DINOv2-B/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/bright0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/bright1.4\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOv2-B/att/bright1.4/pct\endcsname{93}
\expandafter\def\csname val@fp:image/DINOv2-B/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop30\endcsname{0.29}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop30/pct\endcsname{29}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop50\endcsname{0.62}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop50/pct\endcsname{62}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop50off\endcsname{0.60}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop50off/pct\endcsname{60}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop70\endcsname{0.88}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop70/pct\endcsname{88}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop90\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/crop90/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/emoji0.3\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-B/att/emoji0.3/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOv2-B/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/gray\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/gray/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/hflip/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/meme\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/meme/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-B/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-B/att/pad25\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOv2-B/att/pad25/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOv2-B/att/perspective\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-B/att/perspective/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-B/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/recapture\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-B/att/recapture/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOv2-B/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-B/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot15\endcsname{0.91}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot15/pct\endcsname{91}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot5\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot5/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot90\endcsname{0.60}
\expandafter\def\csname val@fp:image/DINOv2-B/att/rot90/pct\endcsname{60}
\expandafter\def\csname val@fp:image/DINOv2-B/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/screenshot\endcsname{0.03}
\expandafter\def\csname val@fp:image/DINOv2-B/att/screenshot/pct\endcsname{3}
\expandafter\def\csname val@fp:image/DINOv2-B/att/skew\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOv2-B/att/skew/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOv2-B/att/social\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-B/att/social/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOv2-B/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-B/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-B/bits\endcsname{24576}
\expandafter\def\csname val@fp:image/DINOv2-B/disc\endcsname{0.460}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/chain\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/crop\endcsname{0.67}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/geometric\endcsname{0.89}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/overlay\endcsname{0.62}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/photometric\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-B/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-B/hard\endcsname{0.003}
\expandafter\def\csname val@fp:image/DINOv2-B/hard/pct\endcsname{0.3}
\expandafter\def\csname val@fp:image/DINOv2-B/ms\endcsname{3.9}
\expandafter\def\csname val@fp:image/DINOv2-B/muAP\endcsname{0.703}
\expandafter\def\csname val@fp:image/DINOv2-B/muAP/pct\endcsname{70.3}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/FPRq@pair@1e-07\endcsname{0.005}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/FPRq@pair@1e-07/pct\endcsname{0.5}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/FPRq@query@0.01\endcsname{0.008}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/FPRq@query@0.01/pct\endcsname{0.8}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/R@1\endcsname{0.832}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/R@1/pct\endcsname{83.2}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/R@10\endcsname{0.909}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/R@10/pct\endcsname{90.9}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@0.0001\endcsname{0.798}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@0.0001/pct\endcsname{79.8}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-05\endcsname{0.710}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-05/pct\endcsname{71.0}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-06\endcsname{0.614}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-06/pct\endcsname{61.4}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-07\endcsname{0.519}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-07/pct\endcsname{51.9}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-08\endcsname{0.421}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@pair@1e-08/pct\endcsname{42.1}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@query@0.01\endcsname{0.538}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/TPR@query@0.01/pct\endcsname{53.8}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/background0.5\endcsname{0.10}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/background0.5/pct\endcsname{10}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/blur2\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/blur2/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/bright0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/bright1.4\endcsname{0.88}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/bright1.4/pct\endcsname{88}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/contrast0.5\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/contrast0.5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop30\endcsname{0.17}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop30/pct\endcsname{17}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop50\endcsname{0.54}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop50/pct\endcsname{54}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop50off\endcsname{0.49}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop50off/pct\endcsname{49}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop70\endcsname{0.82}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop70/pct\endcsname{82}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop90\endcsname{0.94}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/crop90/pct\endcsname{94}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/emoji0.3\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/emoji0.3/pct\endcsname{93}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/gray\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/gray/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/hflip\endcsname{0.94}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/hflip/pct\endcsname{94}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/meme\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/meme/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/noise0.05\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/noise0.05/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/pad25\endcsname{0.86}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/pad25/pct\endcsname{86}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/perspective\endcsname{0.89}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/perspective/pct\endcsname{89}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/recapture\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/recapture/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/resize0.25/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot15\endcsname{0.76}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot15/pct\endcsname{76}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot5\endcsname{0.89}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot5/pct\endcsname{89}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot90\endcsname{0.40}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/rot90/pct\endcsname{40}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/screenshot\endcsname{0.02}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/screenshot/pct\endcsname{2}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/skew\endcsname{0.77}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/skew/pct\endcsname{77}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/social\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/social/pct\endcsname{93}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/text\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/bits\endcsname{256}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/disc\endcsname{0.399}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/chain\endcsname{0.92}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/crop\endcsname{0.59}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/geometric\endcsname{0.79}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/overlay\endcsname{0.60}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/photometric\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/ms\endcsname{1.7}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/muAP\endcsname{0.664}
\expandafter\def\csname val@fp:image/DINOv2-S-LSH256/muAP/pct\endcsname{66.4}
\expandafter\def\csname val@fp:image/DINOv2-S/FPRq@pair@1e-07\endcsname{0.007}
\expandafter\def\csname val@fp:image/DINOv2-S/FPRq@pair@1e-07/pct\endcsname{0.7}
\expandafter\def\csname val@fp:image/DINOv2-S/FPRq@query@0.01\endcsname{0.011}
\expandafter\def\csname val@fp:image/DINOv2-S/FPRq@query@0.01/pct\endcsname{1.1}
\expandafter\def\csname val@fp:image/DINOv2-S/R@1\endcsname{0.877}
\expandafter\def\csname val@fp:image/DINOv2-S/R@1/pct\endcsname{87.7}
\expandafter\def\csname val@fp:image/DINOv2-S/R@10\endcsname{0.930}
\expandafter\def\csname val@fp:image/DINOv2-S/R@10/pct\endcsname{93.0}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@0.0001\endcsname{0.831}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@0.0001/pct\endcsname{83.1}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-05\endcsname{0.753}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-05/pct\endcsname{75.3}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-06\endcsname{0.682}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-06/pct\endcsname{68.2}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-07\endcsname{0.612}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-07/pct\endcsname{61.2}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-08\endcsname{0.572}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@pair@1e-08/pct\endcsname{57.1}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@query@0.01\endcsname{0.625}
\expandafter\def\csname val@fp:image/DINOv2-S/TPR@query@0.01/pct\endcsname{62.5}
\expandafter\def\csname val@fp:image/DINOv2-S/att/background0.5\endcsname{0.21}
\expandafter\def\csname val@fp:image/DINOv2-S/att/background0.5/pct\endcsname{21}
\expandafter\def\csname val@fp:image/DINOv2-S/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/bright1.4\endcsname{0.93}
\expandafter\def\csname val@fp:image/DINOv2-S/att/bright1.4/pct\endcsname{93}
\expandafter\def\csname val@fp:image/DINOv2-S/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop30\endcsname{0.28}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop30/pct\endcsname{28}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop50\endcsname{0.68}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop50/pct\endcsname{68}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop50off\endcsname{0.62}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop50off/pct\endcsname{62}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop70\endcsname{0.91}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop70/pct\endcsname{91}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop90\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/crop90/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/emoji0.3\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/emoji0.3/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/gray\endcsname{0.97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/gray/pct\endcsname{97}
\expandafter\def\csname val@fp:image/DINOv2-S/att/hflip\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-S/att/hflip/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg75\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/jpeg75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/meme\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-S/att/meme/pct\endcsname{98}
\expandafter\def\csname val@fp:image/DINOv2-S/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/pad25\endcsname{0.92}
\expandafter\def\csname val@fp:image/DINOv2-S/att/pad25/pct\endcsname{92}
\expandafter\def\csname val@fp:image/DINOv2-S/att/perspective\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/perspective/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/recapture\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/recapture/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot15\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot15/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot5\endcsname{0.95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot5/pct\endcsname{95}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot90\endcsname{0.58}
\expandafter\def\csname val@fp:image/DINOv2-S/att/rot90/pct\endcsname{58}
\expandafter\def\csname val@fp:image/DINOv2-S/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/screenshot\endcsname{0.04}
\expandafter\def\csname val@fp:image/DINOv2-S/att/screenshot/pct\endcsname{4}
\expandafter\def\csname val@fp:image/DINOv2-S/att/skew\endcsname{0.90}
\expandafter\def\csname val@fp:image/DINOv2-S/att/skew/pct\endcsname{90}
\expandafter\def\csname val@fp:image/DINOv2-S/att/social\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-S/att/social/pct\endcsname{96}
\expandafter\def\csname val@fp:image/DINOv2-S/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/DINOv2-S/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/DINOv2-S/bits\endcsname{12288}
\expandafter\def\csname val@fp:image/DINOv2-S/disc\endcsname{0.444}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/chain\endcsname{0.96}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/crop\endcsname{0.69}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/geometric\endcsname{0.88}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/overlay\endcsname{0.64}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/photometric\endcsname{0.98}
\expandafter\def\csname val@fp:image/DINOv2-S/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/DINOv2-S/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/DINOv2-S/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/DINOv2-S/ms\endcsname{2.0}
\expandafter\def\csname val@fp:image/DINOv2-S/muAP\endcsname{0.703}
\expandafter\def\csname val@fp:image/DINOv2-S/muAP/pct\endcsname{70.3}
\expandafter\def\csname val@fp:image/ISC21-1st/FPRq@pair@1e-07\endcsname{0.007}
\expandafter\def\csname val@fp:image/ISC21-1st/FPRq@pair@1e-07/pct\endcsname{0.7}
\expandafter\def\csname val@fp:image/ISC21-1st/FPRq@query@0.01\endcsname{0.008}
\expandafter\def\csname val@fp:image/ISC21-1st/FPRq@query@0.01/pct\endcsname{0.8}
\expandafter\def\csname val@fp:image/ISC21-1st/R@1\endcsname{0.919}
\expandafter\def\csname val@fp:image/ISC21-1st/R@1/pct\endcsname{91.9}
\expandafter\def\csname val@fp:image/ISC21-1st/R@10\endcsname{0.955}
\expandafter\def\csname val@fp:image/ISC21-1st/R@10/pct\endcsname{95.5}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@0.0001\endcsname{0.912}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@0.0001/pct\endcsname{91.2}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-05\endcsname{0.879}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-05/pct\endcsname{87.9}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-06\endcsname{0.817}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-06/pct\endcsname{81.7}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-07\endcsname{0.755}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-07/pct\endcsname{75.5}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-08\endcsname{0.685}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@pair@1e-08/pct\endcsname{68.5}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@query@0.01\endcsname{0.762}
\expandafter\def\csname val@fp:image/ISC21-1st/TPR@query@0.01/pct\endcsname{76.2}
\expandafter\def\csname val@fp:image/ISC21-1st/att/background0.5\endcsname{0.58}
\expandafter\def\csname val@fp:image/ISC21-1st/att/background0.5/pct\endcsname{58}
\expandafter\def\csname val@fp:image/ISC21-1st/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/bright0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/bright1.4\endcsname{0.93}
\expandafter\def\csname val@fp:image/ISC21-1st/att/bright1.4/pct\endcsname{93}
\expandafter\def\csname val@fp:image/ISC21-1st/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop30\endcsname{0.35}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop30/pct\endcsname{35}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop50\endcsname{0.79}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop50/pct\endcsname{79}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop50off\endcsname{0.72}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop50off/pct\endcsname{72}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop70\endcsname{0.94}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop70/pct\endcsname{94}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop90\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/crop90/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/emoji0.3\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/emoji0.3/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/gray\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/gray/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/hflip/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/jpeg75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISC21-1st/att/meme\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/meme/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/noise0.05\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/noise0.05/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISC21-1st/att/pad25\endcsname{0.96}
\expandafter\def\csname val@fp:image/ISC21-1st/att/pad25/pct\endcsname{96}
\expandafter\def\csname val@fp:image/ISC21-1st/att/perspective\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/perspective/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/recapture\endcsname{0.97}
\expandafter\def\csname val@fp:image/ISC21-1st/att/recapture/pct\endcsname{97}
\expandafter\def\csname val@fp:image/ISC21-1st/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/resize0.25/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot15\endcsname{0.96}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot15/pct\endcsname{96}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot5\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot90\endcsname{0.94}
\expandafter\def\csname val@fp:image/ISC21-1st/att/rot90/pct\endcsname{94}
\expandafter\def\csname val@fp:image/ISC21-1st/att/sat2\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/att/sat2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISC21-1st/att/screenshot\endcsname{0.18}
\expandafter\def\csname val@fp:image/ISC21-1st/att/screenshot/pct\endcsname{18}
\expandafter\def\csname val@fp:image/ISC21-1st/att/skew\endcsname{0.97}
\expandafter\def\csname val@fp:image/ISC21-1st/att/skew/pct\endcsname{97}
\expandafter\def\csname val@fp:image/ISC21-1st/att/social\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/social/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISC21-1st/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISC21-1st/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISC21-1st/bits\endcsname{8192}
\expandafter\def\csname val@fp:image/ISC21-1st/disc\endcsname{0.917}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/chain\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/crop\endcsname{0.76}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/geometric\endcsname{0.97}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/overlay\endcsname{0.75}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/photometric\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISC21-1st/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISC21-1st/hard\endcsname{0.004}
\expandafter\def\csname val@fp:image/ISC21-1st/hard/pct\endcsname{0.4}
\expandafter\def\csname val@fp:image/ISC21-1st/ms\endcsname{8.3}
\expandafter\def\csname val@fp:image/ISC21-1st/muAP\endcsname{0.815}
\expandafter\def\csname val@fp:image/ISC21-1st/muAP/pct\endcsname{81.5}
\expandafter\def\csname val@fp:image/ISCC-Image-256/FPRq@pair@1e-07\endcsname{0.007}
\expandafter\def\csname val@fp:image/ISCC-Image-256/FPRq@pair@1e-07/pct\endcsname{0.7}
\expandafter\def\csname val@fp:image/ISCC-Image-256/FPRq@query@0.01\endcsname{0.010}
\expandafter\def\csname val@fp:image/ISCC-Image-256/FPRq@query@0.01/pct\endcsname{1.0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/R@1\endcsname{0.561}
\expandafter\def\csname val@fp:image/ISCC-Image-256/R@1/pct\endcsname{56.1}
\expandafter\def\csname val@fp:image/ISCC-Image-256/R@10\endcsname{0.598}
\expandafter\def\csname val@fp:image/ISCC-Image-256/R@10/pct\endcsname{59.8}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@0.0001\endcsname{0.559}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@0.0001/pct\endcsname{55.9}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-05\endcsname{0.528}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-05/pct\endcsname{52.8}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-06\endcsname{0.494}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-06/pct\endcsname{49.4}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-07\endcsname{0.458}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-07/pct\endcsname{45.8}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@query@0.01\endcsname{0.466}
\expandafter\def\csname val@fp:image/ISCC-Image-256/TPR@query@0.01/pct\endcsname{46.6}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/bright0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/bright1.4\endcsname{0.67}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/bright1.4/pct\endcsname{67}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop50\endcsname{0.01}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop50/pct\endcsname{1}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop70\endcsname{0.11}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop70/pct\endcsname{11}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop90\endcsname{0.72}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/crop90/pct\endcsname{72}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/emoji0.3\endcsname{0.54}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/emoji0.3/pct\endcsname{54}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg30\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg30/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg50\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg50/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg75\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/jpeg75/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/meme\endcsname{0.16}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/meme/pct\endcsname{16}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/noise0.05\endcsname{0.52}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/noise0.05/pct\endcsname{52}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/pad25\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/pad25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/perspective\endcsname{0.19}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/perspective/pct\endcsname{19}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/recapture\endcsname{0.28}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/recapture/pct\endcsname{28}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/resize0.25\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/resize0.25/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot5\endcsname{0.08}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot5/pct\endcsname{8}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/skew\endcsname{0.03}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/skew/pct\endcsname{3}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/social\endcsname{0.68}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/social/pct\endcsname{68}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/squash0.75\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/text\endcsname{0.70}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/text/pct\endcsname{70}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/webp50\endcsname{0.64}
\expandafter\def\csname val@fp:image/ISCC-Image-256/att/webp50/pct\endcsname{64}
\expandafter\def\csname val@fp:image/ISCC-Image-256/bits\endcsname{256}
\expandafter\def\csname val@fp:image/ISCC-Image-256/disc\endcsname{0.292}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/chain\endcsname{0.48}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/compression\endcsname{0.90}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/crop\endcsname{0.17}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/geometric\endcsname{0.19}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/overlay\endcsname{0.28}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/photometric\endcsname{0.90}
\expandafter\def\csname val@fp:image/ISCC-Image-256/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-256/hard\endcsname{0.001}
\expandafter\def\csname val@fp:image/ISCC-Image-256/hard/pct\endcsname{0.1}
\expandafter\def\csname val@fp:image/ISCC-Image-256/ms\endcsname{11}
\expandafter\def\csname val@fp:image/ISCC-Image-256/muAP\endcsname{0.507}
\expandafter\def\csname val@fp:image/ISCC-Image-256/muAP/pct\endcsname{50.7}
\expandafter\def\csname val@fp:image/ISCC-Image-64/FPRq@pair@1e-07\endcsname{0.004}
\expandafter\def\csname val@fp:image/ISCC-Image-64/FPRq@pair@1e-07/pct\endcsname{0.4}
\expandafter\def\csname val@fp:image/ISCC-Image-64/FPRq@query@0.01\endcsname{0.004}
\expandafter\def\csname val@fp:image/ISCC-Image-64/FPRq@query@0.01/pct\endcsname{0.4}
\expandafter\def\csname val@fp:image/ISCC-Image-64/R@1\endcsname{0.558}
\expandafter\def\csname val@fp:image/ISCC-Image-64/R@1/pct\endcsname{55.8}
\expandafter\def\csname val@fp:image/ISCC-Image-64/R@10\endcsname{0.598}
\expandafter\def\csname val@fp:image/ISCC-Image-64/R@10/pct\endcsname{59.8}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@0.0001\endcsname{0.547}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@0.0001/pct\endcsname{54.7}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-05\endcsname{0.514}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-05/pct\endcsname{51.4}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-06\endcsname{0.471}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-06/pct\endcsname{47.1}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-07\endcsname{0.427}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-07/pct\endcsname{42.7}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@query@0.01\endcsname{0.427}
\expandafter\def\csname val@fp:image/ISCC-Image-64/TPR@query@0.01/pct\endcsname{42.7}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/bright0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/bright1.4\endcsname{0.65}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/bright1.4/pct\endcsname{65}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop50\endcsname{0.01}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop50/pct\endcsname{1}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop70\endcsname{0.12}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop70/pct\endcsname{12}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop90\endcsname{0.72}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/crop90/pct\endcsname{72}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/emoji0.3\endcsname{0.51}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/emoji0.3/pct\endcsname{51}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/gamma0.6\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/gamma0.6/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/gray\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/gray/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg30\endcsname{0.97}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg30/pct\endcsname{97}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg50\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg50/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg75\endcsname{0.97}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/jpeg75/pct\endcsname{97}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/meme\endcsname{0.18}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/meme/pct\endcsname{18}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/noise0.05\endcsname{0.52}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/noise0.05/pct\endcsname{52}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/pad25\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/pad25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/perspective\endcsname{0.18}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/perspective/pct\endcsname{18}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/pixelize0.3\endcsname{0.98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/pixelize0.3/pct\endcsname{98}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/recapture\endcsname{0.26}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/recapture/pct\endcsname{26}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/resize0.25/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot5\endcsname{0.06}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot5/pct\endcsname{6}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/skew\endcsname{0.04}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/skew/pct\endcsname{4}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/social\endcsname{0.67}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/social/pct\endcsname{67}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/text\endcsname{0.70}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/text/pct\endcsname{70}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/webp50\endcsname{0.64}
\expandafter\def\csname val@fp:image/ISCC-Image-64/att/webp50/pct\endcsname{64}
\expandafter\def\csname val@fp:image/ISCC-Image-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:image/ISCC-Image-64/disc\endcsname{0.269}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/chain\endcsname{0.47}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/compression\endcsname{0.89}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/crop\endcsname{0.17}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/geometric\endcsname{0.18}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/overlay\endcsname{0.28}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/photometric\endcsname{0.90}
\expandafter\def\csname val@fp:image/ISCC-Image-64/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/ISCC-Image-64/hard\endcsname{0.001}
\expandafter\def\csname val@fp:image/ISCC-Image-64/hard/pct\endcsname{0.1}
\expandafter\def\csname val@fp:image/ISCC-Image-64/ms\endcsname{11}
\expandafter\def\csname val@fp:image/ISCC-Image-64/muAP\endcsname{0.491}
\expandafter\def\csname val@fp:image/ISCC-Image-64/muAP/pct\endcsname{49.1}
\expandafter\def\csname val@fp:image/MarrHildreth/FPRq@pair@1e-07\endcsname{0.004}
\expandafter\def\csname val@fp:image/MarrHildreth/FPRq@pair@1e-07/pct\endcsname{0.4}
\expandafter\def\csname val@fp:image/MarrHildreth/FPRq@query@0.01\endcsname{0.008}
\expandafter\def\csname val@fp:image/MarrHildreth/FPRq@query@0.01/pct\endcsname{0.8}
\expandafter\def\csname val@fp:image/MarrHildreth/R@1\endcsname{0.586}
\expandafter\def\csname val@fp:image/MarrHildreth/R@1/pct\endcsname{58.6}
\expandafter\def\csname val@fp:image/MarrHildreth/R@10\endcsname{0.655}
\expandafter\def\csname val@fp:image/MarrHildreth/R@10/pct\endcsname{65.5}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@0.0001\endcsname{0.518}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@0.0001/pct\endcsname{51.8}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-05\endcsname{0.470}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-05/pct\endcsname{47.0}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-06\endcsname{0.411}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-06/pct\endcsname{41.1}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-07\endcsname{0.314}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-07/pct\endcsname{31.4}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-08\endcsname{0.057}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@pair@1e-08/pct\endcsname{5.7}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@query@0.01\endcsname{0.362}
\expandafter\def\csname val@fp:image/MarrHildreth/TPR@query@0.01/pct\endcsname{36.2}
\expandafter\def\csname val@fp:image/MarrHildreth/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/blur2\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/blur2/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/bright0.6\endcsname{0.95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/bright0.6/pct\endcsname{95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/bright1.4\endcsname{0.79}
\expandafter\def\csname val@fp:image/MarrHildreth/att/bright1.4/pct\endcsname{79}
\expandafter\def\csname val@fp:image/MarrHildreth/att/contrast0.5\endcsname{0.95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/contrast0.5/pct\endcsname{95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop70\endcsname{0.01}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop70/pct\endcsname{1}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop90\endcsname{0.62}
\expandafter\def\csname val@fp:image/MarrHildreth/att/crop90/pct\endcsname{62}
\expandafter\def\csname val@fp:image/MarrHildreth/att/emoji0.3\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/emoji0.3/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/gamma0.6\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/gamma0.6/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:image/MarrHildreth/att/hflip\endcsname{0.21}
\expandafter\def\csname val@fp:image/MarrHildreth/att/hflip/pct\endcsname{21}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg30\endcsname{0.93}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg30/pct\endcsname{93}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg50\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg50/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg75\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/jpeg75/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/meme\endcsname{0.14}
\expandafter\def\csname val@fp:image/MarrHildreth/att/meme/pct\endcsname{14}
\expandafter\def\csname val@fp:image/MarrHildreth/att/noise0.05\endcsname{0.93}
\expandafter\def\csname val@fp:image/MarrHildreth/att/noise0.05/pct\endcsname{93}
\expandafter\def\csname val@fp:image/MarrHildreth/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/MarrHildreth/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/perspective\endcsname{0.48}
\expandafter\def\csname val@fp:image/MarrHildreth/att/perspective/pct\endcsname{48}
\expandafter\def\csname val@fp:image/MarrHildreth/att/pixelize0.3\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/pixelize0.3/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/recapture\endcsname{0.70}
\expandafter\def\csname val@fp:image/MarrHildreth/att/recapture/pct\endcsname{70}
\expandafter\def\csname val@fp:image/MarrHildreth/att/resize0.25\endcsname{0.92}
\expandafter\def\csname val@fp:image/MarrHildreth/att/resize0.25/pct\endcsname{92}
\expandafter\def\csname val@fp:image/MarrHildreth/att/resize0.5\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/resize0.5/pct\endcsname{94}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot5\endcsname{0.16}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot5/pct\endcsname{16}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/sat2\endcsname{0.95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/sat2/pct\endcsname{95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/MarrHildreth/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/MarrHildreth/att/skew\endcsname{0.36}
\expandafter\def\csname val@fp:image/MarrHildreth/att/skew/pct\endcsname{36}
\expandafter\def\csname val@fp:image/MarrHildreth/att/social\endcsname{0.59}
\expandafter\def\csname val@fp:image/MarrHildreth/att/social/pct\endcsname{59}
\expandafter\def\csname val@fp:image/MarrHildreth/att/squash0.75\endcsname{0.95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/squash0.75/pct\endcsname{95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/text\endcsname{0.95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/text/pct\endcsname{95}
\expandafter\def\csname val@fp:image/MarrHildreth/att/webp50\endcsname{0.93}
\expandafter\def\csname val@fp:image/MarrHildreth/att/webp50/pct\endcsname{93}
\expandafter\def\csname val@fp:image/MarrHildreth/bits\endcsname{576}
\expandafter\def\csname val@fp:image/MarrHildreth/disc\endcsname{0.292}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/chain\endcsname{0.64}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/compression\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/crop\endcsname{0.13}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/geometric\endcsname{0.17}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/overlay\endcsname{0.40}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/photometric\endcsname{0.93}
\expandafter\def\csname val@fp:image/MarrHildreth/fam/scale\endcsname{0.94}
\expandafter\def\csname val@fp:image/MarrHildreth/hard\endcsname{0.001}
\expandafter\def\csname val@fp:image/MarrHildreth/hard/pct\endcsname{0.1}
\expandafter\def\csname val@fp:image/MarrHildreth/ms\endcsname{5.5}
\expandafter\def\csname val@fp:image/MarrHildreth/muAP\endcsname{0.455}
\expandafter\def\csname val@fp:image/MarrHildreth/muAP/pct\endcsname{45.5}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/FPRq@pair@1e-07\endcsname{0.002}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/FPRq@pair@1e-07/pct\endcsname{0.2}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/FPRq@query@0.01\endcsname{0.006}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/FPRq@query@0.01/pct\endcsname{0.6}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/R@1\endcsname{0.864}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/R@1/pct\endcsname{86.4}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/R@10\endcsname{0.915}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/R@10/pct\endcsname{91.5}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@0.0001\endcsname{0.838}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@0.0001/pct\endcsname{83.8}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-05\endcsname{0.721}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-05/pct\endcsname{72.1}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-06\endcsname{0.481}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-06/pct\endcsname{48.1}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-07\endcsname{0.356}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-07/pct\endcsname{35.6}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-08\endcsname{0.289}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@pair@1e-08/pct\endcsname{28.9}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@query@0.01\endcsname{0.401}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/TPR@query@0.01/pct\endcsname{40.1}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/background0.5\endcsname{0.17}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/background0.5/pct\endcsname{17}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/bright0.6\endcsname{0.98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/bright0.6/pct\endcsname{98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/bright1.4\endcsname{0.90}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/bright1.4/pct\endcsname{90}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/contrast0.5\endcsname{0.98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/contrast0.5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop30\endcsname{0.15}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop30/pct\endcsname{15}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop50\endcsname{0.53}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop50/pct\endcsname{53}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop50off\endcsname{0.46}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop50off/pct\endcsname{46}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop70\endcsname{0.89}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop70/pct\endcsname{89}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop90\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/crop90/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/emoji0.3\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/emoji0.3/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/gamma0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/gray\endcsname{0.89}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/gray/pct\endcsname{89}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/hflip\endcsname{0.94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/hflip/pct\endcsname{94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg50\endcsname{0.98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg50/pct\endcsname{98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/meme\endcsname{0.98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/meme/pct\endcsname{98}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/pad25\endcsname{0.94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/pad25/pct\endcsname{94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/perspective\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/perspective/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/recapture\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/recapture/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot15\endcsname{0.90}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot15/pct\endcsname{90}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot5\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot5/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot90\endcsname{0.73}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/rot90/pct\endcsname{73}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/skew\endcsname{0.94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/skew/pct\endcsname{94}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/social\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/social/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/text\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/text/pct\endcsname{97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/bits\endcsname{16384}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/disc\endcsname{0.234}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/chain\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/crop\endcsname{0.60}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/geometric\endcsname{0.91}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/overlay\endcsname{0.62}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/photometric\endcsname{0.97}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/hard\endcsname{0.002}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/hard/pct\endcsname{0.2}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/ms\endcsname{1.1}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/muAP\endcsname{0.657}
\expandafter\def\csname val@fp:image/OpenCLIP-B32/muAP/pct\endcsname{65.7}
\expandafter\def\csname val@fp:image/PDQ-dihedral/FPRq@pair@1e-07\endcsname{0.008}
\expandafter\def\csname val@fp:image/PDQ-dihedral/FPRq@pair@1e-07/pct\endcsname{0.8}
\expandafter\def\csname val@fp:image/PDQ-dihedral/FPRq@query@0.01\endcsname{0.011}
\expandafter\def\csname val@fp:image/PDQ-dihedral/FPRq@query@0.01/pct\endcsname{1.1}
\expandafter\def\csname val@fp:image/PDQ-dihedral/R@1\endcsname{0.623}
\expandafter\def\csname val@fp:image/PDQ-dihedral/R@1/pct\endcsname{62.3}
\expandafter\def\csname val@fp:image/PDQ-dihedral/R@10\endcsname{0.652}
\expandafter\def\csname val@fp:image/PDQ-dihedral/R@10/pct\endcsname{65.2}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@0.0001\endcsname{0.619}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@0.0001/pct\endcsname{61.9}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-05\endcsname{0.594}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-05/pct\endcsname{59.4}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-06\endcsname{0.567}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-06/pct\endcsname{56.7}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-07\endcsname{0.546}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-07/pct\endcsname{54.6}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-08\endcsname{0.508}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@pair@1e-08/pct\endcsname{50.8}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@query@0.01\endcsname{0.549}
\expandafter\def\csname val@fp:image/PDQ-dihedral/TPR@query@0.01/pct\endcsname{54.9}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/blur2\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/blur2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/bright0.6\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/bright1.4\endcsname{0.95}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/bright1.4/pct\endcsname{95}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/contrast0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/contrast0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop70\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop70/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop90\endcsname{0.29}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/crop90/pct\endcsname{29}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/emoji0.3\endcsname{0.88}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/emoji0.3/pct\endcsname{88}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/hflip/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg30\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg30/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg50\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg75\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/jpeg75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/meme\endcsname{0.03}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/meme/pct\endcsname{3}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/noise0.05\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/noise0.05/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/perspective\endcsname{0.29}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/perspective/pct\endcsname{29}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/recapture\endcsname{0.65}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/recapture/pct\endcsname{65}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/resize0.25\endcsname{0.98}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/resize0.25/pct\endcsname{98}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot5\endcsname{0.14}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot5/pct\endcsname{14}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot90\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/rot90/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/sat2\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/sat2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/skew\endcsname{0.03}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/skew/pct\endcsname{3}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/social\endcsname{0.28}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/social/pct\endcsname{28}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/text\endcsname{0.98}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/webp50\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/att/webp50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ-dihedral/bits\endcsname{256}
\expandafter\def\csname val@fp:image/PDQ-dihedral/disc\endcsname{0.367}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/chain\endcsname{0.47}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/compression\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/crop\endcsname{0.06}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/geometric\endcsname{0.35}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/overlay\endcsname{0.38}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ-dihedral/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/PDQ-dihedral/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/PDQ-dihedral/ms\endcsname{31}
\expandafter\def\csname val@fp:image/PDQ-dihedral/muAP\endcsname{0.569}
\expandafter\def\csname val@fp:image/PDQ-dihedral/muAP/pct\endcsname{56.9}
\expandafter\def\csname val@fp:image/PDQ/FPRq@pair@1e-07\endcsname{0.010}
\expandafter\def\csname val@fp:image/PDQ/FPRq@pair@1e-07/pct\endcsname{1.0}
\expandafter\def\csname val@fp:image/PDQ/FPRq@query@0.01\endcsname{0.010}
\expandafter\def\csname val@fp:image/PDQ/FPRq@query@0.01/pct\endcsname{1.0}
\expandafter\def\csname val@fp:image/PDQ/R@1\endcsname{0.579}
\expandafter\def\csname val@fp:image/PDQ/R@1/pct\endcsname{57.9}
\expandafter\def\csname val@fp:image/PDQ/R@10\endcsname{0.611}
\expandafter\def\csname val@fp:image/PDQ/R@10/pct\endcsname{61.1}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@0.0001\endcsname{0.576}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@0.0001/pct\endcsname{57.6}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-05\endcsname{0.546}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-05/pct\endcsname{54.6}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-06\endcsname{0.515}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-06/pct\endcsname{51.5}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-07\endcsname{0.495}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-07/pct\endcsname{49.5}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-08\endcsname{0.457}
\expandafter\def\csname val@fp:image/PDQ/TPR@pair@1e-08/pct\endcsname{45.7}
\expandafter\def\csname val@fp:image/PDQ/TPR@query@0.01\endcsname{0.495}
\expandafter\def\csname val@fp:image/PDQ/TPR@query@0.01/pct\endcsname{49.5}
\expandafter\def\csname val@fp:image/PDQ/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/blur2\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/blur2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/bright0.6\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/bright1.4\endcsname{0.95}
\expandafter\def\csname val@fp:image/PDQ/att/bright1.4/pct\endcsname{95}
\expandafter\def\csname val@fp:image/PDQ/att/contrast0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/contrast0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/crop70\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/crop70/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/crop90\endcsname{0.36}
\expandafter\def\csname val@fp:image/PDQ/att/crop90/pct\endcsname{36}
\expandafter\def\csname val@fp:image/PDQ/att/emoji0.3\endcsname{0.90}
\expandafter\def\csname val@fp:image/PDQ/att/emoji0.3/pct\endcsname{90}
\expandafter\def\csname val@fp:image/PDQ/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg30\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg30/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg50\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg75\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/jpeg75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/meme\endcsname{0.05}
\expandafter\def\csname val@fp:image/PDQ/att/meme/pct\endcsname{5}
\expandafter\def\csname val@fp:image/PDQ/att/noise0.05\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/noise0.05/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/perspective\endcsname{0.34}
\expandafter\def\csname val@fp:image/PDQ/att/perspective/pct\endcsname{34}
\expandafter\def\csname val@fp:image/PDQ/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/recapture\endcsname{0.70}
\expandafter\def\csname val@fp:image/PDQ/att/recapture/pct\endcsname{70}
\expandafter\def\csname val@fp:image/PDQ/att/resize0.25\endcsname{0.98}
\expandafter\def\csname val@fp:image/PDQ/att/resize0.25/pct\endcsname{98}
\expandafter\def\csname val@fp:image/PDQ/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/PDQ/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/rot5\endcsname{0.21}
\expandafter\def\csname val@fp:image/PDQ/att/rot5/pct\endcsname{21}
\expandafter\def\csname val@fp:image/PDQ/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/sat2\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/sat2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/PDQ/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/PDQ/att/skew\endcsname{0.05}
\expandafter\def\csname val@fp:image/PDQ/att/skew/pct\endcsname{5}
\expandafter\def\csname val@fp:image/PDQ/att/social\endcsname{0.36}
\expandafter\def\csname val@fp:image/PDQ/att/social/pct\endcsname{36}
\expandafter\def\csname val@fp:image/PDQ/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/att/text\endcsname{0.98}
\expandafter\def\csname val@fp:image/PDQ/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:image/PDQ/att/webp50\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/att/webp50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/PDQ/bits\endcsname{256}
\expandafter\def\csname val@fp:image/PDQ/disc\endcsname{0.295}
\expandafter\def\csname val@fp:image/PDQ/fam/chain\endcsname{0.53}
\expandafter\def\csname val@fp:image/PDQ/fam/compression\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/fam/crop\endcsname{0.07}
\expandafter\def\csname val@fp:image/PDQ/fam/geometric\endcsname{0.09}
\expandafter\def\csname val@fp:image/PDQ/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/PDQ/fam/overlay\endcsname{0.39}
\expandafter\def\csname val@fp:image/PDQ/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/PDQ/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/PDQ/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/PDQ/ms\endcsname{31}
\expandafter\def\csname val@fp:image/PDQ/muAP\endcsname{0.520}
\expandafter\def\csname val@fp:image/PDQ/muAP/pct\endcsname{52.0}
\expandafter\def\csname val@fp:image/SSCD-large/FPRq@pair@1e-07\endcsname{0.002}
\expandafter\def\csname val@fp:image/SSCD-large/FPRq@pair@1e-07/pct\endcsname{0.2}
\expandafter\def\csname val@fp:image/SSCD-large/FPRq@query@0.01\endcsname{0.010}
\expandafter\def\csname val@fp:image/SSCD-large/FPRq@query@0.01/pct\endcsname{1.0}
\expandafter\def\csname val@fp:image/SSCD-large/R@1\endcsname{0.942}
\expandafter\def\csname val@fp:image/SSCD-large/R@1/pct\endcsname{94.2}
\expandafter\def\csname val@fp:image/SSCD-large/R@10\endcsname{0.969}
\expandafter\def\csname val@fp:image/SSCD-large/R@10/pct\endcsname{96.9}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@0.0001\endcsname{0.935}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@0.0001/pct\endcsname{93.5}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-05\endcsname{0.899}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-05/pct\endcsname{89.9}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-06\endcsname{0.814}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-06/pct\endcsname{81.4}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-07\endcsname{0.703}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-07/pct\endcsname{70.2}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-08\endcsname{0.672}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@pair@1e-08/pct\endcsname{67.2}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@query@0.01\endcsname{0.763}
\expandafter\def\csname val@fp:image/SSCD-large/TPR@query@0.01/pct\endcsname{76.3}
\expandafter\def\csname val@fp:image/SSCD-large/att/background0.5\endcsname{0.52}
\expandafter\def\csname val@fp:image/SSCD-large/att/background0.5/pct\endcsname{52}
\expandafter\def\csname val@fp:image/SSCD-large/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/bright1.4\endcsname{0.97}
\expandafter\def\csname val@fp:image/SSCD-large/att/bright1.4/pct\endcsname{97}
\expandafter\def\csname val@fp:image/SSCD-large/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop30\endcsname{0.75}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop30/pct\endcsname{75}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop50\endcsname{0.93}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop50/pct\endcsname{93}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop50off\endcsname{0.92}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop50off/pct\endcsname{92}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop70\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop70/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop90\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/crop90/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/emoji0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/emoji0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/gamma0.6\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/gamma0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/gray\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-large/att/gray/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-large/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/hflip/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/meme\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/meme/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/pad25\endcsname{0.97}
\expandafter\def\csname val@fp:image/SSCD-large/att/pad25/pct\endcsname{97}
\expandafter\def\csname val@fp:image/SSCD-large/att/perspective\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/perspective/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/recapture\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/recapture/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot15\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot15/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot5\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot90\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/rot90/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/sat2\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/sat2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/screenshot\endcsname{0.08}
\expandafter\def\csname val@fp:image/SSCD-large/att/screenshot/pct\endcsname{8}
\expandafter\def\csname val@fp:image/SSCD-large/att/skew\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/skew/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/social\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/social/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-large/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-large/bits\endcsname{32768}
\expandafter\def\csname val@fp:image/SSCD-large/disc\endcsname{0.823}
\expandafter\def\csname val@fp:image/SSCD-large/fam/chain\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/fam/crop\endcsname{0.92}
\expandafter\def\csname val@fp:image/SSCD-large/fam/geometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/fam/overlay\endcsname{0.72}
\expandafter\def\csname val@fp:image/SSCD-large/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-large/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-large/hard\endcsname{0.007}
\expandafter\def\csname val@fp:image/SSCD-large/hard/pct\endcsname{0.7}
\expandafter\def\csname val@fp:image/SSCD-large/ms\endcsname{4.6}
\expandafter\def\csname val@fp:image/SSCD-large/muAP\endcsname{0.787}
\expandafter\def\csname val@fp:image/SSCD-large/muAP/pct\endcsname{78.7}
\expandafter\def\csname val@fp:image/SSCD-mixup/FPRq@pair@1e-07\endcsname{0.004}
\expandafter\def\csname val@fp:image/SSCD-mixup/FPRq@pair@1e-07/pct\endcsname{0.4}
\expandafter\def\csname val@fp:image/SSCD-mixup/FPRq@query@0.01\endcsname{0.010}
\expandafter\def\csname val@fp:image/SSCD-mixup/FPRq@query@0.01/pct\endcsname{1.0}
\expandafter\def\csname val@fp:image/SSCD-mixup/R@1\endcsname{0.929}
\expandafter\def\csname val@fp:image/SSCD-mixup/R@1/pct\endcsname{92.9}
\expandafter\def\csname val@fp:image/SSCD-mixup/R@10\endcsname{0.961}
\expandafter\def\csname val@fp:image/SSCD-mixup/R@10/pct\endcsname{96.1}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@0.0001\endcsname{0.916}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@0.0001/pct\endcsname{91.6}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-05\endcsname{0.876}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-05/pct\endcsname{87.6}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-06\endcsname{0.763}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-06/pct\endcsname{76.3}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-07\endcsname{0.712}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-07/pct\endcsname{71.2}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-08\endcsname{0.697}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@pair@1e-08/pct\endcsname{69.7}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@query@0.01\endcsname{0.725}
\expandafter\def\csname val@fp:image/SSCD-mixup/TPR@query@0.01/pct\endcsname{72.5}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/background0.5\endcsname{0.46}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/background0.5/pct\endcsname{46}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/bright0.6\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/bright1.4\endcsname{0.97}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/bright1.4/pct\endcsname{97}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/contrast0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop30\endcsname{0.53}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop30/pct\endcsname{53}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop50\endcsname{0.89}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop50/pct\endcsname{89}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop50off\endcsname{0.88}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop50off/pct\endcsname{88}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop70\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop70/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop90\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/crop90/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/emoji0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/emoji0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/gray\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/gray/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/hflip/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/meme\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/meme/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/pad25\endcsname{0.96}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/pad25/pct\endcsname{96}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/perspective\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/perspective/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/recapture\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/recapture/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/resize0.25/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot15\endcsname{0.97}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot15/pct\endcsname{97}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot5\endcsname{0.97}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot90\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/rot90/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/sat2\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/sat2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/screenshot\endcsname{0.06}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/screenshot/pct\endcsname{6}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/skew\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/skew/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/social\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/social/pct\endcsname{98}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/SSCD-mixup/bits\endcsname{16384}
\expandafter\def\csname val@fp:image/SSCD-mixup/disc\endcsname{0.795}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/chain\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/crop\endcsname{0.85}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/geometric\endcsname{0.98}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/overlay\endcsname{0.70}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/SSCD-mixup/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/SSCD-mixup/hard\endcsname{0.007}
\expandafter\def\csname val@fp:image/SSCD-mixup/hard/pct\endcsname{0.7}
\expandafter\def\csname val@fp:image/SSCD-mixup/ms\endcsname{2.7}
\expandafter\def\csname val@fp:image/SSCD-mixup/muAP\endcsname{0.763}
\expandafter\def\csname val@fp:image/SSCD-mixup/muAP/pct\endcsname{76.3}
\expandafter\def\csname val@fp:image/aHash-64/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/FPRq@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/FPRq@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/R@1\endcsname{0.503}
\expandafter\def\csname val@fp:image/aHash-64/R@1/pct\endcsname{50.3}
\expandafter\def\csname val@fp:image/aHash-64/R@10\endcsname{0.581}
\expandafter\def\csname val@fp:image/aHash-64/R@10/pct\endcsname{58.1}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@0.0001\endcsname{0.463}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@0.0001/pct\endcsname{46.3}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-05\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-05/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-06\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-06/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/TPR@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/TPR@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/blur2\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/blur2/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/bright0.6\endcsname{0.88}
\expandafter\def\csname val@fp:image/aHash-64/att/bright0.6/pct\endcsname{88}
\expandafter\def\csname val@fp:image/aHash-64/att/bright1.4\endcsname{0.54}
\expandafter\def\csname val@fp:image/aHash-64/att/bright1.4/pct\endcsname{54}
\expandafter\def\csname val@fp:image/aHash-64/att/contrast0.5\endcsname{0.88}
\expandafter\def\csname val@fp:image/aHash-64/att/contrast0.5/pct\endcsname{88}
\expandafter\def\csname val@fp:image/aHash-64/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/crop70\endcsname{0.02}
\expandafter\def\csname val@fp:image/aHash-64/att/crop70/pct\endcsname{2}
\expandafter\def\csname val@fp:image/aHash-64/att/crop90\endcsname{0.40}
\expandafter\def\csname val@fp:image/aHash-64/att/crop90/pct\endcsname{40}
\expandafter\def\csname val@fp:image/aHash-64/att/emoji0.3\endcsname{0.61}
\expandafter\def\csname val@fp:image/aHash-64/att/emoji0.3/pct\endcsname{61}
\expandafter\def\csname val@fp:image/aHash-64/att/gamma0.6\endcsname{0.85}
\expandafter\def\csname val@fp:image/aHash-64/att/gamma0.6/pct\endcsname{85}
\expandafter\def\csname val@fp:image/aHash-64/att/gray\endcsname{0.92}
\expandafter\def\csname val@fp:image/aHash-64/att/gray/pct\endcsname{92}
\expandafter\def\csname val@fp:image/aHash-64/att/hflip\endcsname{0.12}
\expandafter\def\csname val@fp:image/aHash-64/att/hflip/pct\endcsname{12}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg30\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg30/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg50\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg50/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg75\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/jpeg75/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/meme\endcsname{0.03}
\expandafter\def\csname val@fp:image/aHash-64/att/meme/pct\endcsname{3}
\expandafter\def\csname val@fp:image/aHash-64/att/noise0.05\endcsname{0.89}
\expandafter\def\csname val@fp:image/aHash-64/att/noise0.05/pct\endcsname{89}
\expandafter\def\csname val@fp:image/aHash-64/att/none\endcsname{0.92}
\expandafter\def\csname val@fp:image/aHash-64/att/none/pct\endcsname{92}
\expandafter\def\csname val@fp:image/aHash-64/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/perspective\endcsname{0.24}
\expandafter\def\csname val@fp:image/aHash-64/att/perspective/pct\endcsname{24}
\expandafter\def\csname val@fp:image/aHash-64/att/pixelize0.3\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/pixelize0.3/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/recapture\endcsname{0.43}
\expandafter\def\csname val@fp:image/aHash-64/att/recapture/pct\endcsname{43}
\expandafter\def\csname val@fp:image/aHash-64/att/resize0.25\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/resize0.25/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/resize0.5\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/resize0.5/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/rot5\endcsname{0.05}
\expandafter\def\csname val@fp:image/aHash-64/att/rot5/pct\endcsname{5}
\expandafter\def\csname val@fp:image/aHash-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/sat2\endcsname{0.90}
\expandafter\def\csname val@fp:image/aHash-64/att/sat2/pct\endcsname{90}
\expandafter\def\csname val@fp:image/aHash-64/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/aHash-64/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/aHash-64/att/skew\endcsname{0.07}
\expandafter\def\csname val@fp:image/aHash-64/att/skew/pct\endcsname{7}
\expandafter\def\csname val@fp:image/aHash-64/att/social\endcsname{0.40}
\expandafter\def\csname val@fp:image/aHash-64/att/social/pct\endcsname{40}
\expandafter\def\csname val@fp:image/aHash-64/att/squash0.75\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/squash0.75/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/att/text\endcsname{0.78}
\expandafter\def\csname val@fp:image/aHash-64/att/text/pct\endcsname{78}
\expandafter\def\csname val@fp:image/aHash-64/att/webp50\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/att/webp50/pct\endcsname{91}
\expandafter\def\csname val@fp:image/aHash-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:image/aHash-64/disc\endcsname{0.027}
\expandafter\def\csname val@fp:image/aHash-64/fam/chain\endcsname{0.41}
\expandafter\def\csname val@fp:image/aHash-64/fam/compression\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/fam/crop\endcsname{0.08}
\expandafter\def\csname val@fp:image/aHash-64/fam/geometric\endcsname{0.07}
\expandafter\def\csname val@fp:image/aHash-64/fam/none\endcsname{0.92}
\expandafter\def\csname val@fp:image/aHash-64/fam/overlay\endcsname{0.28}
\expandafter\def\csname val@fp:image/aHash-64/fam/photometric\endcsname{0.85}
\expandafter\def\csname val@fp:image/aHash-64/fam/scale\endcsname{0.91}
\expandafter\def\csname val@fp:image/aHash-64/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/aHash-64/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/aHash-64/ms\endcsname{4.3}
\expandafter\def\csname val@fp:image/aHash-64/muAP\endcsname{0.189}
\expandafter\def\csname val@fp:image/aHash-64/muAP/pct\endcsname{18.9}
\expandafter\def\csname val@fp:image/cal_sources\endcsname{769}
\expandafter\def\csname val@fp:image/dHash-64/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/dHash-64/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/dHash-64/FPRq@query@0.01\endcsname{0.011}
\expandafter\def\csname val@fp:image/dHash-64/FPRq@query@0.01/pct\endcsname{1.1}
\expandafter\def\csname val@fp:image/dHash-64/R@1\endcsname{0.560}
\expandafter\def\csname val@fp:image/dHash-64/R@1/pct\endcsname{56.0}
\expandafter\def\csname val@fp:image/dHash-64/R@10\endcsname{0.615}
\expandafter\def\csname val@fp:image/dHash-64/R@10/pct\endcsname{61.5}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@0.0001\endcsname{0.533}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@0.0001/pct\endcsname{53.3}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-05\endcsname{0.441}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-05/pct\endcsname{44.1}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-06\endcsname{0.000}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-06/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/dHash-64/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/dHash-64/TPR@query@0.01\endcsname{0.313}
\expandafter\def\csname val@fp:image/dHash-64/TPR@query@0.01/pct\endcsname{31.3}
\expandafter\def\csname val@fp:image/dHash-64/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/blur2\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/blur2/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/bright0.6\endcsname{0.91}
\expandafter\def\csname val@fp:image/dHash-64/att/bright0.6/pct\endcsname{91}
\expandafter\def\csname val@fp:image/dHash-64/att/bright1.4\endcsname{0.73}
\expandafter\def\csname val@fp:image/dHash-64/att/bright1.4/pct\endcsname{73}
\expandafter\def\csname val@fp:image/dHash-64/att/contrast0.5\endcsname{0.90}
\expandafter\def\csname val@fp:image/dHash-64/att/contrast0.5/pct\endcsname{90}
\expandafter\def\csname val@fp:image/dHash-64/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/crop70\endcsname{0.01}
\expandafter\def\csname val@fp:image/dHash-64/att/crop70/pct\endcsname{1}
\expandafter\def\csname val@fp:image/dHash-64/att/crop90\endcsname{0.51}
\expandafter\def\csname val@fp:image/dHash-64/att/crop90/pct\endcsname{51}
\expandafter\def\csname val@fp:image/dHash-64/att/emoji0.3\endcsname{0.87}
\expandafter\def\csname val@fp:image/dHash-64/att/emoji0.3/pct\endcsname{87}
\expandafter\def\csname val@fp:image/dHash-64/att/gamma0.6\endcsname{0.94}
\expandafter\def\csname val@fp:image/dHash-64/att/gamma0.6/pct\endcsname{94}
\expandafter\def\csname val@fp:image/dHash-64/att/gray\endcsname{0.99}
\expandafter\def\csname val@fp:image/dHash-64/att/gray/pct\endcsname{99}
\expandafter\def\csname val@fp:image/dHash-64/att/hflip\endcsname{0.10}
\expandafter\def\csname val@fp:image/dHash-64/att/hflip/pct\endcsname{10}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg30\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg30/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg50\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg50/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg75\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/jpeg75/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/meme\endcsname{0.08}
\expandafter\def\csname val@fp:image/dHash-64/att/meme/pct\endcsname{8}
\expandafter\def\csname val@fp:image/dHash-64/att/noise0.05\endcsname{0.94}
\expandafter\def\csname val@fp:image/dHash-64/att/noise0.05/pct\endcsname{94}
\expandafter\def\csname val@fp:image/dHash-64/att/none\endcsname{0.99}
\expandafter\def\csname val@fp:image/dHash-64/att/none/pct\endcsname{99}
\expandafter\def\csname val@fp:image/dHash-64/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/perspective\endcsname{0.30}
\expandafter\def\csname val@fp:image/dHash-64/att/perspective/pct\endcsname{30}
\expandafter\def\csname val@fp:image/dHash-64/att/pixelize0.3\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/pixelize0.3/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/recapture\endcsname{0.53}
\expandafter\def\csname val@fp:image/dHash-64/att/recapture/pct\endcsname{53}
\expandafter\def\csname val@fp:image/dHash-64/att/resize0.25\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/resize0.25/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/resize0.5\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/resize0.5/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/rot5\endcsname{0.06}
\expandafter\def\csname val@fp:image/dHash-64/att/rot5/pct\endcsname{6}
\expandafter\def\csname val@fp:image/dHash-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/sat2\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/sat2/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/dHash-64/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/dHash-64/att/skew\endcsname{0.05}
\expandafter\def\csname val@fp:image/dHash-64/att/skew/pct\endcsname{5}
\expandafter\def\csname val@fp:image/dHash-64/att/social\endcsname{0.51}
\expandafter\def\csname val@fp:image/dHash-64/att/social/pct\endcsname{51}
\expandafter\def\csname val@fp:image/dHash-64/att/squash0.75\endcsname{0.99}
\expandafter\def\csname val@fp:image/dHash-64/att/squash0.75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/dHash-64/att/text\endcsname{0.94}
\expandafter\def\csname val@fp:image/dHash-64/att/text/pct\endcsname{94}
\expandafter\def\csname val@fp:image/dHash-64/att/webp50\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/att/webp50/pct\endcsname{98}
\expandafter\def\csname val@fp:image/dHash-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:image/dHash-64/disc\endcsname{0.195}
\expandafter\def\csname val@fp:image/dHash-64/fam/chain\endcsname{0.52}
\expandafter\def\csname val@fp:image/dHash-64/fam/compression\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/fam/crop\endcsname{0.11}
\expandafter\def\csname val@fp:image/dHash-64/fam/geometric\endcsname{0.07}
\expandafter\def\csname val@fp:image/dHash-64/fam/none\endcsname{0.99}
\expandafter\def\csname val@fp:image/dHash-64/fam/overlay\endcsname{0.38}
\expandafter\def\csname val@fp:image/dHash-64/fam/photometric\endcsname{0.93}
\expandafter\def\csname val@fp:image/dHash-64/fam/scale\endcsname{0.98}
\expandafter\def\csname val@fp:image/dHash-64/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/dHash-64/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/dHash-64/ms\endcsname{4.4}
\expandafter\def\csname val@fp:image/dHash-64/muAP\endcsname{0.356}
\expandafter\def\csname val@fp:image/dHash-64/muAP/pct\endcsname{35.6}
\expandafter\def\csname val@fp:image/fprq/max\endcsname{1.3}
\expandafter\def\csname val@fp:image/fprq/min\endcsname{0.2}
\expandafter\def\csname val@fp:image/pHash-256/FPRq@pair@1e-07\endcsname{0.011}
\expandafter\def\csname val@fp:image/pHash-256/FPRq@pair@1e-07/pct\endcsname{1.1}
\expandafter\def\csname val@fp:image/pHash-256/FPRq@query@0.01\endcsname{0.013}
\expandafter\def\csname val@fp:image/pHash-256/FPRq@query@0.01/pct\endcsname{1.3}
\expandafter\def\csname val@fp:image/pHash-256/R@1\endcsname{0.589}
\expandafter\def\csname val@fp:image/pHash-256/R@1/pct\endcsname{58.9}
\expandafter\def\csname val@fp:image/pHash-256/R@10\endcsname{0.625}
\expandafter\def\csname val@fp:image/pHash-256/R@10/pct\endcsname{62.5}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@0.0001\endcsname{0.582}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@0.0001/pct\endcsname{58.2}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-05\endcsname{0.541}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-05/pct\endcsname{54.1}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-06\endcsname{0.512}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-06/pct\endcsname{51.2}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-07\endcsname{0.492}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-07/pct\endcsname{49.2}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/pHash-256/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/pHash-256/TPR@query@0.01\endcsname{0.494}
\expandafter\def\csname val@fp:image/pHash-256/TPR@query@0.01/pct\endcsname{49.4}
\expandafter\def\csname val@fp:image/pHash-256/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/blur2\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/blur2/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/bright0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-256/att/bright0.6/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/bright1.4\endcsname{0.94}
\expandafter\def\csname val@fp:image/pHash-256/att/bright1.4/pct\endcsname{94}
\expandafter\def\csname val@fp:image/pHash-256/att/contrast0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/contrast0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/crop70\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/crop70/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/crop90\endcsname{0.48}
\expandafter\def\csname val@fp:image/pHash-256/att/crop90/pct\endcsname{48}
\expandafter\def\csname val@fp:image/pHash-256/att/emoji0.3\endcsname{0.89}
\expandafter\def\csname val@fp:image/pHash-256/att/emoji0.3/pct\endcsname{89}
\expandafter\def\csname val@fp:image/pHash-256/att/gamma0.6\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-256/att/gamma0.6/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-256/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg30\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg30/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg50\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg75\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/jpeg75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/meme\endcsname{0.08}
\expandafter\def\csname val@fp:image/pHash-256/att/meme/pct\endcsname{8}
\expandafter\def\csname val@fp:image/pHash-256/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-256/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-256/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/perspective\endcsname{0.38}
\expandafter\def\csname val@fp:image/pHash-256/att/perspective/pct\endcsname{38}
\expandafter\def\csname val@fp:image/pHash-256/att/pixelize0.3\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/pixelize0.3/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/recapture\endcsname{0.71}
\expandafter\def\csname val@fp:image/pHash-256/att/recapture/pct\endcsname{71}
\expandafter\def\csname val@fp:image/pHash-256/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/rot5\endcsname{0.25}
\expandafter\def\csname val@fp:image/pHash-256/att/rot5/pct\endcsname{25}
\expandafter\def\csname val@fp:image/pHash-256/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/sat2\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-256/att/sat2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-256/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-256/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-256/att/skew\endcsname{0.08}
\expandafter\def\csname val@fp:image/pHash-256/att/skew/pct\endcsname{8}
\expandafter\def\csname val@fp:image/pHash-256/att/social\endcsname{0.48}
\expandafter\def\csname val@fp:image/pHash-256/att/social/pct\endcsname{48}
\expandafter\def\csname val@fp:image/pHash-256/att/squash0.75\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/squash0.75/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/att/text\endcsname{0.98}
\expandafter\def\csname val@fp:image/pHash-256/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:image/pHash-256/att/webp50\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/att/webp50/pct\endcsname{100}
\expandafter\def\csname val@fp:image/pHash-256/bits\endcsname{256}
\expandafter\def\csname val@fp:image/pHash-256/disc\endcsname{0.302}
\expandafter\def\csname val@fp:image/pHash-256/fam/chain\endcsname{0.59}
\expandafter\def\csname val@fp:image/pHash-256/fam/compression\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/fam/crop\endcsname{0.10}
\expandafter\def\csname val@fp:image/pHash-256/fam/geometric\endcsname{0.10}
\expandafter\def\csname val@fp:image/pHash-256/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/fam/overlay\endcsname{0.39}
\expandafter\def\csname val@fp:image/pHash-256/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-256/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:image/pHash-256/hard\endcsname{0.001}
\expandafter\def\csname val@fp:image/pHash-256/hard/pct\endcsname{0.1}
\expandafter\def\csname val@fp:image/pHash-256/ms\endcsname{5.6}
\expandafter\def\csname val@fp:image/pHash-256/muAP\endcsname{0.520}
\expandafter\def\csname val@fp:image/pHash-256/muAP/pct\endcsname{52.0}
\expandafter\def\csname val@fp:image/pHash-64/FPRq@pair@1e-07\endcsname{0.003}
\expandafter\def\csname val@fp:image/pHash-64/FPRq@pair@1e-07/pct\endcsname{0.3}
\expandafter\def\csname val@fp:image/pHash-64/FPRq@query@0.01\endcsname{0.003}
\expandafter\def\csname val@fp:image/pHash-64/FPRq@query@0.01/pct\endcsname{0.3}
\expandafter\def\csname val@fp:image/pHash-64/R@1\endcsname{0.563}
\expandafter\def\csname val@fp:image/pHash-64/R@1/pct\endcsname{56.3}
\expandafter\def\csname val@fp:image/pHash-64/R@10\endcsname{0.617}
\expandafter\def\csname val@fp:image/pHash-64/R@10/pct\endcsname{61.7}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@0.0001\endcsname{0.547}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@0.0001/pct\endcsname{54.7}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-05\endcsname{0.496}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-05/pct\endcsname{49.6}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-06\endcsname{0.452}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-06/pct\endcsname{45.2}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-07\endcsname{0.373}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-07/pct\endcsname{37.3}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/pHash-64/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/pHash-64/TPR@query@0.01\endcsname{0.373}
\expandafter\def\csname val@fp:image/pHash-64/TPR@query@0.01/pct\endcsname{37.3}
\expandafter\def\csname val@fp:image/pHash-64/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/blur2\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/blur2/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/bright0.6\endcsname{0.98}
\expandafter\def\csname val@fp:image/pHash-64/att/bright0.6/pct\endcsname{98}
\expandafter\def\csname val@fp:image/pHash-64/att/bright1.4\endcsname{0.82}
\expandafter\def\csname val@fp:image/pHash-64/att/bright1.4/pct\endcsname{82}
\expandafter\def\csname val@fp:image/pHash-64/att/contrast0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/contrast0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/crop70\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/crop70/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/crop90\endcsname{0.56}
\expandafter\def\csname val@fp:image/pHash-64/att/crop90/pct\endcsname{56}
\expandafter\def\csname val@fp:image/pHash-64/att/emoji0.3\endcsname{0.54}
\expandafter\def\csname val@fp:image/pHash-64/att/emoji0.3/pct\endcsname{54}
\expandafter\def\csname val@fp:image/pHash-64/att/gamma0.6\endcsname{0.97}
\expandafter\def\csname val@fp:image/pHash-64/att/gamma0.6/pct\endcsname{97}
\expandafter\def\csname val@fp:image/pHash-64/att/gray\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/gray/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg30\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg30/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg50\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg75\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/jpeg75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/meme\endcsname{0.08}
\expandafter\def\csname val@fp:image/pHash-64/att/meme/pct\endcsname{8}
\expandafter\def\csname val@fp:image/pHash-64/att/noise0.05\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/noise0.05/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/none\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/none/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/perspective\endcsname{0.26}
\expandafter\def\csname val@fp:image/pHash-64/att/perspective/pct\endcsname{26}
\expandafter\def\csname val@fp:image/pHash-64/att/pixelize0.3\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/pixelize0.3/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/recapture\endcsname{0.49}
\expandafter\def\csname val@fp:image/pHash-64/att/recapture/pct\endcsname{49}
\expandafter\def\csname val@fp:image/pHash-64/att/resize0.25\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/resize0.25/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/rot5\endcsname{0.20}
\expandafter\def\csname val@fp:image/pHash-64/att/rot5/pct\endcsname{20}
\expandafter\def\csname val@fp:image/pHash-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/sat2\endcsname{0.98}
\expandafter\def\csname val@fp:image/pHash-64/att/sat2/pct\endcsname{98}
\expandafter\def\csname val@fp:image/pHash-64/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/pHash-64/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/pHash-64/att/skew\endcsname{0.06}
\expandafter\def\csname val@fp:image/pHash-64/att/skew/pct\endcsname{6}
\expandafter\def\csname val@fp:image/pHash-64/att/social\endcsname{0.56}
\expandafter\def\csname val@fp:image/pHash-64/att/social/pct\endcsname{56}
\expandafter\def\csname val@fp:image/pHash-64/att/squash0.75\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/squash0.75/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/att/text\endcsname{0.89}
\expandafter\def\csname val@fp:image/pHash-64/att/text/pct\endcsname{89}
\expandafter\def\csname val@fp:image/pHash-64/att/webp50\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/att/webp50/pct\endcsname{99}
\expandafter\def\csname val@fp:image/pHash-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:image/pHash-64/disc\endcsname{0.240}
\expandafter\def\csname val@fp:image/pHash-64/fam/chain\endcsname{0.52}
\expandafter\def\csname val@fp:image/pHash-64/fam/compression\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/fam/crop\endcsname{0.11}
\expandafter\def\csname val@fp:image/pHash-64/fam/geometric\endcsname{0.08}
\expandafter\def\csname val@fp:image/pHash-64/fam/none\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/fam/overlay\endcsname{0.30}
\expandafter\def\csname val@fp:image/pHash-64/fam/photometric\endcsname{0.97}
\expandafter\def\csname val@fp:image/pHash-64/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:image/pHash-64/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/pHash-64/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/pHash-64/ms\endcsname{5.2}
\expandafter\def\csname val@fp:image/pHash-64/muAP\endcsname{0.469}
\expandafter\def\csname val@fp:image/pHash-64/muAP/pct\endcsname{46.9}
\expandafter\def\csname val@fp:image/pos_sources\endcsname{2{,}000}
\expandafter\def\csname val@fp:image/wHash-64/FPRq@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/FPRq@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/FPRq@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/FPRq@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/R@1\endcsname{0.425}
\expandafter\def\csname val@fp:image/wHash-64/R@1/pct\endcsname{42.5}
\expandafter\def\csname val@fp:image/wHash-64/R@10\endcsname{0.498}
\expandafter\def\csname val@fp:image/wHash-64/R@10/pct\endcsname{49.8}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@0.0001\endcsname{0.380}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@0.0001/pct\endcsname{38.0}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-05\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-05/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-06\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-06/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-07/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-08\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/TPR@pair@1e-08/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/TPR@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/TPR@query@0.01/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/att/background0.5\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/background0.5/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/blur2\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/blur2/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/bright0.6\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/bright0.6/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/bright1.4\endcsname{0.48}
\expandafter\def\csname val@fp:image/wHash-64/att/bright1.4/pct\endcsname{48}
\expandafter\def\csname val@fp:image/wHash-64/att/contrast0.5\endcsname{0.74}
\expandafter\def\csname val@fp:image/wHash-64/att/contrast0.5/pct\endcsname{74}
\expandafter\def\csname val@fp:image/wHash-64/att/crop30\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/crop30/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/crop50off\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/crop50off/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/crop70\endcsname{0.02}
\expandafter\def\csname val@fp:image/wHash-64/att/crop70/pct\endcsname{2}
\expandafter\def\csname val@fp:image/wHash-64/att/crop90\endcsname{0.35}
\expandafter\def\csname val@fp:image/wHash-64/att/crop90/pct\endcsname{35}
\expandafter\def\csname val@fp:image/wHash-64/att/emoji0.3\endcsname{0.56}
\expandafter\def\csname val@fp:image/wHash-64/att/emoji0.3/pct\endcsname{56}
\expandafter\def\csname val@fp:image/wHash-64/att/gamma0.6\endcsname{0.73}
\expandafter\def\csname val@fp:image/wHash-64/att/gamma0.6/pct\endcsname{73}
\expandafter\def\csname val@fp:image/wHash-64/att/gray\endcsname{0.91}
\expandafter\def\csname val@fp:image/wHash-64/att/gray/pct\endcsname{90}
\expandafter\def\csname val@fp:image/wHash-64/att/hflip\endcsname{0.07}
\expandafter\def\csname val@fp:image/wHash-64/att/hflip/pct\endcsname{7}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg30\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg30/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg50\endcsname{0.76}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg50/pct\endcsname{76}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg75\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/jpeg75/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/meme\endcsname{0.03}
\expandafter\def\csname val@fp:image/wHash-64/att/meme/pct\endcsname{3}
\expandafter\def\csname val@fp:image/wHash-64/att/noise0.05\endcsname{0.72}
\expandafter\def\csname val@fp:image/wHash-64/att/noise0.05/pct\endcsname{72}
\expandafter\def\csname val@fp:image/wHash-64/att/none\endcsname{0.91}
\expandafter\def\csname val@fp:image/wHash-64/att/none/pct\endcsname{90}
\expandafter\def\csname val@fp:image/wHash-64/att/pad25\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/pad25/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/perspective\endcsname{0.16}
\expandafter\def\csname val@fp:image/wHash-64/att/perspective/pct\endcsname{16}
\expandafter\def\csname val@fp:image/wHash-64/att/pixelize0.3\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/pixelize0.3/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/recapture\endcsname{0.27}
\expandafter\def\csname val@fp:image/wHash-64/att/recapture/pct\endcsname{27}
\expandafter\def\csname val@fp:image/wHash-64/att/resize0.25\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/att/resize0.25/pct\endcsname{75}
\expandafter\def\csname val@fp:image/wHash-64/att/resize0.5\endcsname{0.76}
\expandafter\def\csname val@fp:image/wHash-64/att/resize0.5/pct\endcsname{76}
\expandafter\def\csname val@fp:image/wHash-64/att/rot15\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/rot15/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/rot5\endcsname{0.02}
\expandafter\def\csname val@fp:image/wHash-64/att/rot5/pct\endcsname{2}
\expandafter\def\csname val@fp:image/wHash-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/sat2\endcsname{0.76}
\expandafter\def\csname val@fp:image/wHash-64/att/sat2/pct\endcsname{76}
\expandafter\def\csname val@fp:image/wHash-64/att/screenshot\endcsname{0.00}
\expandafter\def\csname val@fp:image/wHash-64/att/screenshot/pct\endcsname{0}
\expandafter\def\csname val@fp:image/wHash-64/att/skew\endcsname{0.06}
\expandafter\def\csname val@fp:image/wHash-64/att/skew/pct\endcsname{6}
\expandafter\def\csname val@fp:image/wHash-64/att/social\endcsname{0.35}
\expandafter\def\csname val@fp:image/wHash-64/att/social/pct\endcsname{35}
\expandafter\def\csname val@fp:image/wHash-64/att/squash0.75\endcsname{0.76}
\expandafter\def\csname val@fp:image/wHash-64/att/squash0.75/pct\endcsname{76}
\expandafter\def\csname val@fp:image/wHash-64/att/text\endcsname{0.62}
\expandafter\def\csname val@fp:image/wHash-64/att/text/pct\endcsname{62}
\expandafter\def\csname val@fp:image/wHash-64/att/webp50\endcsname{0.74}
\expandafter\def\csname val@fp:image/wHash-64/att/webp50/pct\endcsname{74}
\expandafter\def\csname val@fp:image/wHash-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:image/wHash-64/disc\endcsname{0.024}
\expandafter\def\csname val@fp:image/wHash-64/fam/chain\endcsname{0.31}
\expandafter\def\csname val@fp:image/wHash-64/fam/compression\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/fam/crop\endcsname{0.07}
\expandafter\def\csname val@fp:image/wHash-64/fam/geometric\endcsname{0.05}
\expandafter\def\csname val@fp:image/wHash-64/fam/none\endcsname{0.91}
\expandafter\def\csname val@fp:image/wHash-64/fam/overlay\endcsname{0.24}
\expandafter\def\csname val@fp:image/wHash-64/fam/photometric\endcsname{0.73}
\expandafter\def\csname val@fp:image/wHash-64/fam/scale\endcsname{0.75}
\expandafter\def\csname val@fp:image/wHash-64/hard\endcsname{0.000}
\expandafter\def\csname val@fp:image/wHash-64/hard/pct\endcsname{0.0}
\expandafter\def\csname val@fp:image/wHash-64/ms\endcsname{63}
\expandafter\def\csname val@fp:image/wHash-64/muAP\endcsname{0.134}
\expandafter\def\csname val@fp:image/wHash-64/muAP/pct\endcsname{13.4}
\expandafter\def\csname val@fp:lat/audio/CLAP\endcsname{1.1}
\expandafter\def\csname val@fp:lat/audio/Chromaprint\endcsname{2.0}
\expandafter\def\csname val@fp:lat/audio/ISCC-Audio-256\endcsname{2.0}
\expandafter\def\csname val@fp:lat/audio/ISCC-Audio-64\endcsname{2.0}
\expandafter\def\csname val@fp:lat/audio/audfprint\endcsname{1.4}
\expandafter\def\csname val@fp:lat/image/BlockMean\endcsname{1.0}
\expandafter\def\csname val@fp:lat/image/BlockMean/usd1m\endcsname{0.04}
\expandafter\def\csname val@fp:lat/image/Blockhash-256\endcsname{19}
\expandafter\def\csname val@fp:lat/image/Blockhash-256/usd1m\endcsname{0.80}
\expandafter\def\csname val@fp:lat/image/ColorMoment\endcsname{3.6}
\expandafter\def\csname val@fp:lat/image/ColorMoment/usd1m\endcsname{0.15}
\expandafter\def\csname val@fp:lat/image/DINOHash-96\endcsname{3.6}
\expandafter\def\csname val@fp:lat/image/DINOHash-96/usd1m\endcsname{1.22}
\expandafter\def\csname val@fp:lat/image/DINOv2-B\endcsname{3.9}
\expandafter\def\csname val@fp:lat/image/DINOv2-B/usd1m\endcsname{1.31}
\expandafter\def\csname val@fp:lat/image/DINOv2-S\endcsname{2.0}
\expandafter\def\csname val@fp:lat/image/DINOv2-S-LSH256\endcsname{1.7}
\expandafter\def\csname val@fp:lat/image/DINOv2-S-LSH256/usd1m\endcsname{0.56}
\expandafter\def\csname val@fp:lat/image/DINOv2-S/usd1m\endcsname{0.66}
\expandafter\def\csname val@fp:lat/image/ISC21-1st\endcsname{8.3}
\expandafter\def\csname val@fp:lat/image/ISC21-1st/usd1m\endcsname{2.81}
\expandafter\def\csname val@fp:lat/image/ISCC-Image-256\endcsname{11}
\expandafter\def\csname val@fp:lat/image/ISCC-Image-256/usd1m\endcsname{0.47}
\expandafter\def\csname val@fp:lat/image/ISCC-Image-64\endcsname{11}
\expandafter\def\csname val@fp:lat/image/ISCC-Image-64/usd1m\endcsname{0.47}
\expandafter\def\csname val@fp:lat/image/MarrHildreth\endcsname{5.5}
\expandafter\def\csname val@fp:lat/image/MarrHildreth/usd1m\endcsname{0.23}
\expandafter\def\csname val@fp:lat/image/OpenCLIP-B32\endcsname{1.1}
\expandafter\def\csname val@fp:lat/image/OpenCLIP-B32/usd1m\endcsname{0.37}
\expandafter\def\csname val@fp:lat/image/PDQ\endcsname{31}
\expandafter\def\csname val@fp:lat/image/PDQ-dihedral\endcsname{31}
\expandafter\def\csname val@fp:lat/image/PDQ-dihedral/usd1m\endcsname{1.29}
\expandafter\def\csname val@fp:lat/image/PDQ/usd1m\endcsname{1.29}
\expandafter\def\csname val@fp:lat/image/SSCD-large\endcsname{4.6}
\expandafter\def\csname val@fp:lat/image/SSCD-large/usd1m\endcsname{1.56}
\expandafter\def\csname val@fp:lat/image/SSCD-mixup\endcsname{2.7}
\expandafter\def\csname val@fp:lat/image/SSCD-mixup/usd1m\endcsname{0.89}
\expandafter\def\csname val@fp:lat/image/aHash-64\endcsname{4.3}
\expandafter\def\csname val@fp:lat/image/aHash-64/usd1m\endcsname{0.18}
\expandafter\def\csname val@fp:lat/image/dHash-64\endcsname{4.4}
\expandafter\def\csname val@fp:lat/image/dHash-64/usd1m\endcsname{0.18}
\expandafter\def\csname val@fp:lat/image/pHash-256\endcsname{5.6}
\expandafter\def\csname val@fp:lat/image/pHash-256/usd1m\endcsname{0.24}
\expandafter\def\csname val@fp:lat/image/pHash-64\endcsname{5.2}
\expandafter\def\csname val@fp:lat/image/pHash-64/usd1m\endcsname{0.22}
\expandafter\def\csname val@fp:lat/image/wHash-64\endcsname{63}
\expandafter\def\csname val@fp:lat/image/wHash-64/usd1m\endcsname{2.66}
\expandafter\def\csname val@fp:lat/video/DINOv2-S-seq\endcsname{136}
\expandafter\def\csname val@fp:lat/video/ISCC-Video-256\endcsname{54}
\expandafter\def\csname val@fp:lat/video/ISCC-Video-64\endcsname{54}
\expandafter\def\csname val@fp:lat/video/SSCD-mixup-seq\endcsname{137}
\expandafter\def\csname val@fp:lat/video/TMK+PDQF\endcsname{51}
\expandafter\def\csname val@fp:lat/video/vPDQ\endcsname{132}
\expandafter\def\csname val@fp:loc/e2e/lightglue/BlockMean/fused/f1\endcsname{0.41}
\expandafter\def\csname val@fp:loc/e2e/lightglue/BlockMean/lpips/f1\endcsname{0.36}
\expandafter\def\csname val@fp:loc/e2e/lightglue/BlockMean/pixel/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/e2e/lightglue/BlockMean/retrieved\endcsname{64.9}
\expandafter\def\csname val@fp:loc/e2e/lightglue/BlockMean/retrieved_aligned\endcsname{64.8}
\expandafter\def\csname val@fp:loc/e2e/lightglue/Blockhash-256/fused/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/e2e/lightglue/Blockhash-256/lpips/f1\endcsname{0.38}
\expandafter\def\csname val@fp:loc/e2e/lightglue/Blockhash-256/pixel/f1\endcsname{0.46}
\expandafter\def\csname val@fp:loc/e2e/lightglue/Blockhash-256/retrieved\endcsname{67.6}
\expandafter\def\csname val@fp:loc/e2e/lightglue/Blockhash-256/retrieved_aligned\endcsname{67.4}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ColorMoment/fused/f1\endcsname{0.08}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ColorMoment/lpips/f1\endcsname{0.07}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ColorMoment/pixel/f1\endcsname{0.08}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ColorMoment/retrieved\endcsname{14.0}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ColorMoment/retrieved_aligned\endcsname{14.0}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOHash-96/fused/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOHash-96/lpips/f1\endcsname{0.43}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOHash-96/pixel/f1\endcsname{0.52}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOHash-96/retrieved\endcsname{75.6}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOHash-96/retrieved_aligned\endcsname{75.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-B/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-B/lpips/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-B/pixel/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-B/retrieved\endcsname{92.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-B/retrieved_aligned\endcsname{91.7}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S-LSH256/fused/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S-LSH256/lpips/f1\endcsname{0.52}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S-LSH256/pixel/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S-LSH256/retrieved\endcsname{86.8}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S-LSH256/retrieved_aligned\endcsname{86.2}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S/lpips/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S/pixel/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S/retrieved\endcsname{92.7}
\expandafter\def\csname val@fp:loc/e2e/lightglue/DINOv2-S/retrieved_aligned\endcsname{92.2}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISC21-1st/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISC21-1st/lpips/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISC21-1st/pixel/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISC21-1st/retrieved\endcsname{92.5}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISC21-1st/retrieved_aligned\endcsname{91.9}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-256/fused/f1\endcsname{0.32}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-256/lpips/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-256/pixel/f1\endcsname{0.33}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-256/retrieved\endcsname{50.4}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-256/retrieved_aligned\endcsname{50.4}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-64/fused/f1\endcsname{0.31}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-64/lpips/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-64/pixel/f1\endcsname{0.32}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-64/retrieved\endcsname{49.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/ISCC-Image-64/retrieved_aligned\endcsname{49.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/MarrHildreth/fused/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/e2e/lightglue/MarrHildreth/lpips/f1\endcsname{0.47}
\expandafter\def\csname val@fp:loc/e2e/lightglue/MarrHildreth/pixel/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/e2e/lightglue/MarrHildreth/retrieved\endcsname{78.2}
\expandafter\def\csname val@fp:loc/e2e/lightglue/MarrHildreth/retrieved_aligned\endcsname{77.8}
\expandafter\def\csname val@fp:loc/e2e/lightglue/OpenCLIP-B32/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/lightglue/OpenCLIP-B32/lpips/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/e2e/lightglue/OpenCLIP-B32/pixel/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/e2e/lightglue/OpenCLIP-B32/retrieved\endcsname{92.4}
\expandafter\def\csname val@fp:loc/e2e/lightglue/OpenCLIP-B32/retrieved_aligned\endcsname{91.9}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ-dihedral/fused/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ-dihedral/lpips/f1\endcsname{0.39}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ-dihedral/pixel/f1\endcsname{0.47}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ-dihedral/retrieved\endcsname{66.8}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ-dihedral/retrieved_aligned\endcsname{66.5}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ/fused/f1\endcsname{0.47}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ/lpips/f1\endcsname{0.42}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ/pixel/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ/retrieved\endcsname{70.7}
\expandafter\def\csname val@fp:loc/e2e/lightglue/PDQ/retrieved_aligned\endcsname{70.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-large/fused/f1\endcsname{0.67}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-large/lpips/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-large/pixel/f1\endcsname{0.70}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-large/retrieved\endcsname{97.7}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-large/retrieved_aligned\endcsname{97.0}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-mixup/fused/f1\endcsname{0.67}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-mixup/lpips/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-mixup/pixel/f1\endcsname{0.70}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-mixup/retrieved\endcsname{97.6}
\expandafter\def\csname val@fp:loc/e2e/lightglue/SSCD-mixup/retrieved_aligned\endcsname{96.9}
\expandafter\def\csname val@fp:loc/e2e/lightglue/aHash-64/fused/f1\endcsname{0.31}
\expandafter\def\csname val@fp:loc/e2e/lightglue/aHash-64/lpips/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/lightglue/aHash-64/pixel/f1\endcsname{0.33}
\expandafter\def\csname val@fp:loc/e2e/lightglue/aHash-64/retrieved\endcsname{50.1}
\expandafter\def\csname val@fp:loc/e2e/lightglue/aHash-64/retrieved_aligned\endcsname{50.1}
\expandafter\def\csname val@fp:loc/e2e/lightglue/dHash-64/fused/f1\endcsname{0.43}
\expandafter\def\csname val@fp:loc/e2e/lightglue/dHash-64/lpips/f1\endcsname{0.38}
\expandafter\def\csname val@fp:loc/e2e/lightglue/dHash-64/pixel/f1\endcsname{0.46}
\expandafter\def\csname val@fp:loc/e2e/lightglue/dHash-64/retrieved\endcsname{66.5}
\expandafter\def\csname val@fp:loc/e2e/lightglue/dHash-64/retrieved_aligned\endcsname{66.3}
\expandafter\def\csname val@fp:loc/e2e/lightglue/n\endcsname{3{,}000}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-256/fused/f1\endcsname{0.48}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-256/lpips/f1\endcsname{0.42}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-256/pixel/f1\endcsname{0.51}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-256/retrieved\endcsname{72.1}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-256/retrieved_aligned\endcsname{71.8}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-64/fused/f1\endcsname{0.31}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-64/lpips/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-64/pixel/f1\endcsname{0.33}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-64/retrieved\endcsname{50.6}
\expandafter\def\csname val@fp:loc/e2e/lightglue/pHash-64/retrieved_aligned\endcsname{50.5}
\expandafter\def\csname val@fp:loc/e2e/lightglue/wHash-64/fused/f1\endcsname{0.26}
\expandafter\def\csname val@fp:loc/e2e/lightglue/wHash-64/lpips/f1\endcsname{0.22}
\expandafter\def\csname val@fp:loc/e2e/lightglue/wHash-64/pixel/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/lightglue/wHash-64/retrieved\endcsname{40.1}
\expandafter\def\csname val@fp:loc/e2e/lightglue/wHash-64/retrieved_aligned\endcsname{40.1}
\expandafter\def\csname val@fp:loc/e2e/sift/BlockMean/fused/f1\endcsname{0.38}
\expandafter\def\csname val@fp:loc/e2e/sift/BlockMean/lpips/f1\endcsname{0.39}
\expandafter\def\csname val@fp:loc/e2e/sift/BlockMean/pixel/f1\endcsname{0.47}
\expandafter\def\csname val@fp:loc/e2e/sift/BlockMean/retrieved\endcsname{64.9}
\expandafter\def\csname val@fp:loc/e2e/sift/BlockMean/retrieved_aligned\endcsname{63.4}
\expandafter\def\csname val@fp:loc/e2e/sift/Blockhash-256/fused/f1\endcsname{0.41}
\expandafter\def\csname val@fp:loc/e2e/sift/Blockhash-256/lpips/f1\endcsname{0.41}
\expandafter\def\csname val@fp:loc/e2e/sift/Blockhash-256/pixel/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/sift/Blockhash-256/retrieved\endcsname{67.6}
\expandafter\def\csname val@fp:loc/e2e/sift/Blockhash-256/retrieved_aligned\endcsname{65.9}
\expandafter\def\csname val@fp:loc/e2e/sift/ColorMoment/fused/f1\endcsname{0.07}
\expandafter\def\csname val@fp:loc/e2e/sift/ColorMoment/lpips/f1\endcsname{0.07}
\expandafter\def\csname val@fp:loc/e2e/sift/ColorMoment/pixel/f1\endcsname{0.09}
\expandafter\def\csname val@fp:loc/e2e/sift/ColorMoment/retrieved\endcsname{14.0}
\expandafter\def\csname val@fp:loc/e2e/sift/ColorMoment/retrieved_aligned\endcsname{13.7}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOHash-96/fused/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOHash-96/lpips/f1\endcsname{0.46}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOHash-96/pixel/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOHash-96/retrieved\endcsname{75.6}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOHash-96/retrieved_aligned\endcsname{73.0}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-B/fused/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-B/lpips/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-B/pixel/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-B/retrieved\endcsname{92.3}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-B/retrieved_aligned\endcsname{88.7}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S-LSH256/fused/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S-LSH256/lpips/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S-LSH256/pixel/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S-LSH256/retrieved\endcsname{86.8}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S-LSH256/retrieved_aligned\endcsname{83.5}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S/fused/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S/lpips/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S/pixel/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S/retrieved\endcsname{92.7}
\expandafter\def\csname val@fp:loc/e2e/sift/DINOv2-S/retrieved_aligned\endcsname{89.1}
\expandafter\def\csname val@fp:loc/e2e/sift/ISC21-1st/fused/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/ISC21-1st/lpips/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/ISC21-1st/pixel/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/e2e/sift/ISC21-1st/retrieved\endcsname{92.5}
\expandafter\def\csname val@fp:loc/e2e/sift/ISC21-1st/retrieved_aligned\endcsname{89.2}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-256/fused/f1\endcsname{0.28}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-256/lpips/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-256/pixel/f1\endcsname{0.36}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-256/retrieved\endcsname{50.4}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-256/retrieved_aligned\endcsname{49.5}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-64/fused/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-64/lpips/f1\endcsname{0.28}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-64/pixel/f1\endcsname{0.35}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-64/retrieved\endcsname{49.3}
\expandafter\def\csname val@fp:loc/e2e/sift/ISCC-Image-64/retrieved_aligned\endcsname{48.4}
\expandafter\def\csname val@fp:loc/e2e/sift/MarrHildreth/fused/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/sift/MarrHildreth/lpips/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/sift/MarrHildreth/pixel/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/MarrHildreth/retrieved\endcsname{78.2}
\expandafter\def\csname val@fp:loc/e2e/sift/MarrHildreth/retrieved_aligned\endcsname{75.4}
\expandafter\def\csname val@fp:loc/e2e/sift/OpenCLIP-B32/fused/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/e2e/sift/OpenCLIP-B32/lpips/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/e2e/sift/OpenCLIP-B32/pixel/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/e2e/sift/OpenCLIP-B32/retrieved\endcsname{92.4}
\expandafter\def\csname val@fp:loc/e2e/sift/OpenCLIP-B32/retrieved_aligned\endcsname{89.1}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ-dihedral/fused/f1\endcsname{0.41}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ-dihedral/lpips/f1\endcsname{0.42}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ-dihedral/pixel/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ-dihedral/retrieved\endcsname{66.8}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ-dihedral/retrieved_aligned\endcsname{65.4}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ/fused/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ/lpips/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ/pixel/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ/retrieved\endcsname{70.7}
\expandafter\def\csname val@fp:loc/e2e/sift/PDQ/retrieved_aligned\endcsname{69.2}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-large/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-large/lpips/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-large/pixel/f1\endcsname{0.73}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-large/retrieved\endcsname{97.7}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-large/retrieved_aligned\endcsname{93.8}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-mixup/fused/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-mixup/lpips/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-mixup/pixel/f1\endcsname{0.73}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-mixup/retrieved\endcsname{97.6}
\expandafter\def\csname val@fp:loc/e2e/sift/SSCD-mixup/retrieved_aligned\endcsname{93.7}
\expandafter\def\csname val@fp:loc/e2e/sift/aHash-64/fused/f1\endcsname{0.28}
\expandafter\def\csname val@fp:loc/e2e/sift/aHash-64/lpips/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/e2e/sift/aHash-64/pixel/f1\endcsname{0.36}
\expandafter\def\csname val@fp:loc/e2e/sift/aHash-64/retrieved\endcsname{50.1}
\expandafter\def\csname val@fp:loc/e2e/sift/aHash-64/retrieved_aligned\endcsname{48.9}
\expandafter\def\csname val@fp:loc/e2e/sift/dHash-64/fused/f1\endcsname{0.40}
\expandafter\def\csname val@fp:loc/e2e/sift/dHash-64/lpips/f1\endcsname{0.41}
\expandafter\def\csname val@fp:loc/e2e/sift/dHash-64/pixel/f1\endcsname{0.49}
\expandafter\def\csname val@fp:loc/e2e/sift/dHash-64/retrieved\endcsname{66.5}
\expandafter\def\csname val@fp:loc/e2e/sift/dHash-64/retrieved_aligned\endcsname{64.8}
\expandafter\def\csname val@fp:loc/e2e/sift/n\endcsname{3{,}000}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-256/fused/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-256/lpips/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-256/pixel/f1\endcsname{0.54}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-256/retrieved\endcsname{72.1}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-256/retrieved_aligned\endcsname{70.3}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-64/fused/f1\endcsname{0.27}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-64/lpips/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-64/pixel/f1\endcsname{0.35}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-64/retrieved\endcsname{50.6}
\expandafter\def\csname val@fp:loc/e2e/sift/pHash-64/retrieved_aligned\endcsname{49.4}
\expandafter\def\csname val@fp:loc/e2e/sift/wHash-64/fused/f1\endcsname{0.24}
\expandafter\def\csname val@fp:loc/e2e/sift/wHash-64/lpips/f1\endcsname{0.24}
\expandafter\def\csname val@fp:loc/e2e/sift/wHash-64/pixel/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/e2e/sift/wHash-64/retrieved\endcsname{40.1}
\expandafter\def\csname val@fp:loc/e2e/sift/wHash-64/retrieved_aligned\endcsname{39.3}
\expandafter\def\csname val@fp:loc/lightglue/aligned\endcsname{99.0}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.01/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.01/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.03/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.03/f1\endcsname{0.49}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.1/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.1/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.25/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/dino/area/0.25/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/lightglue/dino/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/dino/best_f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/lightglue/dino/f1\endcsname{0.52}
\expandafter\def\csname val@fp:loc/lightglue/dino/iou\endcsname{0.42}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/crop90/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/crop90/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/jpeg75/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/jpeg75/f1\endcsname{0.57}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/none/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/none/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/resize0.75_jpeg80/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/dino/post/resize0.75_jpeg80/f1\endcsname{0.48}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/copymove/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/copymove/f1\endcsname{0.51}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/inpaint-lama/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/inpaint-lama/f1\endcsname{0.24}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/inpaint-telea/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/inpaint-telea/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/recolor/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/recolor/f1\endcsname{0.30}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/splice/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/splice/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/lightglue/dino/type/textreplace/f1\endcsname{0.81}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.01/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.01/f1\endcsname{0.51}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.03/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.03/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.1/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.1/f1\endcsname{0.78}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.25/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/fused/area/0.25/f1\endcsname{0.82}
\expandafter\def\csname val@fp:loc/lightglue/fused/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/best_f1\endcsname{0.79}
\expandafter\def\csname val@fp:loc/lightglue/fused/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/lightglue/fused/iou\endcsname{0.56}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/crop90/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/crop90/f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/jpeg75/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/jpeg75/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/none/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/none/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/resize0.75_jpeg80/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/fused/post/resize0.75_jpeg80/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/copymove/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/copymove/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/inpaint-lama/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/inpaint-lama/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/inpaint-telea/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/inpaint-telea/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/recolor/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/recolor/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/splice/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/splice/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/lightglue/fused/type/textreplace/f1\endcsname{0.83}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.01/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.01/f1\endcsname{0.39}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.03/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.03/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.1/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.1/f1\endcsname{0.73}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.25/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/lpips/area/0.25/f1\endcsname{0.80}
\expandafter\def\csname val@fp:loc/lightglue/lpips/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/lpips/best_f1\endcsname{0.78}
\expandafter\def\csname val@fp:loc/lightglue/lpips/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/lightglue/lpips/iou\endcsname{0.48}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/crop90/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/crop90/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/jpeg75/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/jpeg75/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/none/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/none/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/resize0.75_jpeg80/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/lightglue/lpips/post/resize0.75_jpeg80/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/copymove/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/copymove/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/inpaint-lama/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/inpaint-lama/f1\endcsname{0.40}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/inpaint-telea/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/inpaint-telea/f1\endcsname{0.70}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/recolor/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/recolor/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/splice/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/splice/f1\endcsname{0.62}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/lightglue/lpips/type/textreplace/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/lightglue/n\endcsname{3{,}000}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.01/auc\endcsname{0.85}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.01/f1\endcsname{0.00}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.03/auc\endcsname{0.89}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.03/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.1/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.1/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.25/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/lightglue/pdq/area/0.25/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/lightglue/pdq/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/lightglue/pdq/best_f1\endcsname{0.49}
\expandafter\def\csname val@fp:loc/lightglue/pdq/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/iou\endcsname{0.01}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/crop90/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/crop90/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/jpeg75/auc\endcsname{0.84}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/jpeg75/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/none/auc\endcsname{0.85}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/none/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/resize0.75_jpeg80/auc\endcsname{0.83}
\expandafter\def\csname val@fp:loc/lightglue/pdq/post/resize0.75_jpeg80/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/copymove/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/copymove/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/inpaint-lama/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/inpaint-lama/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/inpaint-telea/auc\endcsname{0.88}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/inpaint-telea/f1\endcsname{0.03}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/recolor/auc\endcsname{0.81}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/recolor/f1\endcsname{0.01}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/splice/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/splice/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/textreplace/auc\endcsname{0.89}
\expandafter\def\csname val@fp:loc/lightglue/pdq/type/textreplace/f1\endcsname{0.03}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.01/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.01/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.03/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.03/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.1/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.1/f1\endcsname{0.82}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.25/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/lightglue/pixel/area/0.25/f1\endcsname{0.82}
\expandafter\def\csname val@fp:loc/lightglue/pixel/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/pixel/best_f1\endcsname{0.82}
\expandafter\def\csname val@fp:loc/lightglue/pixel/f1\endcsname{0.72}
\expandafter\def\csname val@fp:loc/lightglue/pixel/iou\endcsname{0.60}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/crop90/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/crop90/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/jpeg75/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/jpeg75/f1\endcsname{0.78}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/none/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/none/f1\endcsname{0.73}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/resize0.75_jpeg80/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/pixel/post/resize0.75_jpeg80/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/copymove/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/copymove/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/inpaint-lama/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/inpaint-lama/f1\endcsname{0.55}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/inpaint-telea/auc\endcsname{0.90}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/inpaint-telea/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/recolor/auc\endcsname{1.00}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/recolor/f1\endcsname{0.78}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/splice/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/splice/f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/textreplace/auc\endcsname{1.00}
\expandafter\def\csname val@fp:loc/lightglue/pixel/type/textreplace/f1\endcsname{0.90}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.01/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.01/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.03/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.03/f1\endcsname{0.62}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.1/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.1/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.25/auc\endcsname{0.88}
\expandafter\def\csname val@fp:loc/lightglue/ssim/area/0.25/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/lightglue/ssim/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/ssim/best_f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/lightglue/ssim/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/lightglue/ssim/iou\endcsname{0.46}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/crop90/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/crop90/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/jpeg75/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/jpeg75/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/none/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/none/f1\endcsname{0.62}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/resize0.75_jpeg80/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/lightglue/ssim/post/resize0.75_jpeg80/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/copymove/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/copymove/f1\endcsname{0.62}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/inpaint-lama/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/inpaint-lama/f1\endcsname{0.44}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/inpaint-telea/auc\endcsname{0.88}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/inpaint-telea/f1\endcsname{0.58}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/recolor/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/recolor/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/splice/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/splice/f1\endcsname{0.67}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/textreplace/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/lightglue/ssim/type/textreplace/f1\endcsname{0.76}
\expandafter\def\csname val@fp:loc/sift/aligned\endcsname{95.6}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.01/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.01/f1\endcsname{0.31}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.03/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.03/f1\endcsname{0.49}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.1/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.1/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.25/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/dino/area/0.25/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/sift/dino/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/dino/best_f1\endcsname{0.70}
\expandafter\def\csname val@fp:loc/sift/dino/f1\endcsname{0.53}
\expandafter\def\csname val@fp:loc/sift/dino/iou\endcsname{0.43}
\expandafter\def\csname val@fp:loc/sift/dino/post/crop90/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/dino/post/crop90/f1\endcsname{0.51}
\expandafter\def\csname val@fp:loc/sift/dino/post/jpeg75/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/dino/post/jpeg75/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/sift/dino/post/none/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/dino/post/none/f1\endcsname{0.57}
\expandafter\def\csname val@fp:loc/sift/dino/post/resize0.75_jpeg80/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/sift/dino/post/resize0.75_jpeg80/f1\endcsname{0.48}
\expandafter\def\csname val@fp:loc/sift/dino/type/copymove/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/dino/type/copymove/f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/sift/dino/type/inpaint-lama/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/sift/dino/type/inpaint-lama/f1\endcsname{0.23}
\expandafter\def\csname val@fp:loc/sift/dino/type/inpaint-telea/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/dino/type/inpaint-telea/f1\endcsname{0.42}
\expandafter\def\csname val@fp:loc/sift/dino/type/recolor/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/sift/dino/type/recolor/f1\endcsname{0.29}
\expandafter\def\csname val@fp:loc/sift/dino/type/splice/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/dino/type/splice/f1\endcsname{0.67}
\expandafter\def\csname val@fp:loc/sift/dino/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/sift/dino/type/textreplace/f1\endcsname{0.84}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.01/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.01/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.03/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.03/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.1/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.1/f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.25/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/fused/area/0.25/f1\endcsname{0.78}
\expandafter\def\csname val@fp:loc/sift/fused/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/fused/best_f1\endcsname{0.81}
\expandafter\def\csname val@fp:loc/sift/fused/f1\endcsname{0.65}
\expandafter\def\csname val@fp:loc/sift/fused/iou\endcsname{0.54}
\expandafter\def\csname val@fp:loc/sift/fused/post/crop90/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/fused/post/crop90/f1\endcsname{0.62}
\expandafter\def\csname val@fp:loc/sift/fused/post/jpeg75/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/fused/post/jpeg75/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/sift/fused/post/none/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/fused/post/none/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/sift/fused/post/resize0.75_jpeg80/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/fused/post/resize0.75_jpeg80/f1\endcsname{0.60}
\expandafter\def\csname val@fp:loc/sift/fused/type/copymove/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/fused/type/copymove/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/sift/fused/type/inpaint-lama/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/fused/type/inpaint-lama/f1\endcsname{0.34}
\expandafter\def\csname val@fp:loc/sift/fused/type/inpaint-telea/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/fused/type/inpaint-telea/f1\endcsname{0.60}
\expandafter\def\csname val@fp:loc/sift/fused/type/recolor/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/fused/type/recolor/f1\endcsname{0.38}
\expandafter\def\csname val@fp:loc/sift/fused/type/splice/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/fused/type/splice/f1\endcsname{0.77}
\expandafter\def\csname val@fp:loc/sift/fused/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/sift/fused/type/textreplace/f1\endcsname{0.91}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.01/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.01/f1\endcsname{0.45}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.03/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.03/f1\endcsname{0.59}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.1/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.1/f1\endcsname{0.76}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.25/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/lpips/area/0.25/f1\endcsname{0.81}
\expandafter\def\csname val@fp:loc/sift/lpips/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/best_f1\endcsname{0.79}
\expandafter\def\csname val@fp:loc/sift/lpips/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/sift/lpips/iou\endcsname{0.52}
\expandafter\def\csname val@fp:loc/sift/lpips/post/crop90/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/lpips/post/crop90/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/sift/lpips/post/jpeg75/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/sift/lpips/post/jpeg75/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/sift/lpips/post/none/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/post/none/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/sift/lpips/post/resize0.75_jpeg80/auc\endcsname{0.97}
\expandafter\def\csname val@fp:loc/sift/lpips/post/resize0.75_jpeg80/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/sift/lpips/type/copymove/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/lpips/type/copymove/f1\endcsname{0.69}
\expandafter\def\csname val@fp:loc/sift/lpips/type/inpaint-lama/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/lpips/type/inpaint-lama/f1\endcsname{0.37}
\expandafter\def\csname val@fp:loc/sift/lpips/type/inpaint-telea/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/type/inpaint-telea/f1\endcsname{0.72}
\expandafter\def\csname val@fp:loc/sift/lpips/type/recolor/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/lpips/type/recolor/f1\endcsname{0.60}
\expandafter\def\csname val@fp:loc/sift/lpips/type/splice/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/sift/lpips/type/splice/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/sift/lpips/type/textreplace/auc\endcsname{0.99}
\expandafter\def\csname val@fp:loc/sift/lpips/type/textreplace/f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/sift/n\endcsname{3{,}000}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.01/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.01/f1\endcsname{0.00}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.03/auc\endcsname{0.89}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.03/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.1/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.1/f1\endcsname{0.05}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.25/auc\endcsname{0.85}
\expandafter\def\csname val@fp:loc/sift/pdq/area/0.25/f1\endcsname{0.07}
\expandafter\def\csname val@fp:loc/sift/pdq/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pdq/best_f1\endcsname{0.50}
\expandafter\def\csname val@fp:loc/sift/pdq/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/iou\endcsname{0.02}
\expandafter\def\csname val@fp:loc/sift/pdq/post/crop90/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/sift/pdq/post/crop90/f1\endcsname{0.03}
\expandafter\def\csname val@fp:loc/sift/pdq/post/jpeg75/auc\endcsname{0.84}
\expandafter\def\csname val@fp:loc/sift/pdq/post/jpeg75/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/post/none/auc\endcsname{0.89}
\expandafter\def\csname val@fp:loc/sift/pdq/post/none/f1\endcsname{0.03}
\expandafter\def\csname val@fp:loc/sift/pdq/post/resize0.75_jpeg80/auc\endcsname{0.82}
\expandafter\def\csname val@fp:loc/sift/pdq/post/resize0.75_jpeg80/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/type/copymove/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pdq/type/copymove/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/type/inpaint-lama/auc\endcsname{0.86}
\expandafter\def\csname val@fp:loc/sift/pdq/type/inpaint-lama/f1\endcsname{0.02}
\expandafter\def\csname val@fp:loc/sift/pdq/type/inpaint-telea/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pdq/type/inpaint-telea/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/type/recolor/auc\endcsname{0.80}
\expandafter\def\csname val@fp:loc/sift/pdq/type/recolor/f1\endcsname{0.01}
\expandafter\def\csname val@fp:loc/sift/pdq/type/splice/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pdq/type/splice/f1\endcsname{0.04}
\expandafter\def\csname val@fp:loc/sift/pdq/type/textreplace/auc\endcsname{0.90}
\expandafter\def\csname val@fp:loc/sift/pdq/type/textreplace/f1\endcsname{0.05}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.01/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.01/f1\endcsname{0.66}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.03/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.03/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.1/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.1/f1\endcsname{0.83}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.25/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/sift/pixel/area/0.25/f1\endcsname{0.82}
\expandafter\def\csname val@fp:loc/sift/pixel/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/sift/pixel/best_f1\endcsname{0.83}
\expandafter\def\csname val@fp:loc/sift/pixel/f1\endcsname{0.75}
\expandafter\def\csname val@fp:loc/sift/pixel/iou\endcsname{0.65}
\expandafter\def\csname val@fp:loc/sift/pixel/post/crop90/auc\endcsname{0.94}
\expandafter\def\csname val@fp:loc/sift/pixel/post/crop90/f1\endcsname{0.71}
\expandafter\def\csname val@fp:loc/sift/pixel/post/jpeg75/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/pixel/post/jpeg75/f1\endcsname{0.84}
\expandafter\def\csname val@fp:loc/sift/pixel/post/none/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/pixel/post/none/f1\endcsname{0.75}
\expandafter\def\csname val@fp:loc/sift/pixel/post/resize0.75_jpeg80/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/pixel/post/resize0.75_jpeg80/f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/sift/pixel/type/copymove/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/pixel/type/copymove/f1\endcsname{0.68}
\expandafter\def\csname val@fp:loc/sift/pixel/type/inpaint-lama/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/pixel/type/inpaint-lama/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/sift/pixel/type/inpaint-telea/auc\endcsname{0.90}
\expandafter\def\csname val@fp:loc/sift/pixel/type/inpaint-telea/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/sift/pixel/type/recolor/auc\endcsname{1.00}
\expandafter\def\csname val@fp:loc/sift/pixel/type/recolor/f1\endcsname{0.84}
\expandafter\def\csname val@fp:loc/sift/pixel/type/splice/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/pixel/type/splice/f1\endcsname{0.79}
\expandafter\def\csname val@fp:loc/sift/pixel/type/textreplace/auc\endcsname{1.00}
\expandafter\def\csname val@fp:loc/sift/pixel/type/textreplace/f1\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.01/auc\endcsname{0.96}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.01/f1\endcsname{0.48}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.03/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.03/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.1/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.1/f1\endcsname{0.61}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.25/auc\endcsname{0.89}
\expandafter\def\csname val@fp:loc/sift/ssim/area/0.25/f1\endcsname{0.60}
\expandafter\def\csname val@fp:loc/sift/ssim/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/ssim/best_f1\endcsname{0.74}
\expandafter\def\csname val@fp:loc/sift/ssim/f1\endcsname{0.57}
\expandafter\def\csname val@fp:loc/sift/ssim/iou\endcsname{0.45}
\expandafter\def\csname val@fp:loc/sift/ssim/post/crop90/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/sift/ssim/post/crop90/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/sift/ssim/post/jpeg75/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/ssim/post/jpeg75/f1\endcsname{0.60}
\expandafter\def\csname val@fp:loc/sift/ssim/post/none/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/ssim/post/none/f1\endcsname{0.64}
\expandafter\def\csname val@fp:loc/sift/ssim/post/resize0.75_jpeg80/auc\endcsname{0.91}
\expandafter\def\csname val@fp:loc/sift/ssim/post/resize0.75_jpeg80/f1\endcsname{0.51}
\expandafter\def\csname val@fp:loc/sift/ssim/type/copymove/auc\endcsname{0.87}
\expandafter\def\csname val@fp:loc/sift/ssim/type/copymove/f1\endcsname{0.63}
\expandafter\def\csname val@fp:loc/sift/ssim/type/inpaint-lama/auc\endcsname{0.92}
\expandafter\def\csname val@fp:loc/sift/ssim/type/inpaint-lama/f1\endcsname{0.39}
\expandafter\def\csname val@fp:loc/sift/ssim/type/inpaint-telea/auc\endcsname{0.88}
\expandafter\def\csname val@fp:loc/sift/ssim/type/inpaint-telea/f1\endcsname{0.56}
\expandafter\def\csname val@fp:loc/sift/ssim/type/recolor/auc\endcsname{0.95}
\expandafter\def\csname val@fp:loc/sift/ssim/type/recolor/f1\endcsname{0.23}
\expandafter\def\csname val@fp:loc/sift/ssim/type/splice/auc\endcsname{0.93}
\expandafter\def\csname val@fp:loc/sift/ssim/type/splice/f1\endcsname{0.72}
\expandafter\def\csname val@fp:loc/sift/ssim/type/textreplace/auc\endcsname{0.98}
\expandafter\def\csname val@fp:loc/sift/ssim/type/textreplace/f1\endcsname{0.74}
\expandafter\def\csname val@fp:paired/DINOv2-S/DINOv2-S-LSH256/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/DINOv2-S/DINOv2-S-LSH256/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/DINOv2-S/OpenCLIP-B32/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/DINOv2-S/OpenCLIP-B32/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/ISCC-Image-64/ISCC-Image-256/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/ISCC-Image-64/ISCC-Image-256/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/PDQ/ISCC-Image-64/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/PDQ/ISCC-Image-64/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/PDQ/PDQ-dihedral/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/PDQ/PDQ-dihedral/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/SSCD-mixup/DINOv2-S/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/SSCD-mixup/DINOv2-S/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/SSCD-mixup/ISC21-1st/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/SSCD-mixup/ISC21-1st/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:paired/pHash-64/PDQ/p\endcsname{$<10^{-3}$}
\expandafter\def\csname val@fp:paired/pHash-64/PDQ/p_mcnemar\endcsname{$<10^{-4}$}
\expandafter\def\csname val@fp:price/gpu\endcsname{1.212}
\expandafter\def\csname val@fp:sec/audio/mag/CLAP/pitch\endcsname{2.0}
\expandafter\def\csname val@fp:sec/audio/mag/CLAP/tempo\endcsname{1.1}
\expandafter\def\csname val@fp:sec/audio/mag/Chromaprint/pitch\endcsname{0.25}
\expandafter\def\csname val@fp:sec/audio/mag/Chromaprint/tempo\endcsname{1.05}
\expandafter\def\csname val@fp:sec/audio/mag/ISCC-Audio-64/pitch\endcsname{0.25}
\expandafter\def\csname val@fp:sec/audio/mag/ISCC-Audio-64/tempo\endcsname{1.02}
\expandafter\def\csname val@fp:sec/audio/mag/audfprint/pitch\endcsname{0.25}
\expandafter\def\csname val@fp:sec/audio/mag/audfprint/tempo\endcsname{1.02}
\expandafter\def\csname val@fp:sec/audio/n\endcsname{60}
\expandafter\def\csname val@fp:sec/audio/pgd/20/CLAP/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/audio/pgd/20/Chromaprint/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/audio/pgd/20/ISCC-Audio-64/pct\endcsname{27}
\expandafter\def\csname val@fp:sec/audio/pgd/20/audfprint/pct\endcsname{12}
\expandafter\def\csname val@fp:sec/audio/pgd/30/CLAP/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/audio/pgd/30/Chromaprint/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/audio/pgd/30/ISCC-Audio-64/pct\endcsname{12}
\expandafter\def\csname val@fp:sec/audio/pgd/30/audfprint/pct\endcsname{5}
\expandafter\def\csname val@fp:sec/audio/pgd/40/CLAP/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/audio/pgd/40/Chromaprint/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/audio/pgd/40/ISCC-Audio-64/pct\endcsname{3}
\expandafter\def\csname val@fp:sec/audio/pgd/40/audfprint/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/audio/rescore_changed\endcsname{0}
\expandafter\def\csname val@fp:sec/audio/snr/20\endcsname{24}
\expandafter\def\csname val@fp:sec/audio/snr/30\endcsname{34}
\expandafter\def\csname val@fp:sec/audio/snr/40\endcsname{43}
\expandafter\def\csname val@fp:sec/audio/thdelta\endcsname{0.0043}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/16/pct\endcsname{26}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/16/psnr\endcsname{29.8}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/4/pct\endcsname{8}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/4/psnr\endcsname{41.1}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/8/pct\endcsname{22}
\expandafter\def\csname val@fp:sec/collision/DINOv2-B/8/psnr\endcsname{35.5}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/16/pct\endcsname{70}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/16/psnr\endcsname{29.9}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/4/pct\endcsname{26}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/4/psnr\endcsname{41.2}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/8/pct\endcsname{49}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S-LSH256/8/psnr\endcsname{35.6}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/16/pct\endcsname{47}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/16/psnr\endcsname{29.7}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/4/pct\endcsname{18}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/4/psnr\endcsname{40.8}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/8/pct\endcsname{36}
\expandafter\def\csname val@fp:sec/collision/DINOv2-S/8/psnr\endcsname{35.4}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/16/psnr\endcsname{29.8}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/4/pct\endcsname{87}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/4/psnr\endcsname{41.3}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/collision/ISC21-1st/8/psnr\endcsname{35.6}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/16/pct\endcsname{4}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/16/psnr\endcsname{27.0}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/4/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/4/psnr\endcsname{38.8}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/8/pct\endcsname{2}
\expandafter\def\csname val@fp:sec/collision/ISCC-Image-64/8/psnr\endcsname{32.8}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/16/pct\endcsname{21}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/16/psnr\endcsname{29.6}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/4/pct\endcsname{1}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/4/psnr\endcsname{40.6}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/8/pct\endcsname{5}
\expandafter\def\csname val@fp:sec/collision/OpenCLIP-B32/8/psnr\endcsname{35.1}
\expandafter\def\csname val@fp:sec/collision/PDQ/16/pct\endcsname{6}
\expandafter\def\csname val@fp:sec/collision/PDQ/16/psnr\endcsname{28.9}
\expandafter\def\csname val@fp:sec/collision/PDQ/4/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/PDQ/4/psnr\endcsname{39.3}
\expandafter\def\csname val@fp:sec/collision/PDQ/8/pct\endcsname{3}
\expandafter\def\csname val@fp:sec/collision/PDQ/8/psnr\endcsname{34.0}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/16/pct\endcsname{89}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/16/psnr\endcsname{29.7}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/4/pct\endcsname{24}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/4/psnr\endcsname{41.1}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/8/pct\endcsname{58}
\expandafter\def\csname val@fp:sec/collision/SSCD-large/8/psnr\endcsname{35.4}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/16/pct\endcsname{98}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/16/psnr\endcsname{29.6}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/4/pct\endcsname{60}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/4/psnr\endcsname{40.8}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/8/pct\endcsname{97}
\expandafter\def\csname val@fp:sec/collision/SSCD-mixup/8/psnr\endcsname{35.3}
\expandafter\def\csname val@fp:sec/collision/aHash-64/16/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/aHash-64/16/psnr\endcsname{27.1}
\expandafter\def\csname val@fp:sec/collision/aHash-64/4/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/aHash-64/4/psnr\endcsname{38.7}
\expandafter\def\csname val@fp:sec/collision/aHash-64/8/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/aHash-64/8/psnr\endcsname{32.9}
\expandafter\def\csname val@fp:sec/collision/dHash-64/16/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/dHash-64/16/psnr\endcsname{27.4}
\expandafter\def\csname val@fp:sec/collision/dHash-64/4/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/dHash-64/4/psnr\endcsname{38.7}
\expandafter\def\csname val@fp:sec/collision/dHash-64/8/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/dHash-64/8/psnr\endcsname{33.0}
\expandafter\def\csname val@fp:sec/collision/pHash-64/16/pct\endcsname{1}
\expandafter\def\csname val@fp:sec/collision/pHash-64/16/psnr\endcsname{27.0}
\expandafter\def\csname val@fp:sec/collision/pHash-64/4/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/collision/pHash-64/4/psnr\endcsname{38.8}
\expandafter\def\csname val@fp:sec/collision/pHash-64/8/pct\endcsname{1}
\expandafter\def\csname val@fp:sec/collision/pHash-64/8/psnr\endcsname{32.8}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256-wrongkey/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256-wrongkey/lpips\endcsname{0.512}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256-wrongkey/reid/pct\endcsname{0.0}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256-wrongkey/reid_top1\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256-wrongkey/ssim\endcsname{0.122}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256/lpips\endcsname{0.239}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256/reid/pct\endcsname{0.8}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256/reid_top1\endcsname{0.008}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S-LSH256/ssim\endcsname{0.374}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S/lpips\endcsname{0.183}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S/reid/pct\endcsname{1.7}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S/reid_top1\endcsname{0.017}
\expandafter\def\csname val@fp:sec/inv/DINOv2-S/ssim\endcsname{0.424}
\expandafter\def\csname val@fp:sec/inv/ISCC-Image-64/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/ISCC-Image-64/lpips\endcsname{0.328}
\expandafter\def\csname val@fp:sec/inv/ISCC-Image-64/reid/pct\endcsname{0.1}
\expandafter\def\csname val@fp:sec/inv/ISCC-Image-64/reid_top1\endcsname{0.001}
\expandafter\def\csname val@fp:sec/inv/ISCC-Image-64/ssim\endcsname{0.310}
\expandafter\def\csname val@fp:sec/inv/OpenCLIP-B32/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/OpenCLIP-B32/lpips\endcsname{0.180}
\expandafter\def\csname val@fp:sec/inv/OpenCLIP-B32/reid/pct\endcsname{1.9}
\expandafter\def\csname val@fp:sec/inv/OpenCLIP-B32/reid_top1\endcsname{0.019}
\expandafter\def\csname val@fp:sec/inv/OpenCLIP-B32/ssim\endcsname{0.429}
\expandafter\def\csname val@fp:sec/inv/PDQ/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/PDQ/lpips\endcsname{0.298}
\expandafter\def\csname val@fp:sec/inv/PDQ/reid/pct\endcsname{0.2}
\expandafter\def\csname val@fp:sec/inv/PDQ/reid_top1\endcsname{0.002}
\expandafter\def\csname val@fp:sec/inv/PDQ/ssim\endcsname{0.441}
\expandafter\def\csname val@fp:sec/inv/SSCD-mixup/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/SSCD-mixup/lpips\endcsname{0.202}
\expandafter\def\csname val@fp:sec/inv/SSCD-mixup/reid/pct\endcsname{0.9}
\expandafter\def\csname val@fp:sec/inv/SSCD-mixup/reid_top1\endcsname{0.009}
\expandafter\def\csname val@fp:sec/inv/SSCD-mixup/ssim\endcsname{0.409}
\expandafter\def\csname val@fp:sec/inv/mean-image/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/mean-image/lpips\endcsname{0.539}
\expandafter\def\csname val@fp:sec/inv/mean-image/reid/pct\endcsname{0.0}
\expandafter\def\csname val@fp:sec/inv/mean-image/reid_top1\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/mean-image/ssim\endcsname{0.265}
\expandafter\def\csname val@fp:sec/inv/ntest\endcsname{5{,}000}
\expandafter\def\csname val@fp:sec/inv/ntrain\endcsname{100{,}000}
\expandafter\def\csname val@fp:sec/inv/pHash-64/chance\endcsname{0.000}
\expandafter\def\csname val@fp:sec/inv/pHash-64/lpips\endcsname{0.306}
\expandafter\def\csname val@fp:sec/inv/pHash-64/reid/pct\endcsname{0.1}
\expandafter\def\csname val@fp:sec/inv/pHash-64/reid_top1\endcsname{0.001}
\expandafter\def\csname val@fp:sec/inv/pHash-64/ssim\endcsname{0.404}
\expandafter\def\csname val@fp:sec/n\endcsname{100}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/lpips\endcsname{0.078}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/pct7\endcsname{99}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/psnr\endcsname{29.2}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/rate\endcsname{0.99}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/16/rate7\endcsname{0.99}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/lpips\endcsname{0.001}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/pct\endcsname{65}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/pct7\endcsname{81}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/psnr\endcsname{46.1}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/rate\endcsname{0.65}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/2/rate7\endcsname{0.81}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/lpips\endcsname{0.004}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/pct\endcsname{77}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/pct7\endcsname{91}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/psnr\endcsname{40.5}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/rate\endcsname{0.77}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/4/rate7\endcsname{0.91}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/lpips\endcsname{0.017}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/pct\endcsname{91}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/pct7\endcsname{95}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/psnr\endcsname{34.9}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/rate\endcsname{0.91}
\expandafter\def\csname val@fp:sec/surrogate/ISCC-Image-64/8/rate7\endcsname{0.95}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/lpips\endcsname{0.095}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/psnr\endcsname{29.3}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/rate\endcsname{0.99}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/pct\endcsname{8}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/pct7\endcsname{22}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/psnr\endcsname{45.5}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/rate\endcsname{0.08}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/2/rate7\endcsname{0.22}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/lpips\endcsname{0.008}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/pct\endcsname{33}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/pct7\endcsname{56}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/psnr\endcsname{39.9}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/rate\endcsname{0.33}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/4/rate7\endcsname{0.56}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/lpips\endcsname{0.028}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/pct\endcsname{81}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/pct7\endcsname{97}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/psnr\endcsname{34.5}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/rate\endcsname{0.81}
\expandafter\def\csname val@fp:sec/surrogate/PDQ/8/rate7\endcsname{0.97}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/16/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/16/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/16/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/16/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/2/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/2/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/2/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/2/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/4/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/4/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/4/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/4/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/8/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/8/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/8/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/aHash-64/8/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/16/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/16/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/16/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/16/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/2/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/2/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/2/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/2/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/4/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/4/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/4/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/4/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/8/lpips\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/8/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/8/psnr\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/dHash-64/8/rate\endcsname{--}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/lpips\endcsname{0.078}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/psnr\endcsname{29.1}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/rate\endcsname{0.99}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/lpips\endcsname{0.001}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/pct\endcsname{44}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/pct7\endcsname{74}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/psnr\endcsname{45.6}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/rate\endcsname{0.44}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/2/rate7\endcsname{0.74}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/lpips\endcsname{0.003}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/pct\endcsname{74}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/pct7\endcsname{88}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/psnr\endcsname{40.4}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/rate\endcsname{0.74}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/4/rate7\endcsname{0.88}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/lpips\endcsname{0.017}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/pct\endcsname{90}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/pct7\endcsname{95}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/psnr\endcsname{34.9}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/rate\endcsname{0.90}
\expandafter\def\csname val@fp:sec/surrogate/pHash-64/8/rate7\endcsname{0.95}
\expandafter\def\csname val@fp:sec/transfer/16/BlockMean/pct\endcsname{54}
\expandafter\def\csname val@fp:sec/transfer/16/Blockhash-256/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/16/ColorMoment/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/16/DINOHash-96/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/DINOv2-B/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/DINOv2-S-LSH256/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/DINOv2-S/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/ISC21-1st/pct\endcsname{35}
\expandafter\def\csname val@fp:sec/transfer/16/ISCC-Image-256/pct\endcsname{55}
\expandafter\def\csname val@fp:sec/transfer/16/ISCC-Image-64/pct\endcsname{56}
\expandafter\def\csname val@fp:sec/transfer/16/MarrHildreth/pct\endcsname{89}
\expandafter\def\csname val@fp:sec/transfer/16/OpenCLIP-B32/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/PDQ-dihedral/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/16/PDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/16/SSCD-large/pct\endcsname{96}
\expandafter\def\csname val@fp:sec/transfer/16/SSCD-mixup/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/16/aHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/16/dHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/16/pHash-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/16/pHash-64/pct\endcsname{11}
\expandafter\def\csname val@fp:sec/transfer/16/wHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/2/BlockMean/pct\endcsname{11}
\expandafter\def\csname val@fp:sec/transfer/2/Blockhash-256/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/2/ColorMoment/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/2/DINOHash-96/pct\endcsname{72}
\expandafter\def\csname val@fp:sec/transfer/2/DINOv2-B/pct\endcsname{60}
\expandafter\def\csname val@fp:sec/transfer/2/DINOv2-S-LSH256/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/transfer/2/DINOv2-S/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/transfer/2/ISC21-1st/pct\endcsname{2}
\expandafter\def\csname val@fp:sec/transfer/2/ISCC-Image-256/pct\endcsname{52}
\expandafter\def\csname val@fp:sec/transfer/2/ISCC-Image-64/pct\endcsname{54}
\expandafter\def\csname val@fp:sec/transfer/2/MarrHildreth/pct\endcsname{84}
\expandafter\def\csname val@fp:sec/transfer/2/OpenCLIP-B32/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/2/PDQ-dihedral/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/2/PDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/2/SSCD-large/pct\endcsname{61}
\expandafter\def\csname val@fp:sec/transfer/2/SSCD-mixup/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/transfer/2/aHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/2/dHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/2/pHash-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/2/pHash-64/pct\endcsname{2}
\expandafter\def\csname val@fp:sec/transfer/2/wHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/4/BlockMean/pct\endcsname{21}
\expandafter\def\csname val@fp:sec/transfer/4/Blockhash-256/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/4/ColorMoment/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/4/DINOHash-96/pct\endcsname{91}
\expandafter\def\csname val@fp:sec/transfer/4/DINOv2-B/pct\endcsname{89}
\expandafter\def\csname val@fp:sec/transfer/4/DINOv2-S-LSH256/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/4/DINOv2-S/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/4/ISC21-1st/pct\endcsname{2}
\expandafter\def\csname val@fp:sec/transfer/4/ISCC-Image-256/pct\endcsname{53}
\expandafter\def\csname val@fp:sec/transfer/4/ISCC-Image-64/pct\endcsname{54}
\expandafter\def\csname val@fp:sec/transfer/4/MarrHildreth/pct\endcsname{85}
\expandafter\def\csname val@fp:sec/transfer/4/OpenCLIP-B32/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/4/PDQ-dihedral/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/4/PDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/4/SSCD-large/pct\endcsname{43}
\expandafter\def\csname val@fp:sec/transfer/4/SSCD-mixup/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/4/aHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/4/dHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/4/pHash-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/4/pHash-64/pct\endcsname{3}
\expandafter\def\csname val@fp:sec/transfer/4/wHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/8/BlockMean/pct\endcsname{35}
\expandafter\def\csname val@fp:sec/transfer/8/Blockhash-256/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/8/ColorMoment/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/8/DINOHash-96/pct\endcsname{98}
\expandafter\def\csname val@fp:sec/transfer/8/DINOv2-B/pct\endcsname{99}
\expandafter\def\csname val@fp:sec/transfer/8/DINOv2-S-LSH256/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/8/DINOv2-S/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/8/ISC21-1st/pct\endcsname{10}
\expandafter\def\csname val@fp:sec/transfer/8/ISCC-Image-256/pct\endcsname{53}
\expandafter\def\csname val@fp:sec/transfer/8/ISCC-Image-64/pct\endcsname{55}
\expandafter\def\csname val@fp:sec/transfer/8/MarrHildreth/pct\endcsname{86}
\expandafter\def\csname val@fp:sec/transfer/8/OpenCLIP-B32/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/8/PDQ-dihedral/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/8/PDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/8/SSCD-large/pct\endcsname{70}
\expandafter\def\csname val@fp:sec/transfer/8/SSCD-mixup/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/transfer/8/aHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/8/dHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/transfer/8/pHash-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/transfer/8/pHash-64/pct\endcsname{6}
\expandafter\def\csname val@fp:sec/transfer/8/wHash-64/pct\endcsname{--}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/DINOv2-S-mean/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/DINOv2-S-seq/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/ISCC-Video-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/ISCC-Video-64/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/SSCD-mixup-mean/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/SSCD-mixup-seq/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/TMK+PDQF/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/4/vPDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/DINOv2-S-mean/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/DINOv2-S-seq/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/ISCC-Video-256/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/ISCC-Video-64/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/SSCD-mixup-mean/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/SSCD-mixup-seq/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/TMK+PDQF/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/frame_pgd/8/vPDQ/pct\endcsname{0}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-mean/crop_keep_median\endcsname{0.8}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-mean/speed_median\endcsname{2.0}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-mean/speed_never\endcsname{11}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-seq/crop_keep_median\endcsname{0.9}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-seq/speed_median\endcsname{1.1}
\expandafter\def\csname val@fp:sec/video/magnitude/DINOv2-S-seq/speed_never\endcsname{2}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-256/crop_keep_median\endcsname{0.9}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-256/speed_median\endcsname{>2.0}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-256/speed_never\endcsname{30}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-64/crop_keep_median\endcsname{0.9}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-64/speed_median\endcsname{>2.0}
\expandafter\def\csname val@fp:sec/video/magnitude/ISCC-Video-64/speed_never\endcsname{29}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-mean/crop_keep_median\endcsname{0.8}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-mean/speed_median\endcsname{2.0}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-mean/speed_never\endcsname{12}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-seq/crop_keep_median\endcsname{0.8}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-seq/speed_median\endcsname{1.1}
\expandafter\def\csname val@fp:sec/video/magnitude/SSCD-mixup-seq/speed_never\endcsname{5}
\expandafter\def\csname val@fp:sec/video/magnitude/TMK+PDQF/crop_keep_median\endcsname{0.9}
\expandafter\def\csname val@fp:sec/video/magnitude/TMK+PDQF/speed_median\endcsname{>2.0}
\expandafter\def\csname val@fp:sec/video/magnitude/TMK+PDQF/speed_never\endcsname{30}
\expandafter\def\csname val@fp:sec/video/magnitude/vPDQ/crop_keep_median\endcsname{0.9}
\expandafter\def\csname val@fp:sec/video/magnitude/vPDQ/speed_median\endcsname{1.25}
\expandafter\def\csname val@fp:sec/video/magnitude/vPDQ/speed_never\endcsname{13}
\expandafter\def\csname val@fp:sec/video/n\endcsname{30}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/lpips\endcsname{0.117}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/psnr\endcsname{30.0}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/psnr\endcsname{47.3}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/lpips\endcsname{0.008}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/psnr\endcsname{41.8}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/lpips\endcsname{0.033}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/psnr\endcsname{35.9}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-B/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/lpips\endcsname{0.120}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/psnr\endcsname{30.0}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/psnr\endcsname{47.3}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/lpips\endcsname{0.008}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/psnr\endcsname{41.8}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/lpips\endcsname{0.034}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/psnr\endcsname{35.9}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S-LSH256/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/lpips\endcsname{0.122}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/psnr\endcsname{30.0}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/psnr\endcsname{47.3}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/lpips\endcsname{0.008}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/psnr\endcsname{41.7}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/lpips\endcsname{0.035}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/psnr\endcsname{35.8}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/DINOv2-S/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/lpips\endcsname{0.113}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/psnr\endcsname{30.0}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/psnr\endcsname{47.4}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/lpips\endcsname{0.006}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/psnr\endcsname{41.8}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/lpips\endcsname{0.028}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/psnr\endcsname{35.9}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/ISC21-1st/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/lpips\endcsname{0.122}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/psnr\endcsname{29.9}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/psnr\endcsname{47.5}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/lpips\endcsname{0.008}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/psnr\endcsname{41.8}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/lpips\endcsname{0.035}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/psnr\endcsname{35.8}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/OpenCLIP-B32/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/lpips\endcsname{0.120}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/psnr\endcsname{30.0}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/psnr\endcsname{47.5}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/lpips\endcsname{0.007}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/psnr\endcsname{41.9}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/lpips\endcsname{0.032}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/psnr\endcsname{35.9}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-large/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/lpips\endcsname{0.119}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/psnr\endcsname{29.9}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/16/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/lpips\endcsname{0.002}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/psnr\endcsname{47.3}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/2/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/lpips\endcsname{0.007}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/psnr\endcsname{41.8}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/4/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/lpips\endcsname{0.032}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/pct\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/pct7\endcsname{100}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/psnr\endcsname{35.8}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/rate\endcsname{1.00}
\expandafter\def\csname val@fp:sec/whitebox/SSCD-mixup/8/rate7\endcsname{1.00}
\expandafter\def\csname val@fp:sens/any/DINOv2-B/TPR@pair@1e-07\endcsname{0.650}
\expandafter\def\csname val@fp:sens/any/DINOv2-B/TPR@query@0.01\endcsname{0.653}
\expandafter\def\csname val@fp:sens/any/DINOv2-S-LSH256/TPR@pair@1e-07\endcsname{0.519}
\expandafter\def\csname val@fp:sens/any/DINOv2-S-LSH256/TPR@query@0.01\endcsname{0.538}
\expandafter\def\csname val@fp:sens/any/DINOv2-S/TPR@pair@1e-07\endcsname{0.612}
\expandafter\def\csname val@fp:sens/any/DINOv2-S/TPR@query@0.01\endcsname{0.625}
\expandafter\def\csname val@fp:sens/any/ISC21-1st/TPR@pair@1e-07\endcsname{0.755}
\expandafter\def\csname val@fp:sens/any/ISC21-1st/TPR@query@0.01\endcsname{0.762}
\expandafter\def\csname val@fp:sens/any/ISCC-Image-256/TPR@pair@1e-07\endcsname{0.458}
\expandafter\def\csname val@fp:sens/any/ISCC-Image-256/TPR@query@0.01\endcsname{0.466}
\expandafter\def\csname val@fp:sens/any/OpenCLIP-B32/TPR@pair@1e-07\endcsname{0.356}
\expandafter\def\csname val@fp:sens/any/OpenCLIP-B32/TPR@query@0.01\endcsname{0.401}
\expandafter\def\csname val@fp:sens/any/PDQ-dihedral/TPR@pair@1e-07\endcsname{0.546}
\expandafter\def\csname val@fp:sens/any/PDQ-dihedral/TPR@query@0.01\endcsname{0.549}
\expandafter\def\csname val@fp:sens/any/PDQ/TPR@pair@1e-07\endcsname{0.495}
\expandafter\def\csname val@fp:sens/any/PDQ/TPR@query@0.01\endcsname{0.495}
\expandafter\def\csname val@fp:sens/any/SSCD-mixup/TPR@pair@1e-07\endcsname{0.712}
\expandafter\def\csname val@fp:sens/any/SSCD-mixup/TPR@query@0.01\endcsname{0.725}
\expandafter\def\csname val@fp:sens/any/pHash-256/TPR@pair@1e-07\endcsname{0.492}
\expandafter\def\csname val@fp:sens/any/pHash-256/TPR@query@0.01\endcsname{0.494}
\expandafter\def\csname val@fp:sens/none/DINOv2-B/TPR@pair@1e-07\endcsname{0.199}
\expandafter\def\csname val@fp:sens/none/DINOv2-B/TPR@query@0.01\endcsname{0.201}
\expandafter\def\csname val@fp:sens/none/DINOv2-S-LSH256/TPR@pair@1e-07\endcsname{0.174}
\expandafter\def\csname val@fp:sens/none/DINOv2-S-LSH256/TPR@query@0.01\endcsname{0.174}
\expandafter\def\csname val@fp:sens/none/DINOv2-S/TPR@pair@1e-07\endcsname{0.192}
\expandafter\def\csname val@fp:sens/none/DINOv2-S/TPR@query@0.01\endcsname{0.194}
\expandafter\def\csname val@fp:sens/none/ISC21-1st/TPR@pair@1e-07\endcsname{0.212}
\expandafter\def\csname val@fp:sens/none/ISC21-1st/TPR@query@0.01\endcsname{0.213}
\expandafter\def\csname val@fp:sens/none/ISCC-Image-256/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:sens/none/ISCC-Image-256/TPR@query@0.01\endcsname{0.211}
\expandafter\def\csname val@fp:sens/none/OpenCLIP-B32/TPR@pair@1e-07\endcsname{0.170}
\expandafter\def\csname val@fp:sens/none/OpenCLIP-B32/TPR@query@0.01\endcsname{0.185}
\expandafter\def\csname val@fp:sens/none/PDQ-dihedral/TPR@pair@1e-07\endcsname{0.223}
\expandafter\def\csname val@fp:sens/none/PDQ-dihedral/TPR@query@0.01\endcsname{0.223}
\expandafter\def\csname val@fp:sens/none/PDQ/TPR@pair@1e-07\endcsname{0.214}
\expandafter\def\csname val@fp:sens/none/PDQ/TPR@query@0.01\endcsname{0.214}
\expandafter\def\csname val@fp:sens/none/SSCD-mixup/TPR@pair@1e-07\endcsname{0.217}
\expandafter\def\csname val@fp:sens/none/SSCD-mixup/TPR@query@0.01\endcsname{0.236}
\expandafter\def\csname val@fp:sens/none/pHash-256/TPR@pair@1e-07\endcsname{0.000}
\expandafter\def\csname val@fp:sens/none/pHash-256/TPR@query@0.01\endcsname{0.000}
\expandafter\def\csname val@fp:sens/two/DINOv2-B/TPR@pair@1e-07\endcsname{0.537}
\expandafter\def\csname val@fp:sens/two/DINOv2-B/TPR@query@0.01\endcsname{0.542}
\expandafter\def\csname val@fp:sens/two/DINOv2-S-LSH256/TPR@pair@1e-07\endcsname{0.462}
\expandafter\def\csname val@fp:sens/two/DINOv2-S-LSH256/TPR@query@0.01\endcsname{0.462}
\expandafter\def\csname val@fp:sens/two/DINOv2-S/TPR@pair@1e-07\endcsname{0.544}
\expandafter\def\csname val@fp:sens/two/DINOv2-S/TPR@query@0.01\endcsname{0.546}
\expandafter\def\csname val@fp:sens/two/ISC21-1st/TPR@pair@1e-07\endcsname{0.665}
\expandafter\def\csname val@fp:sens/two/ISC21-1st/TPR@query@0.01\endcsname{0.704}
\expandafter\def\csname val@fp:sens/two/ISCC-Image-256/TPR@pair@1e-07\endcsname{0.448}
\expandafter\def\csname val@fp:sens/two/ISCC-Image-256/TPR@query@0.01\endcsname{0.448}
\expandafter\def\csname val@fp:sens/two/OpenCLIP-B32/TPR@pair@1e-07\endcsname{0.344}
\expandafter\def\csname val@fp:sens/two/OpenCLIP-B32/TPR@query@0.01\endcsname{0.365}
\expandafter\def\csname val@fp:sens/two/PDQ-dihedral/TPR@pair@1e-07\endcsname{0.523}
\expandafter\def\csname val@fp:sens/two/PDQ-dihedral/TPR@query@0.01\endcsname{0.523}
\expandafter\def\csname val@fp:sens/two/PDQ/TPR@pair@1e-07\endcsname{0.471}
\expandafter\def\csname val@fp:sens/two/PDQ/TPR@query@0.01\endcsname{0.476}
\expandafter\def\csname val@fp:sens/two/SSCD-mixup/TPR@pair@1e-07\endcsname{0.512}
\expandafter\def\csname val@fp:sens/two/SSCD-mixup/TPR@query@0.01\endcsname{0.601}
\expandafter\def\csname val@fp:sens/two/pHash-256/TPR@pair@1e-07\endcsname{0.472}
\expandafter\def\csname val@fp:sens/two/pHash-256/TPR@query@0.01\endcsname{0.476}
\expandafter\def\csname val@fp:stab/BlockMean/below\endcsname{0}
\expandafter\def\csname val@fp:stab/BlockMean/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/BlockMean/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/BlockMean/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/Blockhash-256/below\endcsname{200}
\expandafter\def\csname val@fp:stab/Blockhash-256/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/Blockhash-256/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/Blockhash-256/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/ColorMoment/below\endcsname{200}
\expandafter\def\csname val@fp:stab/ColorMoment/differ/pct\endcsname{94}
\expandafter\def\csname val@fp:stab/ColorMoment/identical/pct\endcsname{6}
\expandafter\def\csname val@fp:stab/DINOHash-96/below\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOHash-96/bitsmax\endcsname{1}
\expandafter\def\csname val@fp:stab/DINOHash-96/differ/pct\endcsname{1}
\expandafter\def\csname val@fp:stab/DINOHash-96/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/DINOv2-B/below\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-B/cosmax\endcsname{0.00000012}
\expandafter\def\csname val@fp:stab/DINOv2-B/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/DINOv2-B/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-S-LSH256/below\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-S-LSH256/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-S-LSH256/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-S-LSH256/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/DINOv2-S/below\endcsname{0}
\expandafter\def\csname val@fp:stab/DINOv2-S/cosmax\endcsname{0.00000012}
\expandafter\def\csname val@fp:stab/DINOv2-S/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/DINOv2-S/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/ISC21-1st/below\endcsname{0}
\expandafter\def\csname val@fp:stab/ISC21-1st/cosmax\endcsname{0.00000077}
\expandafter\def\csname val@fp:stab/ISC21-1st/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/ISC21-1st/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-256/below\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-256/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-256/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-256/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/ISCC-Image-64/below\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-64/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-64/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/ISCC-Image-64/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/MarrHildreth/below\endcsname{23}
\expandafter\def\csname val@fp:stab/MarrHildreth/bitsmax\endcsname{64}
\expandafter\def\csname val@fp:stab/MarrHildreth/differ/pct\endcsname{89}
\expandafter\def\csname val@fp:stab/MarrHildreth/identical/pct\endcsname{11}
\expandafter\def\csname val@fp:stab/OpenCLIP-B32/below\endcsname{0}
\expandafter\def\csname val@fp:stab/OpenCLIP-B32/cosmax\endcsname{0.000048}
\expandafter\def\csname val@fp:stab/OpenCLIP-B32/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/OpenCLIP-B32/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ-dihedral/below\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ-dihedral/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ-dihedral/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ-dihedral/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/PDQ/below\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/PDQ/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/SSCD-large/below\endcsname{0}
\expandafter\def\csname val@fp:stab/SSCD-large/cosmax\endcsname{0.00014}
\expandafter\def\csname val@fp:stab/SSCD-large/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/SSCD-large/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/SSCD-mixup/below\endcsname{0}
\expandafter\def\csname val@fp:stab/SSCD-mixup/cosmax\endcsname{0.000077}
\expandafter\def\csname val@fp:stab/SSCD-mixup/differ/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/SSCD-mixup/identical/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/aHash-64/below\endcsname{200}
\expandafter\def\csname val@fp:stab/aHash-64/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/aHash-64/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/aHash-64/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/dHash-64/below\endcsname{0}
\expandafter\def\csname val@fp:stab/dHash-64/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/dHash-64/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/dHash-64/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/n\endcsname{200}
\expandafter\def\csname val@fp:stab/pHash-256/below\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-256/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-256/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-256/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/pHash-64/below\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-64/bitsmax\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-64/differ/pct\endcsname{0}
\expandafter\def\csname val@fp:stab/pHash-64/identical/pct\endcsname{100}
\expandafter\def\csname val@fp:stab/wHash-64/below\endcsname{200}
\expandafter\def\csname val@fp:stab/wHash-64/bitsmax\endcsname{31}
\expandafter\def\csname val@fp:stab/wHash-64/differ/pct\endcsname{14}
\expandafter\def\csname val@fp:stab/wHash-64/identical/pct\endcsname{86}
\expandafter\def\csname val@fp:tloc/audio/audfprint/_all/median_ms\endcsname{5}
\expandafter\def\csname val@fp:tloc/audio/audfprint/_all/within05\endcsname{88.1}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt10/median_ms\endcsname{4}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt10/within05\endcsname{94.4}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt10_mp3_noise20/median_ms\endcsname{4}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt10_mp3_noise20/within05\endcsname{89.5}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt5/median_ms\endcsname{6}
\expandafter\def\csname val@fp:tloc/audio/audfprint/excerpt5/within05\endcsname{86.1}
\expandafter\def\csname val@fp:tloc/audio/audfprint/rerecord/median_ms\endcsname{5}
\expandafter\def\csname val@fp:tloc/audio/audfprint/rerecord/within05\endcsname{82.6}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/_all/median_ms\endcsname{27}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/_all/within05\endcsname{98.9}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt10/median_ms\endcsname{25}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt10/within05\endcsname{99.6}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt10_mp3_noise20/median_ms\endcsname{26}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt10_mp3_noise20/within05\endcsname{99.6}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt5/median_ms\endcsname{30}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/excerpt5/within05\endcsname{98.8}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/rerecord/median_ms\endcsname{26}
\expandafter\def\csname val@fp:tloc/audio/chromaprint/rerecord/within05\endcsname{97.5}
\expandafter\def\csname val@fp:tloc/video/DINOv2-S/excerpt2.5/median_ms\endcsname{71}
\expandafter\def\csname val@fp:tloc/video/DINOv2-S/excerpt2.5/within1\endcsname{100.0}
\expandafter\def\csname val@fp:tloc/video/DINOv2-S/insert/iou\endcsname{0.98}
\expandafter\def\csname val@fp:tloc/video/DINOv2-S/insert/median_ms\endcsname{73}
\expandafter\def\csname val@fp:tloc/video/DINOv2-S/insert/within1\endcsname{100.0}
\expandafter\def\csname val@fp:tloc/video/SSCD-mixup/excerpt2.5/median_ms\endcsname{72}
\expandafter\def\csname val@fp:tloc/video/SSCD-mixup/excerpt2.5/within1\endcsname{100.0}
\expandafter\def\csname val@fp:tloc/video/SSCD-mixup/insert/iou\endcsname{1.00}
\expandafter\def\csname val@fp:tloc/video/SSCD-mixup/insert/median_ms\endcsname{75}
\expandafter\def\csname val@fp:tloc/video/SSCD-mixup/insert/within1\endcsname{100.0}
\expandafter\def\csname val@fp:verify/DINOv2-S/one/fp\endcsname{180}
\expandafter\def\csname val@fp:verify/DINOv2-S/one/tpr\endcsname{0.612}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k12/fp\endcsname{4{,}390}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k12/k\endcsname{12}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k12/ret_fp\endcsname{15{,}694}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k12/ret_tpr\endcsname{0.831}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k12/tpr\endcsname{0.793}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_match/fp\endcsname{146}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_match/k\endcsname{266}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_match/ret_fp\endcsname{15{,}694}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_match/ret_tpr\endcsname{0.831}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_match/tpr\endcsname{0.268}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_zero/fp\endcsname{0}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_zero/k\endcsname{1119}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_zero/ret_fp\endcsname{15{,}694}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_zero/ret_tpr\endcsname{0.831}
\expandafter\def\csname val@fp:verify/DINOv2-S/pair@0.0001/k_zero/tpr\endcsname{0.023}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k12/fp\endcsname{104}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k12/k\endcsname{12}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k12/ret_fp\endcsname{289}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k12/ret_tpr\endcsname{0.625}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k12/tpr\endcsname{0.604}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_match/fp\endcsname{124}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_match/k\endcsname{9}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_match/ret_fp\endcsname{289}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_match/ret_tpr\endcsname{0.625}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_match/tpr\endcsname{0.609}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_zero/fp\endcsname{0}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_zero/k\endcsname{278}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_zero/ret_fp\endcsname{289}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_zero/ret_tpr\endcsname{0.625}
\expandafter\def\csname val@fp:verify/DINOv2-S/query@0.01/k_zero/tpr\endcsname{0.206}
\expandafter\def\csname val@fp:verify/PDQ/one/fp\endcsname{267}
\expandafter\def\csname val@fp:verify/PDQ/one/tpr\endcsname{0.495}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k12/fp\endcsname{2{,}565}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k12/k\endcsname{12}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k12/ret_fp\endcsname{20{,}607}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k12/ret_tpr\endcsname{0.576}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k12/tpr\endcsname{0.559}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_match/fp\endcsname{212}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_match/k\endcsname{167}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_match/ret_fp\endcsname{20{,}607}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_match/ret_tpr\endcsname{0.576}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_match/tpr\endcsname{0.299}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_zero/fp\endcsname{0}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_zero/k\endcsname{684}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_zero/ret_fp\endcsname{20{,}607}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_zero/ret_tpr\endcsname{0.576}
\expandafter\def\csname val@fp:verify/PDQ/pair@0.0001/k_zero/tpr\endcsname{0.066}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k12/fp\endcsname{134}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k12/k\endcsname{12}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k12/ret_fp\endcsname{267}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k12/ret_tpr\endcsname{0.495}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k12/tpr\endcsname{0.481}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_match/fp\endcsname{267}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_match/k\endcsname{0}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_match/ret_fp\endcsname{267}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_match/ret_tpr\endcsname{0.495}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_match/tpr\endcsname{0.495}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_zero/fp\endcsname{0}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_zero/k\endcsname{644}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_zero/ret_fp\endcsname{267}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_zero/ret_tpr\endcsname{0.495}
\expandafter\def\csname val@fp:verify/PDQ/query@0.01/k_zero/tpr\endcsname{0.065}
\expandafter\def\csname val@fp:verify/n_test\endcsname{26{,}820}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/FPRq@query@0.01\endcsname{0.032}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/FPRq@query@0.01/pct\endcsname{3.2}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/R@1\endcsname{0.947}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/R@1/pct\endcsname{94.7}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/R@10\endcsname{0.977}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/R@10/pct\endcsname{97.7}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/TPR@pair@0.0001\endcsname{0.653}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/TPR@pair@0.0001/pct\endcsname{65.3}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/TPR@query@0.01\endcsname{0.547}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/TPR@query@0.01/pct\endcsname{54.7}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/bright\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/bright/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/contrast\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/contrast/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/crop50\endcsname{0.92}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/crop50/pct\endcsname{92}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/crop75\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/crop75/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/excerpt2.5\endcsname{0.89}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/excerpt2.5/pct\endcsname{89}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/gray\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/gray/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h265_crf32\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/h265_crf32/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/hflip\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/hflip/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/insert\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/insert/pct\endcsname{96}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/letterbox\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/letterbox/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/logo\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/logo/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/noise\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/noise/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/pip\endcsname{0.20}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/pip/pct\endcsname{20}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/rot5\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/rot5/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/rot90\endcsname{0.83}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/rot90/pct\endcsname{83}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/screenrec\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/screenrec/pct\endcsname{95}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/speed1.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/speed1.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/text\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/att/text/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/bits\endcsname{12288}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/chain\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/crop\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/geometric\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/overlay\endcsname{0.73}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/fam/temporal\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/ms\endcsname{136}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/muAP\endcsname{0.831}
\expandafter\def\csname val@fp:video/DINOv2-S-mean/muAP/pct\endcsname{83.1}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/FPRq@query@0.01\endcsname{0.062}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/FPRq@query@0.01/pct\endcsname{6.2}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/R@1\endcsname{0.872}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/R@1/pct\endcsname{87.2}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/R@10\endcsname{0.977}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/R@10/pct\endcsname{97.7}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/TPR@pair@0.0001\endcsname{0.523}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/TPR@pair@0.0001/pct\endcsname{52.3}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/TPR@query@0.01\endcsname{0.437}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/TPR@query@0.01/pct\endcsname{43.7}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/blur3\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/blur3/pct\endcsname{95}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/bright\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/bright/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/contrast\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/contrast/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/crop50\endcsname{0.59}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/crop50/pct\endcsname{59}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/crop75\endcsname{0.89}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/crop75/pct\endcsname{89}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/excerpt2.5\endcsname{0.92}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/excerpt2.5/pct\endcsname{92}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/fps15\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/fps15/pct\endcsname{96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/gray\endcsname{0.94}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/gray/pct\endcsname{94}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h264_crf28\endcsname{0.98}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h264_crf28/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h264_crf35\endcsname{0.97}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h264_crf35/pct\endcsname{97}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h265_crf32\endcsname{0.97}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/h265_crf32/pct\endcsname{98}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/hflip\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/hflip/pct\endcsname{96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/insert\endcsname{0.53}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/insert/pct\endcsname{52}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/letterbox\endcsname{0.95}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/letterbox/pct\endcsname{95}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/logo\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/logo/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/noise\endcsname{0.91}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/noise/pct\endcsname{91}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/pip\endcsname{0.12}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/pip/pct\endcsname{12}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/resize0.25\endcsname{0.93}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/resize0.25/pct\endcsname{92}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/rot5\endcsname{0.91}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/rot5/pct\endcsname{91}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/rot90\endcsname{0.76}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/rot90/pct\endcsname{76}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/screenrec\endcsname{0.82}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/screenrec/pct\endcsname{82}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/speed1.25\endcsname{0.76}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/speed1.25/pct\endcsname{76}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/text\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/att/text/pct\endcsname{100}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/bits\endcsname{61440}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/chain\endcsname{0.82}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/codec\endcsname{0.97}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/crop\endcsname{0.74}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/geometric\endcsname{0.89}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/overlay\endcsname{0.71}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/photometric\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/scale\endcsname{0.96}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/fam/temporal\endcsname{0.79}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/ms\endcsname{136}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/muAP\endcsname{0.691}
\expandafter\def\csname val@fp:video/DINOv2-S-seq/muAP/pct\endcsname{69.1}
\expandafter\def\csname val@fp:video/ISCC-Video-256/FPRq@query@0.01\endcsname{0.068}
\expandafter\def\csname val@fp:video/ISCC-Video-256/FPRq@query@0.01/pct\endcsname{6.8}
\expandafter\def\csname val@fp:video/ISCC-Video-256/R@1\endcsname{0.801}
\expandafter\def\csname val@fp:video/ISCC-Video-256/R@1/pct\endcsname{80.1}
\expandafter\def\csname val@fp:video/ISCC-Video-256/R@10\endcsname{0.851}
\expandafter\def\csname val@fp:video/ISCC-Video-256/R@10/pct\endcsname{85.1}
\expandafter\def\csname val@fp:video/ISCC-Video-256/TPR@pair@0.0001\endcsname{0.664}
\expandafter\def\csname val@fp:video/ISCC-Video-256/TPR@pair@0.0001/pct\endcsname{66.4}
\expandafter\def\csname val@fp:video/ISCC-Video-256/TPR@query@0.01\endcsname{0.652}
\expandafter\def\csname val@fp:video/ISCC-Video-256/TPR@query@0.01/pct\endcsname{65.2}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/bright\endcsname{0.99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/bright/pct\endcsname{99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/contrast\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/contrast/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/crop50\endcsname{0.11}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/crop50/pct\endcsname{11}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/crop75\endcsname{0.68}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/crop75/pct\endcsname{68}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/excerpt2.5\endcsname{0.98}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/excerpt2.5/pct\endcsname{98}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h265_crf32\endcsname{0.99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/h265_crf32/pct\endcsname{99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/hflip\endcsname{0.12}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/hflip/pct\endcsname{12}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/insert\endcsname{0.57}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/insert/pct\endcsname{57}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/letterbox\endcsname{0.78}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/letterbox/pct\endcsname{78}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/logo\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/logo/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/noise\endcsname{0.99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/noise/pct\endcsname{99}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/pip\endcsname{0.01}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/pip/pct\endcsname{1}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/rot5\endcsname{0.86}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/rot5/pct\endcsname{86}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/screenrec\endcsname{0.96}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/screenrec/pct\endcsname{96}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/speed1.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/speed1.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/text\endcsname{0.98}
\expandafter\def\csname val@fp:video/ISCC-Video-256/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:video/ISCC-Video-256/bits\endcsname{256}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/chain\endcsname{0.96}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/crop\endcsname{0.39}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/geometric\endcsname{0.44}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/overlay\endcsname{0.66}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/photometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-256/fam/temporal\endcsname{0.89}
\expandafter\def\csname val@fp:video/ISCC-Video-256/ms\endcsname{54}
\expandafter\def\csname val@fp:video/ISCC-Video-256/muAP\endcsname{0.749}
\expandafter\def\csname val@fp:video/ISCC-Video-256/muAP/pct\endcsname{74.9}
\expandafter\def\csname val@fp:video/ISCC-Video-64/FPRq@query@0.01\endcsname{0.062}
\expandafter\def\csname val@fp:video/ISCC-Video-64/FPRq@query@0.01/pct\endcsname{6.2}
\expandafter\def\csname val@fp:video/ISCC-Video-64/R@1\endcsname{0.731}
\expandafter\def\csname val@fp:video/ISCC-Video-64/R@1/pct\endcsname{73.1}
\expandafter\def\csname val@fp:video/ISCC-Video-64/R@10\endcsname{0.817}
\expandafter\def\csname val@fp:video/ISCC-Video-64/R@10/pct\endcsname{81.7}
\expandafter\def\csname val@fp:video/ISCC-Video-64/TPR@pair@0.0001\endcsname{0.634}
\expandafter\def\csname val@fp:video/ISCC-Video-64/TPR@pair@0.0001/pct\endcsname{63.4}
\expandafter\def\csname val@fp:video/ISCC-Video-64/TPR@query@0.01\endcsname{0.620}
\expandafter\def\csname val@fp:video/ISCC-Video-64/TPR@query@0.01/pct\endcsname{62.0}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/bright\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/bright/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/contrast\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/contrast/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/crop50\endcsname{0.03}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/crop50/pct\endcsname{2}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/crop75\endcsname{0.33}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/crop75/pct\endcsname{32}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/excerpt2.5\endcsname{0.88}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/excerpt2.5/pct\endcsname{88}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h265_crf32\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/h265_crf32/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/hflip\endcsname{0.07}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/hflip/pct\endcsname{7}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/insert\endcsname{0.33}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/insert/pct\endcsname{33}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/letterbox\endcsname{0.49}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/letterbox/pct\endcsname{49}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/logo\endcsname{0.99}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/logo/pct\endcsname{99}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/noise\endcsname{0.98}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/noise/pct\endcsname{98}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/pip\endcsname{0.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/pip/pct\endcsname{0}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/rot5\endcsname{0.42}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/rot5/pct\endcsname{42}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/screenrec\endcsname{0.82}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/screenrec/pct\endcsname{82}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/speed1.25\endcsname{0.99}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/speed1.25/pct\endcsname{99}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/text\endcsname{0.95}
\expandafter\def\csname val@fp:video/ISCC-Video-64/att/text/pct\endcsname{95}
\expandafter\def\csname val@fp:video/ISCC-Video-64/bits\endcsname{64.0}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/chain\endcsname{0.82}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/crop\endcsname{0.18}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/geometric\endcsname{0.25}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/overlay\endcsname{0.65}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/photometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/ISCC-Video-64/fam/temporal\endcsname{0.80}
\expandafter\def\csname val@fp:video/ISCC-Video-64/ms\endcsname{54}
\expandafter\def\csname val@fp:video/ISCC-Video-64/muAP\endcsname{0.700}
\expandafter\def\csname val@fp:video/ISCC-Video-64/muAP/pct\endcsname{70.0}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/FPRq@query@0.01\endcsname{0.036}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/FPRq@query@0.01/pct\endcsname{3.6}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/R@1\endcsname{0.958}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/R@1/pct\endcsname{95.8}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/R@10\endcsname{0.998}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/R@10/pct\endcsname{99.8}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/TPR@pair@0.0001\endcsname{0.697}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/TPR@pair@0.0001/pct\endcsname{69.7}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/TPR@query@0.01\endcsname{0.543}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/TPR@query@0.01/pct\endcsname{54.3}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/bright\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/bright/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/contrast\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/contrast/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/crop50\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/crop50/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/crop75\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/crop75/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/excerpt2.5\endcsname{0.97}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/excerpt2.5/pct\endcsname{97}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h265_crf32\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/h265_crf32/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/hflip\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/hflip/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/insert\endcsname{0.95}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/insert/pct\endcsname{95}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/letterbox\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/letterbox/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/logo\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/logo/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/noise\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/noise/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/pip\endcsname{0.11}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/pip/pct\endcsname{11}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/rot5\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/rot5/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/rot90\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/rot90/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/screenrec\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/screenrec/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/speed1.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/speed1.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/text\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/att/text/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/bits\endcsname{16384}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/chain\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/crop\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/geometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/overlay\endcsname{0.70}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/photometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/fam/temporal\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/ms\endcsname{137}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/muAP\endcsname{0.893}
\expandafter\def\csname val@fp:video/SSCD-mixup-mean/muAP/pct\endcsname{89.3}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/FPRq@query@0.01\endcsname{0.032}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/FPRq@query@0.01/pct\endcsname{3.2}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/R@1\endcsname{0.921}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/R@1/pct\endcsname{92.1}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/R@10\endcsname{0.998}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/R@10/pct\endcsname{99.8}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/TPR@pair@0.0001\endcsname{0.535}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/TPR@pair@0.0001/pct\endcsname{53.5}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/TPR@query@0.01\endcsname{0.502}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/TPR@query@0.01/pct\endcsname{50.2}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/blur3\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/blur3/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/bright\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/bright/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/contrast\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/contrast/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/crop50\endcsname{0.92}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/crop50/pct\endcsname{92}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/crop75\endcsname{0.96}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/crop75/pct\endcsname{96}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/excerpt2.5\endcsname{0.93}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/excerpt2.5/pct\endcsname{93}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/fps15\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/fps15/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/gray\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/gray/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h264_crf28\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h264_crf28/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h264_crf35\endcsname{0.97}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h264_crf35/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h265_crf32\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/h265_crf32/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/hflip\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/hflip/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/insert\endcsname{0.66}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/insert/pct\endcsname{66}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/letterbox\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/letterbox/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/logo\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/logo/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/noise\endcsname{0.97}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/noise/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/pip\endcsname{0.07}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/pip/pct\endcsname{7}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/resize0.25\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/resize0.25/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/resize0.5\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/resize0.5/pct\endcsname{99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/rot5\endcsname{0.95}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/rot5/pct\endcsname{95}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/rot90\endcsname{0.95}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/rot90/pct\endcsname{95}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/screenrec\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/screenrec/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/speed1.25\endcsname{0.81}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/speed1.25/pct\endcsname{81}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/text\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/bits\endcsname{81920}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/chain\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/codec\endcsname{0.98}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/crop\endcsname{0.94}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/geometric\endcsname{0.97}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/overlay\endcsname{0.68}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/photometric\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/scale\endcsname{0.99}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/fam/temporal\endcsname{0.85}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/ms\endcsname{137}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/muAP\endcsname{0.806}
\expandafter\def\csname val@fp:video/SSCD-mixup-seq/muAP/pct\endcsname{80.6}
\expandafter\def\csname val@fp:video/TMK+PDQF/FPRq@query@0.01\endcsname{0.066}
\expandafter\def\csname val@fp:video/TMK+PDQF/FPRq@query@0.01/pct\endcsname{6.6}
\expandafter\def\csname val@fp:video/TMK+PDQF/R@1\endcsname{0.778}
\expandafter\def\csname val@fp:video/TMK+PDQF/R@1/pct\endcsname{77.8}
\expandafter\def\csname val@fp:video/TMK+PDQF/R@10\endcsname{0.825}
\expandafter\def\csname val@fp:video/TMK+PDQF/R@10/pct\endcsname{82.5}
\expandafter\def\csname val@fp:video/TMK+PDQF/TPR@pair@0.0001\endcsname{0.635}
\expandafter\def\csname val@fp:video/TMK+PDQF/TPR@pair@0.0001/pct\endcsname{63.5}
\expandafter\def\csname val@fp:video/TMK+PDQF/TPR@query@0.01\endcsname{0.631}
\expandafter\def\csname val@fp:video/TMK+PDQF/TPR@query@0.01/pct\endcsname{63.1}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/bright\endcsname{0.99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/bright/pct\endcsname{99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/contrast\endcsname{0.99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/contrast/pct\endcsname{99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/crop50\endcsname{0.02}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/crop50/pct\endcsname{2}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/crop75\endcsname{0.38}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/crop75/pct\endcsname{38}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/excerpt2.5\endcsname{0.97}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/excerpt2.5/pct\endcsname{97}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h265_crf32\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/h265_crf32/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/hflip\endcsname{0.05}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/hflip/pct\endcsname{5}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/insert\endcsname{0.58}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/insert/pct\endcsname{58}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/letterbox\endcsname{0.88}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/letterbox/pct\endcsname{88}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/logo\endcsname{0.98}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/logo/pct\endcsname{98}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/noise\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/noise/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/pip\endcsname{0.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/pip/pct\endcsname{0}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/rot5\endcsname{0.66}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/rot5/pct\endcsname{66}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/screenrec\endcsname{0.99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/screenrec/pct\endcsname{99}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/speed1.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/speed1.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/text\endcsname{0.97}
\expandafter\def\csname val@fp:video/TMK+PDQF/att/text/pct\endcsname{98}
\expandafter\def\csname val@fp:video/TMK+PDQF/bits\endcsname{2106752}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/chain\endcsname{0.99}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/crop\endcsname{0.20}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/geometric\endcsname{0.40}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/overlay\endcsname{0.65}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/photometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/TMK+PDQF/fam/temporal\endcsname{0.89}
\expandafter\def\csname val@fp:video/TMK+PDQF/ms\endcsname{51}
\expandafter\def\csname val@fp:video/TMK+PDQF/muAP\endcsname{0.723}
\expandafter\def\csname val@fp:video/TMK+PDQF/muAP/pct\endcsname{72.3}
\expandafter\def\csname val@fp:video/cal_sources\endcsname{20}
\expandafter\def\csname val@fp:video/fprq/cihi\endcsname{17}
\expandafter\def\csname val@fp:video/fprq/max\endcsname{6.8}
\expandafter\def\csname val@fp:video/fprq/min\endcsname{3.2}
\expandafter\def\csname val@fp:video/q_per_source\endcsname{25}
\expandafter\def\csname val@fp:video/test_sources\endcsname{20}
\expandafter\def\csname val@fp:video/vPDQ/FPRq@query@0.01\endcsname{0.032}
\expandafter\def\csname val@fp:video/vPDQ/FPRq@query@0.01/pct\endcsname{3.2}
\expandafter\def\csname val@fp:video/vPDQ/R@1\endcsname{0.628}
\expandafter\def\csname val@fp:video/vPDQ/R@1/pct\endcsname{62.8}
\expandafter\def\csname val@fp:video/vPDQ/R@10\endcsname{0.641}
\expandafter\def\csname val@fp:video/vPDQ/R@10/pct\endcsname{64.1}
\expandafter\def\csname val@fp:video/vPDQ/TPR@pair@0.0001\endcsname{0.609}
\expandafter\def\csname val@fp:video/vPDQ/TPR@pair@0.0001/pct\endcsname{60.9}
\expandafter\def\csname val@fp:video/vPDQ/TPR@query@0.01\endcsname{0.577}
\expandafter\def\csname val@fp:video/vPDQ/TPR@query@0.01/pct\endcsname{57.7}
\expandafter\def\csname val@fp:video/vPDQ/att/blur3\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/blur3/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/bright\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/bright/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/contrast\endcsname{0.98}
\expandafter\def\csname val@fp:video/vPDQ/att/contrast/pct\endcsname{98}
\expandafter\def\csname val@fp:video/vPDQ/att/crop50\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/crop50/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/crop75\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/crop75/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/excerpt2.5\endcsname{0.59}
\expandafter\def\csname val@fp:video/vPDQ/att/excerpt2.5/pct\endcsname{59}
\expandafter\def\csname val@fp:video/vPDQ/att/fps15\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/fps15/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/gray\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/gray/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/h264_crf28\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/h264_crf28/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/h264_crf35\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/h264_crf35/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/h265_crf32\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/h265_crf32/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/hflip\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/hflip/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/insert\endcsname{0.34}
\expandafter\def\csname val@fp:video/vPDQ/att/insert/pct\endcsname{34}
\expandafter\def\csname val@fp:video/vPDQ/att/letterbox\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/letterbox/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/logo\endcsname{0.97}
\expandafter\def\csname val@fp:video/vPDQ/att/logo/pct\endcsname{97}
\expandafter\def\csname val@fp:video/vPDQ/att/noise\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/noise/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/none/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/pip\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/pip/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/resize0.25\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/resize0.25/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/resize0.5\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/att/resize0.5/pct\endcsname{100}
\expandafter\def\csname val@fp:video/vPDQ/att/rot5\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/rot5/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/rot90\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/rot90/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/screenrec\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/att/screenrec/pct\endcsname{0}
\expandafter\def\csname val@fp:video/vPDQ/att/speed1.25\endcsname{0.88}
\expandafter\def\csname val@fp:video/vPDQ/att/speed1.25/pct\endcsname{88}
\expandafter\def\csname val@fp:video/vPDQ/att/text\endcsname{0.93}
\expandafter\def\csname val@fp:video/vPDQ/att/text/pct\endcsname{93}
\expandafter\def\csname val@fp:video/vPDQ/bits\endcsname{1258}
\expandafter\def\csname val@fp:video/vPDQ/fam/chain\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/codec\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/crop\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/geometric\endcsname{0.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/none\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/overlay\endcsname{0.63}
\expandafter\def\csname val@fp:video/vPDQ/fam/photometric\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/scale\endcsname{1.00}
\expandafter\def\csname val@fp:video/vPDQ/fam/temporal\endcsname{0.70}
\expandafter\def\csname val@fp:video/vPDQ/ms\endcsname{132}
\expandafter\def\csname val@fp:video/vPDQ/muAP\endcsname{0.617}
\expandafter\def\csname val@fp:video/vPDQ/muAP/pct\endcsname{61.7}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/_all/fp/pct\endcsname{37}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/_all/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/aac_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/aac_64/wm/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/babble_0db/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/babble_0db/wm/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/babble_10db/fp/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/babble_10db/wm/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/compressor/fp/pct\endcsname{42}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/compressor/wm/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt10/fp/pct\endcsname{34}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt10/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt10_mp3_noise20/fp/pct\endcsname{3}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt10_mp3_noise20/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/excerpt5/wm/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/lowpass_2k/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/lowpass_2k/wm/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/mp3_64/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/mp3_64/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/noise_10db/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/noise_10db/wm/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/noise_20db/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/noise_20db/wm/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/none/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/opus_24/fp/pct\endcsname{60}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/opus_24/wm/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/phone/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/phone/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/pitch+2/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/pitch+2/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/rerecord/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/rerecord/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/resample_8k/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/resample_8k/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/reverb/fp/pct\endcsname{43}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/reverb/wm/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/speed_1.05/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/speed_1.05/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/tempo_0.9/fp/pct\endcsname{72}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/tempo_0.9/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/tempo_1.1/fp/pct\endcsname{56}
\expandafter\def\csname val@fp:wm/audio/CLAP/att/tempo_1.1/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/CLAP/both/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/audio/CLAP/either/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/CLAP/fp/pct\endcsname{37}
\expandafter\def\csname val@fp:wm/audio/CLAP/fp_only/pct\endcsname{25}
\expandafter\def\csname val@fp:wm/audio/CLAP/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/CLAP/wm_only/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/_all/fp/pct\endcsname{67}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/_all/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/aac_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/aac_64/wm/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/babble_0db/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/babble_0db/wm/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/babble_10db/fp/pct\endcsname{94}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/babble_10db/wm/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/compressor/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/compressor/wm/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt10/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt10/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt10_mp3_noise20/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt10_mp3_noise20/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt5/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/excerpt5/wm/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/lowpass_2k/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/lowpass_2k/wm/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/mp3_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/mp3_64/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/noise_10db/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/noise_10db/wm/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/noise_20db/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/noise_20db/wm/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/none/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/opus_24/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/opus_24/wm/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/phone/fp/pct\endcsname{30}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/phone/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/pitch+2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/pitch+2/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/rerecord/fp/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/rerecord/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/resample_8k/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/resample_8k/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/reverb/fp/pct\endcsname{81}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/reverb/wm/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/speed_1.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/speed_1.05/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/tempo_0.9/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/tempo_0.9/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/tempo_1.1/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/att/tempo_1.1/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/both/pct\endcsname{21}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/either/pct\endcsname{71}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/fp/pct\endcsname{67}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/fp_only/pct\endcsname{46}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/Chromaprint/wm_only/pct\endcsname{3}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/_all/fp/pct\endcsname{46}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/_all/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/aac_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/aac_64/wm/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/babble_0db/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/babble_0db/wm/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/babble_10db/fp/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/babble_10db/wm/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/compressor/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/compressor/wm/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt10/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt10/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt10_mp3_noise20/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt10_mp3_noise20/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/excerpt5/wm/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/lowpass_2k/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/lowpass_2k/wm/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/mp3_64/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/mp3_64/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/noise_10db/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/noise_10db/wm/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/noise_20db/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/noise_20db/wm/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/none/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/opus_24/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/opus_24/wm/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/phone/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/phone/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/pitch+2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/pitch+2/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/rerecord/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/rerecord/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/resample_8k/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/resample_8k/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/reverb/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/reverb/wm/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/speed_1.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/speed_1.05/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/tempo_0.9/fp/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/tempo_0.9/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/tempo_1.1/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/att/tempo_1.1/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/both/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/either/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/fp/pct\endcsname{46}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/fp_only/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-256/wm_only/pct\endcsname{7}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/_all/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/_all/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/aac_64/fp/pct\endcsname{94}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/aac_64/wm/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/babble_0db/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/babble_0db/wm/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/babble_10db/fp/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/babble_10db/wm/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/compressor/fp/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/compressor/wm/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt10/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt10/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt10_mp3_noise20/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt10_mp3_noise20/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/excerpt5/wm/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/lowpass_2k/fp/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/lowpass_2k/wm/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/mp3_64/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/mp3_64/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/noise_10db/fp/pct\endcsname{74}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/noise_10db/wm/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/noise_20db/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/noise_20db/wm/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/none/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/none/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/opus_24/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/opus_24/wm/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/phone/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/phone/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/pitch+2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/pitch+2/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/rerecord/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/rerecord/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/resample_8k/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/resample_8k/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/reverb/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/reverb/wm/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/speed_1.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/speed_1.05/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/tempo_0.9/fp/pct\endcsname{19}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/tempo_0.9/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/tempo_1.1/fp/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/att/tempo_1.1/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/both/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/either/pct\endcsname{48}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/fp_only/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/ISCC-Audio-64/wm_only/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/_all/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/_all/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/aac_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/aac_64/wm/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/babble_0db/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/babble_0db/wm/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/babble_10db/fp/pct\endcsname{86}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/babble_10db/wm/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/compressor/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/compressor/wm/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt10/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt10/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt10_mp3_noise20/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt10_mp3_noise20/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt5/fp/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/excerpt5/wm/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/lowpass_2k/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/lowpass_2k/wm/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/mp3_64/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/mp3_64/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/noise_10db/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/noise_10db/wm/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/noise_20db/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/noise_20db/wm/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/none/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/opus_24/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/opus_24/wm/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/phone/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/phone/wm/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/pitch+2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/pitch+2/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/rerecord/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/rerecord/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/resample_8k/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/resample_8k/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/reverb/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/reverb/wm/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/speed_1.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/speed_1.05/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/tempo_0.9/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/tempo_0.9/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/tempo_1.1/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/att/tempo_1.1/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/audio/audfprint/both/pct\endcsname{23}
\expandafter\def\csname val@fp:wm/audio/audfprint/either/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/audio/audfprint/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/audio/audfprint/fp_only/pct\endcsname{41}
\expandafter\def\csname val@fp:wm/audio/audfprint/wm/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/audio/audfprint/wm_only/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/falsekey/k\endcsname{1}
\expandafter\def\csname val@fp:wm/audio/falsekey/n\endcsname{8{,}400}
\expandafter\def\csname val@fp:wm/audio/falsekey/nsrc\endcsname{400}
\expandafter\def\csname val@fp:wm/audio/falsekey/pct\endcsname{0.01}
\expandafter\def\csname val@fp:wm/audio/falsekey_registry/pct\endcsname{0.00}
\expandafter\def\csname val@fp:wm/audio/keyok/colliding\endcsname{18}
\expandafter\def\csname val@fp:wm/audio/keyok/n\endcsname{1{,}020}
\expandafter\def\csname val@fp:wm/audio/keyok/pct1\endcsname{24.3}
\expandafter\def\csname val@fp:wm/audio/keyok/unique/pct\endcsname{23.9}
\expandafter\def\csname val@fp:wm/audio/n_assets\endcsname{200}
\expandafter\def\csname val@fp:wm/audio/n_colliding\endcsname{2}
\expandafter\def\csname val@fp:wm/audio/n_queries\endcsname{4{,}200}
\expandafter\def\csname val@fp:wm/audio/nkeys\endcsname{199}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/BlockMean/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/BlockMean/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/BlockMean/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/BlockMean/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/BlockMean/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/Blockhash-256/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ColorMoment/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ColorMoment/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ColorMoment/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ColorMoment/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/_all/fp/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/blur2/fp/pct\endcsname{21}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/bright0.6/fp/pct\endcsname{17}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/bright1.4/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/contrast0.5/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop90/fp/pct\endcsname{3}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/emoji0.3/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/gamma0.6/fp/pct\endcsname{17}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/gray/fp/pct\endcsname{17}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/hflip/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg30/fp/pct\endcsname{30}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg50/fp/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg75/fp/pct\endcsname{87}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/meme/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/noise0.05/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/perspective/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/pixelize0.3/fp/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/recapture/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/resize0.25/fp/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/resize0.5/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot5/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/sat2/fp/pct\endcsname{29}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/social/fp/pct\endcsname{3}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/text/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/webp50/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/both/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/drift/pct\endcsname{64.0}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/either/pct\endcsname{63}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/fp/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/fp_only/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/unmarkedreg/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOHash-96/wm_only/pct\endcsname{41}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/_all/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/blur2/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/bright0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/bright1.4/fp/pct\endcsname{56}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/contrast0.5/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop50/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop50off/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop70/fp/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop90/fp/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/emoji0.3/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/gamma0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/gray/fp/pct\endcsname{79}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/hflip/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg30/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg50/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/meme/fp/pct\endcsname{81}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/noise0.05/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/pad25/fp/pct\endcsname{27}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/perspective/fp/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/recapture/fp/pct\endcsname{60}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/resize0.25/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot15/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot5/fp/pct\endcsname{46}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot90/fp/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/sat2/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/skew/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/social/fp/pct\endcsname{56}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/text/fp/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/webp50/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/both/pct\endcsname{56}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/drift/pct\endcsname{9.0}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/either/pct\endcsname{70}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/fp_only/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/unmarkedreg/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-B/wm_only/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/_all/fp/pct\endcsname{51}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/blur2/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/bright0.6/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/bright1.4/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/contrast0.5/fp/pct\endcsname{89}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop70/fp/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop90/fp/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/emoji0.3/fp/pct\endcsname{41}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/gamma0.6/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/gray/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/hflip/fp/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg30/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg50/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg75/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/meme/fp/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/noise0.05/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/pad25/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/perspective/fp/pct\endcsname{26}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/pixelize0.3/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/recapture/fp/pct\endcsname{23}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/resize0.25/fp/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot15/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot5/fp/pct\endcsname{11}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot90/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/sat2/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/skew/fp/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/social/fp/pct\endcsname{31}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/text/fp/pct\endcsname{73}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/webp50/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/both/pct\endcsname{47}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/drift/pct\endcsname{21.3}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/either/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/fp/pct\endcsname{51}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/fp_only/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/unmarkedreg/fp/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-S-LSH256/wm_only/pct\endcsname{15}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/_all/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/blur2/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/bright0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/bright1.4/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/contrast0.5/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop70/fp/pct\endcsname{7}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop90/fp/pct\endcsname{70}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/emoji0.3/fp/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/gamma0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/gray/fp/pct\endcsname{76}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/hflip/fp/pct\endcsname{68}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg30/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg50/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/meme/fp/pct\endcsname{83}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/noise0.05/fp/pct\endcsname{89}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/pad25/fp/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/perspective/fp/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/recapture/fp/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/resize0.25/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot15/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot5/fp/pct\endcsname{31}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot90/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/sat2/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/skew/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/social/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/text/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/webp50/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/both/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/drift/pct\endcsname{5.7}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/either/pct\endcsname{69}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/fp_only/pct\endcsname{7}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/unmarkedreg/fp/pct\endcsname{53}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/DINOv2-S/wm_only/pct\endcsname{7}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/_all/fp/pct\endcsname{76}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/blur2/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/bright0.6/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/bright1.4/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/contrast0.5/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop70/fp/pct\endcsname{48}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop90/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/emoji0.3/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/gamma0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/gray/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/hflip/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg30/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg50/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/meme/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/noise0.05/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/pad25/fp/pct\endcsname{59}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/perspective/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/pixelize0.3/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/recapture/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/resize0.25/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot15/fp/pct\endcsname{75}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot5/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot90/fp/pct\endcsname{9}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/sat2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/skew/fp/pct\endcsname{71}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/social/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/text/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/webp50/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/both/pct\endcsname{60}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/drift/pct\endcsname{8.7}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/either/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/fp/pct\endcsname{76}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/fp_only/pct\endcsname{16}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/unmarkedreg/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISC21-1st/wm_only/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/_all/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/bright0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/bright1.4/fp/pct\endcsname{9}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/contrast0.5/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop90/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/emoji0.3/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/gamma0.6/fp/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg30/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg50/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg75/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/noise0.05/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/pad25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/perspective/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/recapture/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/sat2/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/text/fp/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/webp50/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/both/pct\endcsname{45}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/drift/pct\endcsname{56.7}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/either/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/fp_only/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/unmarkedreg/fp/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-256/wm_only/pct\endcsname{17}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/_all/fp/pct\endcsname{47}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/bright0.6/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/bright1.4/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/contrast0.5/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop90/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/emoji0.3/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/gamma0.6/fp/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/gray/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg30/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg50/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg75/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/noise0.05/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/pad25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/perspective/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/recapture/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/resize0.25/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/resize0.5/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/sat2/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/social/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/text/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/webp50/fp/pct\endcsname{89}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/both/pct\endcsname{43}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/drift/pct\endcsname{62.0}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/either/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/fp/pct\endcsname{47}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/fp_only/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/unmarkedreg/fp/pct\endcsname{19}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/ISCC-Image-64/wm_only/pct\endcsname{19}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/_all/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/bright0.6/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/bright1.4/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/contrast0.5/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/emoji0.3/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/gamma0.6/fp/pct\endcsname{86}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg30/fp/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg50/fp/pct\endcsname{59}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg75/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/noise0.05/fp/pct\endcsname{24}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/resize0.25/fp/pct\endcsname{76}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/resize0.5/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/sat2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/text/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/webp50/fp/pct\endcsname{45}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/both/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/drift/pct\endcsname{82.0}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/either/pct\endcsname{63}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/fp_only/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/unmarkedreg/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/MarrHildreth/wm_only/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/_all/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/blur2/fp/pct\endcsname{63}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/bright0.6/fp/pct\endcsname{15}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/bright1.4/fp/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/contrast0.5/fp/pct\endcsname{13}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop70/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop90/fp/pct\endcsname{51}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/emoji0.3/fp/pct\endcsname{13}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/gamma0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/gray/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/hflip/fp/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg30/fp/pct\endcsname{43}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg50/fp/pct\endcsname{73}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg75/fp/pct\endcsname{94}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/noise0.05/fp/pct\endcsname{42}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/pad25/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/perspective/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/pixelize0.3/fp/pct\endcsname{79}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/recapture/fp/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/resize0.25/fp/pct\endcsname{71}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot90/fp/pct\endcsname{3}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/sat2/fp/pct\endcsname{94}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/skew/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/text/fp/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/webp50/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/both/pct\endcsname{34}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/drift/pct\endcsname{4.3}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/either/pct\endcsname{63}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/fp_only/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/unmarkedreg/fp/pct\endcsname{26}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/OpenCLIP-B32/wm_only/pct\endcsname{29}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/_all/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/bright0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/bright1.4/fp/pct\endcsname{74}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/contrast0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/emoji0.3/fp/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/gamma0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/hflip/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg30/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg50/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/noise0.05/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/recapture/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/resize0.25/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/resize0.5/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot90/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/sat2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/squash0.75/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/text/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/webp50/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/both/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/drift/pct\endcsname{0.3}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/either/pct\endcsname{67}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/fp_only/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/unmarkedreg/fp/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/PDQ-dihedral/wm_only/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/image/PDQ/att/_all/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/PDQ/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/PDQ/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/bright0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/bright1.4/fp/pct\endcsname{77}
\expandafter\def\csname val@fp:wm/image/PDQ/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/PDQ/att/contrast0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/emoji0.3/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/image/PDQ/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/PDQ/att/gamma0.6/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/PDQ/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg30/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg50/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/noise0.05/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/perspective/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/PDQ/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/PDQ/att/pixelize0.3/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/recapture/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/PDQ/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/PDQ/att/resize0.25/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/PDQ/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/resize0.5/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/PDQ/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/sat2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/PDQ/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/PDQ/att/squash0.75/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/PDQ/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/PDQ/att/text/fp/pct\endcsname{81}
\expandafter\def\csname val@fp:wm/image/PDQ/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/webp50/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/PDQ/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/PDQ/both/pct\endcsname{47}
\expandafter\def\csname val@fp:wm/image/PDQ/drift/pct\endcsname{0.3}
\expandafter\def\csname val@fp:wm/image/PDQ/either/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/PDQ/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/PDQ/fp_only/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/PDQ/unmarkedreg/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/PDQ/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/PDQ/wm_only/pct\endcsname{15}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/_all/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/blur2/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/bright0.6/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/bright1.4/fp/pct\endcsname{48}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/contrast0.5/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop70/fp/pct\endcsname{31}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop90/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/emoji0.3/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/gamma0.6/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/gray/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/hflip/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg30/fp/pct\endcsname{66}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg50/fp/pct\endcsname{73}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg75/fp/pct\endcsname{83}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/meme/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/noise0.05/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/pad25/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/perspective/fp/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/pixelize0.3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/recapture/fp/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/resize0.25/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot15/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot5/fp/pct\endcsname{41}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot90/fp/pct\endcsname{9}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/sat2/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/skew/fp/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/social/fp/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/text/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/webp50/fp/pct\endcsname{69}
\expandafter\def\csname val@fp:wm/image/SSCD-large/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/SSCD-large/both/pct\endcsname{53}
\expandafter\def\csname val@fp:wm/image/SSCD-large/drift/pct\endcsname{33.7}
\expandafter\def\csname val@fp:wm/image/SSCD-large/either/pct\endcsname{70}
\expandafter\def\csname val@fp:wm/image/SSCD-large/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/image/SSCD-large/fp_only/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/SSCD-large/unmarkedreg/fp/pct\endcsname{48}
\expandafter\def\csname val@fp:wm/image/SSCD-large/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/SSCD-large/wm_only/pct\endcsname{9}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/_all/fp/pct\endcsname{68}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/blur2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/bright0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/bright1.4/fp/pct\endcsname{55}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/contrast0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop70/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop90/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/emoji0.3/fp/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/gamma0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/gray/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/hflip/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg30/fp/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg50/fp/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/meme/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/noise0.05/fp/pct\endcsname{69}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/pad25/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/perspective/fp/pct\endcsname{79}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/pixelize0.3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/recapture/fp/pct\endcsname{44}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot5/fp/pct\endcsname{27}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot90/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/sat2/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/skew/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/social/fp/pct\endcsname{75}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/text/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/webp50/fp/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/both/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/drift/pct\endcsname{17.7}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/either/pct\endcsname{72}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/fp/pct\endcsname{68}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/fp_only/pct\endcsname{9}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/unmarkedreg/fp/pct\endcsname{53}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/SSCD-mixup/wm_only/pct\endcsname{4}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/aHash-64/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/aHash-64/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/aHash-64/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/aHash-64/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/aHash-64/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/dHash-64/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/dHash-64/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/dHash-64/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/dHash-64/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/dHash-64/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/falsekey/k\endcsname{487}
\expandafter\def\csname val@fp:wm/image/falsekey/n\endcsname{18{,}000}
\expandafter\def\csname val@fp:wm/image/falsekey/pct\endcsname{2.71}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/_all/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/blur2/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/bright0.6/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/bright1.4/fp/pct\endcsname{72}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/contrast0.5/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/emoji0.3/fp/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/gamma0.6/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg30/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg50/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/noise0.05/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/perspective/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/pixelize0.3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/recapture/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/sat2/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/squash0.75/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/text/fp/pct\endcsname{79}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/webp50/fp/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-256/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/pHash-256/both/pct\endcsname{47}
\expandafter\def\csname val@fp:wm/image/pHash-256/drift/pct\endcsname{0.3}
\expandafter\def\csname val@fp:wm/image/pHash-256/either/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/image/pHash-256/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/pHash-256/fp_only/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/pHash-256/unmarkedreg/fp/pct\endcsname{49}
\expandafter\def\csname val@fp:wm/image/pHash-256/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/pHash-256/wm_only/pct\endcsname{15}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/_all/fp/pct\endcsname{37}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/blur2/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/bright0.6/fp/pct\endcsname{67}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/bright1.4/fp/pct\endcsname{6}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/contrast0.5/fp/pct\endcsname{67}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/emoji0.3/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/gamma0.6/fp/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg30/fp/pct\endcsname{84}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg50/fp/pct\endcsname{85}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg75/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/noise0.05/fp/pct\endcsname{71}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/pixelize0.3/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/recapture/fp/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/resize0.25/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/resize0.5/fp/pct\endcsname{91}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/sat2/fp/pct\endcsname{74}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/squash0.75/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/text/fp/pct\endcsname{14}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/webp50/fp/pct\endcsname{84}
\expandafter\def\csname val@fp:wm/image/pHash-64/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/pHash-64/both/pct\endcsname{36}
\expandafter\def\csname val@fp:wm/image/pHash-64/drift/pct\endcsname{22.3}
\expandafter\def\csname val@fp:wm/image/pHash-64/either/pct\endcsname{63}
\expandafter\def\csname val@fp:wm/image/pHash-64/fp/pct\endcsname{37}
\expandafter\def\csname val@fp:wm/image/pHash-64/fp_only/pct\endcsname{1}
\expandafter\def\csname val@fp:wm/image/pHash-64/unmarkedreg/fp/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/image/pHash-64/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/pHash-64/wm_only/pct\endcsname{26}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/_all/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/_all/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/background0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/background0.5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/blur2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/blur2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/bright0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/bright0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/bright1.4/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/bright1.4/wm/pct\endcsname{33}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/contrast0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/contrast0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop30/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop50/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop50off/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop50off/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop70/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop70/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/crop90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/emoji0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/emoji0.3/wm/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/gamma0.6/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/gamma0.6/wm/pct\endcsname{99}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/gray/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/gray/wm/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg30/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg30/wm/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg50/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/jpeg75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/meme/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/meme/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/noise0.05/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/noise0.05/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/none/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/pad25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/pad25/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/perspective/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/perspective/wm/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/pixelize0.3/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/pixelize0.3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/recapture/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/recapture/wm/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/resize0.25/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/resize0.5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot15/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot15/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot5/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/rot90/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/sat2/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/sat2/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/screenshot/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/screenshot/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/skew/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/skew/wm/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/social/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/social/wm/pct\endcsname{97}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/squash0.75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/squash0.75/wm/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/text/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/webp50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/att/webp50/wm/pct\endcsname{96}
\expandafter\def\csname val@fp:wm/image/wHash-64/both/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/drift/pct\endcsname{100.0}
\expandafter\def\csname val@fp:wm/image/wHash-64/either/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/wHash-64/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/unmarkedreg/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/image/wHash-64/wm/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/image/wHash-64/wm_only/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/_all/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/crop75/fp/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/excerpt2.5/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/gray/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/hflip/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/insert/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/letterbox/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/noise/fp/pct\endcsname{18}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/resize0.25/fp/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/rot5/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/screenrec/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/speed1.25/fp/pct\endcsname{82}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/text/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/both/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/fp/pct\endcsname{61}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-mean/wm_only/pct\endcsname{31}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/_all/fp/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/crop75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/excerpt2.5/fp/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/fps15/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/gray/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h264_crf35/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h265_crf32/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/hflip/fp/pct\endcsname{70}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/insert/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/letterbox/fp/pct\endcsname{10}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/noise/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/resize0.25/fp/pct\endcsname{45}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/screenrec/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/speed1.25/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/text/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/both/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/fp/pct\endcsname{50}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/DINOv2-S-seq/wm_only/pct\endcsname{42}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/_all/fp/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/crop75/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/excerpt2.5/fp/pct\endcsname{72}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/insert/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/letterbox/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/noise/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/rot5/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/screenrec/fp/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/speed1.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/text/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/both/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/either/pct\endcsname{93}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/fp/pct\endcsname{65}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-256/wm_only/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/_all/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/crop75/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/excerpt2.5/fp/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/insert/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/letterbox/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/noise/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/rot5/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/screenrec/fp/pct\endcsname{15}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/speed1.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/text/fp/pct\endcsname{85}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/both/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/fp/pct\endcsname{62}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/ISCC-Video-64/wm_only/pct\endcsname{30}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/_all/fp/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/crop75/fp/pct\endcsname{8}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/excerpt2.5/fp/pct\endcsname{42}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/gray/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/hflip/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/insert/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/letterbox/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/noise/fp/pct\endcsname{2}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/resize0.25/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/screenrec/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/speed1.25/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/text/fp/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/both/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/fp/pct\endcsname{57}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-mean/wm_only/pct\endcsname{35}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/_all/fp/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/crop75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/excerpt2.5/fp/pct\endcsname{60}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/fps15/fp/pct\endcsname{90}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/gray/fp/pct\endcsname{32}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/hflip/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/insert/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/letterbox/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/logo/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/noise/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/resize0.25/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/screenrec/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/speed1.25/fp/pct\endcsname{22}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/text/fp/pct\endcsname{52}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/both/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/fp/pct\endcsname{54}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/SSCD-mixup-seq/wm_only/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/_all/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/contrast/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/crop75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/excerpt2.5/fp/pct\endcsname{80}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/insert/fp/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/letterbox/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/logo/fp/pct\endcsname{95}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/noise/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/screenrec/fp/pct\endcsname{38}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/speed1.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/text/fp/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/both/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/fp/pct\endcsname{64}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/TMK+PDQF/wm_only/pct\endcsname{28}
\expandafter\def\csname val@fp:wm/video/falsekey/k\endcsname{0}
\expandafter\def\csname val@fp:wm/video/falsekey/n\endcsname{1{,}000}
\expandafter\def\csname val@fp:wm/video/falsekey/pct\endcsname{0.00}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/_all/fp/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/_all/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/blur3/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/blur3/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/bright/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/bright/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/contrast/fp/pct\endcsname{98}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/contrast/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/crop50/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/crop50/wm/pct\endcsname{20}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/crop75/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/crop75/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/excerpt2.5/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/excerpt2.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/fps15/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/fps15/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/gray/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/gray/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h264_crf28/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h264_crf28/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h264_crf35/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h264_crf35/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h265_crf32/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/h265_crf32/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/hflip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/hflip/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/insert/fp/pct\endcsname{12}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/insert/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/letterbox/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/letterbox/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/logo/fp/pct\endcsname{85}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/logo/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/noise/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/noise/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/none/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/none/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/pip/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/pip/wm/pct\endcsname{5}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/resize0.25/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/resize0.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/resize0.5/fp/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/resize0.5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/rot5/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/rot5/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/rot90/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/rot90/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/screenrec/fp/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/screenrec/wm/pct\endcsname{78}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/speed1.25/fp/pct\endcsname{40}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/speed1.25/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/text/fp/pct\endcsname{88}
\expandafter\def\csname val@fp:wm/video/vPDQ/att/text/wm/pct\endcsname{100}
\expandafter\def\csname val@fp:wm/video/vPDQ/both/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/video/vPDQ/either/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/vPDQ/fp/pct\endcsname{58}
\expandafter\def\csname val@fp:wm/video/vPDQ/fp_only/pct\endcsname{0}
\expandafter\def\csname val@fp:wm/video/vPDQ/wm/pct\endcsname{92}
\expandafter\def\csname val@fp:wm/video/vPDQ/wm_only/pct\endcsname{34}
\makeatother

